The challenge of uncertainty quantification of large language models in medicine

This study investigates uncertainty quantification in large language models (LLMs) for medical applications, emphasizing both technical innovations and philosophical implications. As LLMs become integral to clinical decision-making, accurately communicating uncertainty is crucial for ensuring reliable, safe, and ethical AI-assisted healthcare. Our research frames uncertainty not as a barrier but as an essential part of knowledge that invites a dynamic and reflective approach to AI design. By integrating advanced probabilistic methods such as Bayesian inference, deep ensembles, and Monte Carlo dropout with linguistic analysis that computes predictive and semantic entropy, we propose a comprehensive framework that manages both epistemic and aleatoric uncertainties. The framework incorporates surrogate modeling to address limitations of proprietary APIs, multi-source data integration for better context, and dynamic calibration via continual and meta-learning. Explainability is embedded through uncertainty maps and confidence metrics to support user trust and clinical interpretability. Our approach supports transparent and ethical decision-making aligned with Responsible and Reflective AI principles. Philosophically, we advocate accepting controlled ambiguity instead of striving for absolute predictability, recognizing the inherent provisionality of medical knowledge.

==> main.bbl.tex <==
@inproceedings{Ong2024,
pages = {677-682},
publisher = {IEEE},
series = {2024 21st International Conference on Ubiquitous Robots (UR)},
title = {A Simple Baseline for Uncertainty-Aware Language-Oriented Task Planner for Embodied Agents},
booktitle = {2024 21st International Conference on Ubiquitous Robots (UR)},
isbn = {9798350361087},
year = {2024-6-24},
author = {Ong, Hyobin and Yoon, Youngwoo and Choi, Jaewoo and Jang, Minsu},
}

@article{Kämmer2024,
number = {7},
publisher = {BMJ Publishing Group Ltd,},
title = {Effects of interacting with a large language model compared with a human coach on the clinical diagnostic process and outcomes among fourth-year medical students: study protocol for a prospective, randomised experiment using patient vignettes},
issn = {2044-6055},
journal = {BMJ open.},
lccn = {2011262022},
year = {2024-07-02},
volume = {14},
author = {Kämmer, Juliane E and Hautz, Wolf E and Krummrey, Gert and Sauter, Thomas C and Penders, Dorothea and Birrenbach, Tanja and Bienefeld, Nadine},
address = {[London] :},
}

@article{Cung2024,
number = {2},
pages = {106-115},
publisher = {Blackwell Science, Inc},
title = {The performance of artificial intelligence chatbot large language models to address skeletal biology and bone health queries},
issn = {0884-0431},
journal = {Journal of bone and mineral research : JBMR.},
lccn = {sn 99003247},
year = {2024-03-22},
volume = {39},
author = {Cung, Michelle and Sosa, Branden and Yang, He S and McDonald, Michelle M and Matthews, Brya G and Vlug, Annegreet G and Imel, Erik A and Wein, Marc N and Stein, Emily Margaret and Greenblatt, Matthew B},
address = {Malden, MA :},
}

@article{Cai2024,
publisher = {Institute of Electrical and Electronics Engineers,},
title = {Enhancing Weakly Supervised Semantic Segmentation with Multi-label Contrastive Learning and LLM Features Guidance},
issn = {2168-2194},
journal = {IEEE journal of biomedical and health informatics.},
lccn = {2012200554},
year = {2024},
author = {Cai, Wentian and Li, Yijiang and Chen, Yandan and Lin, Jing and Huang, Zihao and Gao, Ping and Gadekallu, Thippa Reddy and Wang, Wei and Gao, Ying},
address = {New York, NY :},
}

@article{Shin2024,
publisher = {Blackwell Science},
title = {Performance of the ChatGPT large language model for decision support in community pharmacy},
issn = {0306-5251},
journal = {British journal of clinical pharmacology : BJCP.},
lccn = {00242387},
year = {2024-08-27},
author = {Shin, Euibeom and Hartman, Maggie and Ramanathan, Murali},
address = {[Oxford, England] :},
}

@article{Yeung2023,
publisher = {Frontiers Media S.A.,},
title = {AI chatbots not yet ready for clinical use},
issn = {2673-253X},
journal = {Frontiers in digital health.},
lccn = {2021229572},
year = {2023-4-12},
volume = {5},
author = {Au Yeung, Joshua and Kraljevic, Zeljko and Luintel, Akish and Balston, Alfred and Idowu, Esther and Dobson, Richard J and Teo, James T},
address = {[Lausanne, Switzerland] :},
}


@book{kochenderfer2022,
  title={Decision Making Under Uncertainty: Theory and Application},
  author={Kochenderfer, Mykel J. and Amato, Christopher and Chowdhary, Girish and How, Jonathan P. and Reynolds, H. J. and Thornton, Jason and Vian, John},
  year={2022},
  publisher={MIT Press}
}

@Article{Wu2020,
AUTHOR = {Wu, Junyi and Shang, Shari},
TITLE = {Managing Uncertainty in AI-Enabled Decision Making and Achieving Sustainability},
JOURNAL = {Sustainability},
VOLUME = {12},
YEAR = {2020},
NUMBER = {21},
ARTICLE-NUMBER = {8758},
URL = {https://www.mdpi.com/2071-1050/12/21/8758},
ISSN = {2071-1050},
ABSTRACT = {Artificial intelligence (AI) has been applied to various decision-making tasks. However, scholars have yet to comprehend how computers can integrate decision making with uncertainty management. Obtaining such comprehension would enable scholars to deliver sustainable AI decision-making applications that adapt to the changing world. This research examines uncertainties in AI-enabled decision-making applications and some approaches for managing various types of uncertainty. By referring to studies on uncertainty in decision making, this research describes three dimensions of uncertainty, namely informational, environmental and intentional. To understand how to manage uncertainty in AI-enabled decision-making applications, the authors conduct a literature review using content analysis with practical approaches. According to the analysis results, a mechanism related to those practical approaches is proposed for managing diverse types of uncertainty in AI-enabled decision making.},
DOI = {10.3390/su12218758}
}




@article{Gutreuter2022,
number = {3},
publisher = {Public Library of Science,},
title = {Comparative performance of multiple-list estimators of key population size},
issn = {2767-3375},
journal = {PLOS global public health.},
lccn = {2021201877},
year = {2022-3-10},
volume = {2},
author = {Gutreuter, Steve and Wheldon, Mark C},
address = {San Francisco, California :},
}

@article{Sommer2017,
number = {12},
pages = {2853-2863},
publisher = {Butterworth-Heinemann,},
title = {Quality of fracture reduction assessed by radiological parameters and its influence on functional results in patients with pilon fractures—A prospective multicentre study},
issn = {0020-1383},
journal = {Injury.},
lccn = {2007233053},
year = {2017-12},
volume = {48},
author = {Sommer, Christoph and Nork, Sean E and Graves, Matthew and Blauth, Michael and Rudin, Mark and Stoffel, Karl},
address = {Oxford :},
}


@article{Hosseini2023,
abstract = {Objective ChatGPT is the first large language model (LLM) to reach a large, mainstream audience. Its rapid adoption and exploration by the population at large has sparked a wide range of discussions regarding its acceptable and optimal integration in different areas. In a hybrid (virtual and in-person) panel discussion event, we examined various perspectives regarding the use of ChatGPT in education, research, and healthcare. Materials and methods We surveyed in-person and online attendees using an audience interaction platform (Slido). We quantitatively analyzed received responses on questions about the use of ChatGPT in various contexts. We compared pairwise categorical groups with a Fisher's Exact. More trainees had tried ChatGPT compared with faculty. Those who had used ChatGPT were more interested in using it in a wider range of contexts going forwards. Of the three discussed contexts, the greatest uncertainty was shown about using ChatGPT in education. Pros and cons were raised during discussion for the use of this technology in education, research, and healthcare. Discussion There was a range of perspectives around the uses of ChatGPT in education, research, and healthcare, with still much uncertainty around its acceptability and optimal uses. There were different perspectives from respondents of different roles (trainee vs faculty vs staff). More discussion is needed to explore perceptions around the use of LLMs such as ChatGPT in vital sectors such as education, healthcare and research. Given involved risks and unforeseen challenges, taking a thoughtful and measured approach in adoption would reduce the likelihood of harm.},
author = {Hosseini, Mohammad and Gao, Catherine A. and Liebovitz, David M. and Carvalho, Alexandre M. and Ahmad, Faraz S. and Luo, Yuan and MacDonald, Ngan and Holmes, Kristi L. and Kho, Abel},
doi = {10.1371/journal.pone.0292216},
file = {:F\:/Medical 1/paper 2.pdf:pdf},
isbn = {1111111111},
issn = {19326203},
journal = {PLoS ONE},
mendeley-groups = {Certainty},
number = {10 October},
pages = {1--15},
pmid = {37796786},
title = {{An exploratory survey about using ChatGPT in education, healthcare, and research}},
volume = {18},
year = {2023}
}


@InProceedings{Wang2020,
author="Wang, Shuo
and Tarroni, Giacomo
and Qin, Chen
and Mo, Yuanhan
and Dai, Chengliang
and Chen, Chen
and Glocker, Ben
and Guo, Yike
and Rueckert, Daniel
and Bai, Wenjia",
editor="Martel, Anne L.
and Abolmaesumi, Purang
and Stoyanov, Danail
and Mateus, Diana
and Zuluaga, Maria A.
and Zhou, S. Kevin
and Racoceanu, Daniel
and Joskowicz, Leo",
title="Deep Generative Model-Based Quality Control for Cardiac MRI Segmentation",
booktitle="Medical Image Computing and Computer Assisted Intervention -- MICCAI 2020",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="88--97",
abstract="In recent years, convolutional neural networks have demonstrated promising performance in a variety of medical image segmentation tasks. However, when a trained segmentation model is deployed into the real clinical world, the model may not perform optimally. A major challenge is the potential poor-quality segmentations generated due to degraded image quality or domain shift issues. There is a timely need to develop an automated quality control method that can detect poor segmentations and feedback to clinicians. Here we propose a novel deep generative model-based framework for quality control of cardiac MRI segmentation. It first learns a manifold of good-quality image-segmentation pairs using a generative model. The quality of a given test segmentation is then assessed by evaluating the difference from its projection onto the good-quality manifold. In particular, the projection is refined through iterative search in the latent space. The proposed method achieves high prediction accuracy on two publicly available cardiac MRI datasets. Moreover, it shows better generalisation ability than traditional regression-based methods. Our approach provides a real-time and model-agnostic quality control for cardiac MRI segmentation, which has the potential to be integrated into clinical image analysis workflows.",
isbn="978-3-030-59719-1"
}
@misc{jones2021,
      title={Selective Classification Can Magnify Disparities Across Groups}, 
      author={Erik Jones and Shiori Sagawa and Pang Wei Koh and Ananya Kumar and Percy Liang},
      year={2021},
      eprint={2010.14134},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      url={https://arxiv.org/abs/2010.14134}, 
}

@misc{xiong2024,
      title={Can LLMs Express Their Uncertainty? An Empirical Evaluation of Confidence Elicitation in LLMs}, 
      author={Miao Xiong and Zhiyuan Hu and Xinyang Lu and Yifei Li and Jie Fu and Junxian He and Bryan Hooi},
      year={2024},
      eprint={2306.13063},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2306.13063}, 
}



@article{Savage2024,
abstract = {Doi: 10.1093/jamia/ocae254 Journal of the American Medical Informatics Association, 00, 00, 2024 Publication Date: 10/10/2024 Abstract Introduction The inability of large language models (LLMs) to communicate uncertainty is a significant barrier to their use in medicine. Before LLMs can be integrated into patient care, the field must assess methods to estimate uncertainty in ways that are useful to physician-users.Objective Evaluate the ability for uncertainty proxies to quantify LLM confidence when performing diagnosis and treatment selection tasks by assessing the properties of discrimination and calibration.Methods We examined confidence elicitation (CE), token-level probability (TLP), and sample consistency (SC) proxies across GPT3.5, GPT4, Llama2, and Llama3. Uncertainty proxies were evaluated against 3 datasets of open-ended patient scenarios.Results SC discrimination outperformed TLP and CE methods. SC by sentence embedding achieved the highest discriminative performance (ROC AUC 0.68-0.79), yet with poor calibration. SC by GPT annotation achieved the second-best discrimination (ROC AUC 0.66-0.74) with accurate calibration. Verbalized confidence (CE) was found to consistently overestimate model confidence.Discussion and Conclusions SC is the most effective method for estimating LLM uncertainty of the proxies evaluated. SC by sentence embedding can effectively estimate uncertainty if the user has a set of reference cases with which to re-calibrate their results, while SC by GPT annotation is the more effective method if the user does not have reference cases and requires accurate raw calibration. Our results confirm LLMs are consistently over-confident when verbalizing their confidence (CE).},
author = {Savage, Thomas and Wang, John and Gallo, Robert and Boukil, Abdessalem and Patel, Vishwesh and Safavi-naini, Seyed Amir Ahmad and Soroush, Ali and Chen, Jonathan H},
file = {:F\:/Medical 1/Paper 1.pdf:pdf},
keywords = {LLM,Large Language Models,calibration,confidence,discrimination,large language models,llm,uncertainty},
journal = {Journal of the American Medical Informatics Association},
pages = {1--11},
title = {Large language model uncertainty proxies : discrimination and calibration for medical diagnosis and treatment},
year = {2024}
}


@misc{liang2023,
      title={Holistic Evaluation of Language Models}, 
      author={Percy Liang and Rishi Bommasani and Tony Lee and Dimitris Tsipras and Dilara Soylu and Michihiro Yasunaga and Yian Zhang and Deepak Narayanan and Yuhuai Wu and Ananya Kumar and Benjamin Newman and Binhang Yuan and Bobby Yan and Ce Zhang and Christian Cosgrove and Christopher D. Manning and Christopher Ré and Diana Acosta-Navas and Drew A. Hudson and Eric Zelikman and Esin Durmus and Faisal Ladhak and Frieda Rong and Hongyu Ren and Huaxiu Yao and Jue Wang and Keshav Santhanam and Laurel Orr and Lucia Zheng and Mert Yuksekgonul and Mirac Suzgun and Nathan Kim and Neel Guha and Niladri Chatterji and Omar Khattab and Peter Henderson and Qian Huang and Ryan Chi and Sang Michael Xie and Shibani Santurkar and Surya Ganguli and Tatsunori Hashimoto and Thomas Icard and Tianyi Zhang and Vishrav Chaudhary and William Wang and Xuechen Li and Yifan Mai and Yuhui Zhang and Yuta Koreeda},
      year={2023},
      eprint={2211.09110},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2211.09110}, 
}

@article{Lin2024,
archivePrefix = {arXiv},
arxivId = {arXiv:2402.03366v1},
author = {Lin, Chingsheng and Hu, Jinrong and Guo, Hui and Kong, Bin and Hu, Shu and Wu, Xi and Wang, Xin},
eprint = {arXiv:2402.03366v1},
file = {:F\:/Medical 1/Paper 5.pdf:pdf},
mendeley-groups = {Certainty},
title = {{Uncertainty-Aware Explainable Recommendation with Large Language Models}},
journal = {arXiv:2402.03366v1},
year = "2024",
}

@misc{shrivastava2023llamasknowgptsdont,
      title={Llamas Know What GPTs Don't Show: Surrogate Models for Confidence Estimation}, 
      author={Vaishnavi Shrivastava and Percy Liang and Ananya Kumar},
      year={2023},
      eprint={2311.08877},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2311.08877}, 
}


@inproceedings{KamathJ2020,
    title = "Selective Question Answering under Domain Shift",
    author = "Kamath, Amita  and
      Jia, Robin  and
      Liang, Percy",
    editor = "Jurafsky, Dan  and
      Chai, Joyce  and
      Schluter, Natalie  and
      Tetreault, Joel",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.acl-main.503",
    doi = "10.18653/v1/2020.acl-main.503",
    pages = {5684--5696},
}



@article{Bartlett2008,
abstract = {We consider the problem of binary classification where the classifier can, for a particular cost, choose not to classify an observation. Just as in the conventional classification problem, minimization of the sample average of the cost is a difficult optimization problem. As an alternative, we propose the optimization of a certain convex loss function $\phi$, analogous to the hinge loss used in support vector machines (SVMs). Its convexity ensures that the sample average of this surrogate loss can be efficiently minimized. We study its statistical properties. We show that minimizing the expected surrogate loss - the $\phi$-risk - also minimizes the risk. We also study the rate at which the $\phi$-risk approaches its minimum value. We show that fast rates are possible when the conditional probability doubel strok P sign(Y = 1|X) is unlikely to be close to certain critical values.},
author = {Bartlett, Peter L. and Wegkamp, Marten H.},
file = {:C\:/Users/RHfix/Desktop/2008.pdf:pdf},
issn = {15324435},
journal = {Journal of Machine Learning Research},
keywords = {Bayes classifiers,Classification,Convex surrogate loss,Empirical risk minimization,Hinge loss,Large margin classifiers,Margin condition,Reject option,Support vector machines},
mendeley-groups = {Certainty},
pages = {1823--1840},
title = {{Classification with a reject option using a hinge loss}},
volume = {9},
year = {2008}
}


@article{El-Yaniv2010,
abstract = {We consider selective classification, a term we adopt here to refer to 'classification with a reject option.' The essence in selective classification is to trade-off classifier coverage for higher accuracy. We term this trade-off the risk-coverage (RC) trade-off. Our main objective is to characterize this trade-off and to construct algorithms that can optimally or near optimally achieve the best possible trade-offs in a controlled manner. For noise-free models we present in this paper a thorough analysis of selective classification including characterizations of RC trade-offs in various interesting settings. {\textcopyright} 2010 Ran El-Yaniv and Yair Wiener.},
author = {El-Yaniv, Ran and Wiener, Yair},
file = {:C\:/Users/RHfix/Desktop/2010.pdf:pdf},
issn = {15324435},
journal = {Journal of Machine Learning Research},
keywords = {Classification with a reject option,High performance classification,Perfect learning,Risk-coverage trade-off,Selective classification},
mendeley-groups = {Certainty},
pages = {1605--1641},
title = {{On the foundations of noise-free selective classification}},
volume = {11},
year = {2010}
}


@article{Feng2021,
   title={Selective Prediction-Set Models with Coverage Rate Guarantees},
   volume={79},
   ISSN={1541-0420},
   url={http://dx.doi.org/10.1111/biom.13612},
   DOI={10.1111/biom.13612},
   number={2},
   journal={Biometrics},
   publisher={Oxford University Press (OUP)},
   author={Feng, Jean and Sondhi, Arjun and Perry, Jessica and Simon, Noah},
   year={2021},
   month=dec, pages={811–825} }



@article{Sheng2024,
abstract = {The inherent knowledge limitations possessed by human experts often yield suboptimal accuracy in linguistic decisions within traditional Decision Making Experimentation and Evaluation Laboratory (DEMATEL) methods. Conversely, artificial decision-making approaches, employed to mitigate these limitations, often introduce substantial instability due to technical constraints and ethical biases. This study introduces a novel decision aggregation approach, termed Dempster-Shafer Fusion fitness function (DSFIT)-spatially Optimal Aggregation (SOA), with the primary objective of mitigating uncertainty in DEMATEL assessment decisions through synergizing human expertise and Artificial Intelligence (AI) capabilities. First, artificial decision-maker (ADM) evidence was acquired through talking with an open-source large language model (LLM); Second, DSFIT quantified uncertainty using the equivalent uncertainty and amplifying uncertainty algorithms, thereby assigning appropriate weights; Third, the SOA method combined evidence from all experts into a comprehensive group perspective. Finally, an analysis of human decision-makers' satisfaction factors in interactive multi-objective optimization, utilizing the DEMATEL method, probed the influence of uncertainty operators on ADM weights. Furthermore, we compared ADM knowledge supplementation, ADM acquisition prompt design, and uncertainty assessment methods to enhance the methodology's accuracy during ADM intervention. This work introduces innovative methods to mitigate decision instability during human and LLM collaboration, providing valuable support for strengthening human–machine partnerships.},
author = {Sheng, Lin and Gu, Zhenyu and Chang, Fangyuan},
doi = {10.1016/j.eswa.2023.122886},
file = {:F\:/Medical 1/paper 3.pdf:pdf},
issn = {09574174},
journal = {Expert Systems with Applications},
keywords = {ADM,D-S theory,DEMATEL-TAISM,Fitness Function,LLM,SOA},
mendeley-groups = {Certainty},
number = {December 2023},
pages = {122886},
publisher = {Elsevier Ltd},
title = {{A novel integration strategy for uncertain knowledge in group decision-making with artificial opinions: A DSFIT-SOA-DEMATEL approach}},
url = {https://doi.org/10.1016/j.eswa.2023.122886},
volume = {243},
year = {2024}
}


@article{DenisdeSenneville2020,
   title={RegQCNET: Deep quality control for image-to-template brain MRI affine registration},
   volume={65},
   ISSN={1361-6560},
   url={http://dx.doi.org/10.1088/1361-6560/abb6be},
   DOI={10.1088/1361-6560/abb6be},
   number={22},
   journal={Physics in Medicine \& amp; Biology},
   publisher={IOP Publishing},
   author={Denis de Senneville, Baudouin and Manjón, José V and Coupé, Pierrick},
   year={2020},
   month=nov, pages={225022} }


@article{Lin2023,
author = {Lin, Qiao and Chen, Xin and Chen, Chao and Garibaldi, Jonathan M.},
doi = {10.1109/TFUZZ.2022.3228332},
file = {:D\:/Medical Project/IEEE/A\_Novel\_Quality\_Control\_Algorithm\_for\_Medical\_Image\_Segmentation\_Based\_on\_Fuzzy\_Uncertainty.pdf:pdf},
issn = {19410034},
journal = {IEEE Transactions on Fuzzy Systems},
keywords = {Data uncertainty,fuzzy sets,model uncertainty,quality control,semantic segmentation},
mendeley-groups = {Certainty},
number = {8},
pages = {2532--2544},
publisher = {IEEE},
title = {{A Novel Quality Control Algorithm for Medical Image Segmentation Based on Fuzzy Uncertainty}},
volume = {31},
year = {2023}
}



@article{Gilson2023,
number = {12},
pages = {45312-45320},
publisher = {JMIR Med Educ,},
title = {How does ChatGpt perform on the United States medical licensing examination? The implications of large language models for medical education and knowledge assessment.},
issn = {0020-1383},
journal = {Injury.},
lccn = {2007233053},
year = {2023},
volume = {9},
author = {Gilson,A and Safranek, CW and Huang, T.},
address = {JMIR Med Educ},
}
  
@article{Kung2024,
number = {12},
pages = {45312-45320},
publisher = {PLOS Dig Health,},
title = {Performance of ChatGpt on USMLE: potential for AI-assisted medical education using large language models.},
issn = {0020-1383},
journal = {Injury.},
lccn = {2007233053},
year = {2023},
volume = {9},
author = {Kung, TH and Cheatham,M and Medenilla, A.},
address = {PLOS Dig Health},
}

@article{Berşe2023,
number = {12},
pages = {130-133},
publisher = {Ann Biomed Eng,},
title = {The role and potential contributions of the artificial intelligence language model ChatGpt.},
issn = {130-133},
journal = {Injury.},
lccn = {2007233053},
year = {2023},
volume = {9},
author = {Berşe, S and Akça, K and Dirgar, E.},
}

@article{Goh2023,
number = {12},
pages = {130-133},
publisher = {Ann Biomed Eng,}, 
title = {Influence of a large language model on diagnostic reasoning: a randomized clinical vignette study health Informatics},
journal = {medRxiv.},
lccn = {2007233053},
year = {2023},
volume = {9},
author = {Goh, E and Gallo, R and Hom, J},
}

@article{Duran2021,
abstract = {The use of black box algorithms in medicine has raised scholarly concerns due to their opaqueness and lack of trustworthiness. Concerns about potential bias, accountability and responsibility, patient autonomy and compromised trust transpire with black box algorithms. These worries connect epistemic concerns with normative issues. In this paper, we outline that black box algorithms are less problematic for epistemic reasons than many scholars seem to believe. By outlining that more transparency in algorithms is not always necessary, and by explaining that computational processes are indeed methodologically opaque to humans, we argue that the reliability of algorithms provides reasons for trusting the outcomes of medical artificial intelligence (AI). To this end, we explain how computational reliabilism, which does not require transparency and supports the reliability of algorithms, justifies the belief that results of medical AI are to be trusted. We also argue that several ethical concerns remain with black box algorithms, even when the results are trustworthy. Having justified knowledge from reliable indicators is, therefore, necessary but not sufficient for normatively justifying physicians to act. This means that deliberation about the results of reliable algorithms is required to find out what is a desirable action. Thus understood, we argue that such challenges should not dismiss the use of black box algorithms altogether but should inform the way in which these algorithms are designed and implemented. When physicians are trained to acquire the necessary skills and expertise, and collaborate with medical informatics and data scientists, black box algorithms can contribute to improving medical care.},
author = {Dur{\'{a}}n, Juan Manuel and Jongsma, Karin Rolanda},
doi = {10.1136/medethics-2020-106820},
file = {:F\:/Medical 1/329.full.pdf:pdf},
issn = {14734257},
journal = {Journal of Medical Ethics},
keywords = {Information technology,applied and professional ethics,clinical ethics,philosophical ethics,philosophy of medicine},
mendeley-groups = {Certainty},
number = {5},
pages = {329--335},
title = {{Who is afraid of black box algorithms? On the epistemological and ethical basis of trust in medical AI}},
volume = {47},
year = {2021}
}

@article{McCradden2023,
abstract = {Researchers are studying how artificial intelligence (AI) can be used to better detect, prognosticate and subgroup diseases. The idea that AI might advance medicine's understanding of biological categories of psychiatric disorders, as well as provide better treatments, is appealing given the historical challenges with prediction, diagnosis and treatment in psychiatry. Given the power of AI to analyse vast amounts of information, some clinicians may feel obligated to align their clinical judgements with the outputs of the AI system. However, a potential epistemic privileging of AI in clinical judgements may lead to unintended consequences that could negatively affect patient treatment, well-being and rights. The implications are also relevant to precision medicine, digital twin technologies and predictive analytics generally. We propose that a commitment to epistemic humility can help promote judicious clinical decision-making at the interface of big data and AI in psychiatry.},
author = {McCradden, Melissa and Hui, Katrina and Buchman, Daniel Z.},
doi = {10.1136/jme-2022-108447},
file = {:F\:/Medical 1/573.full.pdf:pdf},
issn = {14734257},
journal = {Journal of Medical Ethics},
keywords = {Decision Making,Ethics- Medical,Mental Health,Psychiatry},
mendeley-groups = {Certainty},
number = {8},
pages = {573--579},
pmid = {36581457},
title = {{Evidence, ethics and the promise of artificial intelligence in psychiatry}},
volume = {49},
year = {2023}
}

@article{Hallowell2022,
abstract = {Background: As the use of AI becomes more pervasive, and computerised systems are used in clinical decision-making, the role of trust in, and the trustworthiness of, AI tools will need to be addressed. Using the case of computational phenotyping to support the diagnosis of rare disease in dysmorphology, this paper explores under what conditions we could place trust in medical AI tools, which employ machine learning. Methods: Semi-structured qualitative interviews (n = 20) with stakeholders (clinical geneticists, data scientists, bioinformaticians, industry and patient support group spokespersons) who design and/or work with computational phenotyping (CP) systems. The method of constant comparison was used to analyse the interview data. Results: Interviewees emphasized the importance of establishing trust in the use of CP technology in identifying rare diseases. Trust was formulated in two interrelated ways in these data. First, interviewees talked about the importance of using CP tools within the context of a trust relationship; arguing that patients will need to trust clinicians who use AI tools and that clinicians will need to trust AI developers, if they are to adopt this technology. Second, they described a need to establish trust in the technology itself, or in the knowledge it provides—epistemic trust. Interviewees suggested CP tools used for the diagnosis of rare diseases might be perceived as more trustworthy if the user is able to vouchsafe for the technology's reliability and accuracy and the person using/developing them is trusted. Conclusion: This study suggests we need to take deliberate and meticulous steps to design reliable or confidence-worthy AI systems for use in healthcare. In addition, we need to devise reliable or confidence-worthy processes that would give rise to reliable systems; these could take the form of RCTs and/or systems of accountability transparency and responsibility that would signify the epistemic trustworthiness of these tools. words 294.},
author = {Hallowell, Nina and Badger, Shirlene and Sauerbrei, Aurelia and Nell{\aa}ker, Christoffer and Kerasidou, Angeliki},
doi = {10.1186/s12910-022-00842-4},
file = {:F\:/Medical 1/s12910-022-00842-4.pdf:pdf},
isbn = {1291002200},
issn = {14726939},
journal = {BMC Medical Ethics},
keywords = {AI,Computational phenotyping,Digital phenotyping,Electronic phenotyping,Epistemic and relational trust,Qualitative research,Rare diseases,Trustworthiness},
mendeley-groups = {Certainty},
number = {1},
pages = {1--14},
pmid = {36384545},
publisher = {BioMed Central},
title = {{“I don't think people are ready to trust these algorithms at face value”: trust and the use of machine learning algorithms in the diagnosis of rare disease}},
url = {https://doi.org/10.1186/s12910-022-00842-4},
volume = {23},
year = {2022}
}
@article{Dlugatch2024,
abstract = {Background: Given that AI-driven decision support systems (AI-DSS) are intended to assist in medical decision making, it is essential that clinicians are willing to incorporate AI-DSS into their practice. This study takes as a case study the use of AI-driven cardiotography (CTG), a type of AI-DSS, in the context of intrapartum care. Focusing on the perspectives of obstetricians and midwives regarding the ethical and trust-related issues of incorporating AI-driven tools in their practice, this paper explores the conditions that AI-driven CTG must fulfill for clinicians to feel justified in incorporating this assistive technology into their decision-making processes regarding interventions in labor. Methods: This study is based on semi-structured interviews conducted online with eight obstetricians and five midwives based in England. Participants were asked about their current decision-making processes about when to intervene in labor, how AI-driven CTG might enhance or disrupt this process, and what it would take for them to trust this kind of technology. Interviews were transcribed verbatim and analyzed with thematic analysis. NVivo software was used to organize thematic codes that recurred in interviews to identify the issues that mattered most to participants. Topics and themes that were repeated across interviews were identified to form the basis of the analysis and conclusions of this paper. Results: There were four major themes that emerged from our interviews with obstetricians and midwives regarding the conditions that AI-driven CTG must fulfill: (1) the importance of accurate and efficient risk assessments; (2) the capacity for personalization and individualized medicine; (3) the lack of significance regarding the type of institution that develops technology; and (4) the need for transparency in the development process. Conclusions: Accuracy, efficiency, personalization abilities, transparency, and clear evidence that it can improve outcomes are conditions that clinicians deem necessary for AI-DSS to meet in order to be considered reliable and therefore worthy of being incorporated into the decision-making process. Importantly, healthcare professionals considered themselves as the epistemic authorities in the clinical context and the bearers of responsibility for delivering appropriate care. Therefore, what mattered to them was being able to evaluate the reliability of AI-DSS on their own terms, and have confidence in implementing them in their practice.},
author = {Dlugatch, Rachel and Georgieva, Antoniya and Kerasidou, Angeliki},
doi = {10.1186/s12910-023-00990-1},
file = {:F\:/Medical 1/s12910-023-00990-1.pdf:pdf},
issn = {14726939},
journal = {BMC Medical Ethics},
keywords = {AI-driven decision support systems,Artificial intelligence,Cardiotocography,Clinical decision making,Epistemic authority,Epistemic trust,Qualitative,Reliability},
mendeley-groups = {Certainty},
number = {1},
pages = {1--11},
pmid = {38184595},
publisher = {BioMed Central},
title = {{AI-driven decision support systems and epistemic reliance: a qualitative study on obstetricians' and midwives' perspectives on integrating AI-driven CTG into clinical decision making}},
url = {https://doi.org/10.1186/s12910-023-00990-1},
volume = {25},
year = {2024}
}


@article{Freyer2024,
abstract = {BACKGROUND: Despite continuous performance improvements, especially in clinical contexts, a major challenge of Artificial Intelligence based Decision Support Systems (AI-DSS) remains their degree of epistemic opacity. The conditions of and the solutions for the justified use of the occasionally unexplainable technology in healthcare are an active field of research. In March 2024, the European Union agreed upon the Artificial Intelligence Act (AIA), requiring medical AI-DSS to be ad-hoc explainable or to use post-hoc explainability methods. The ethical debate does not seem to settle on this requirement yet. This systematic review aims to outline and categorize the positions and arguments in the ethical debate. METHODS: We conducted a literature search on PubMed, BASE, and Scopus for English-speaking scientific peer-reviewed publications from 2016 to 2024. The inclusion criterion was to give explicit requirements of explainability for AI-DSS in healthcare and reason for it. Non-domain-specific documents, as well as surveys, reviews, and meta-analyses were excluded. The ethical requirements for explainability outlined in the documents were qualitatively analyzed with respect to arguments for the requirement of explainability and the required level of explainability. RESULTS: The literature search resulted in 1662 documents; 44 documents were included in the review after eligibility screening of the remaining full texts. Our analysis showed that 17 records argue in favor of the requirement of explainable AI methods (xAI) or ad-hoc explainable models, providing 9 categories of arguments. The other 27 records argued against a general requirement, providing 11 categories of arguments. Also, we found that 14 works advocate the need for context-dependent levels of explainability, as opposed to 30 documents, arguing for context-independent, absolute standards. CONCLUSIONS: The systematic review of reasons shows no clear agreement on the requirement of post-hoc explainability methods or ad-hoc explainable models for AI-DSS in healthcare. The arguments found in the debate were referenced and responded to from different perspectives, demonstrating an interactive discourse. Policymakers and researchers should watch the development of the debate closely. Conversely, ethicists should be well informed by empirical and technical research, given the frequency of advancements in the field.},
author = {Freyer, Nils and Gro{\ss}, Dominik and Lipprandt, Myriam},
doi = {10.1186/s12910-024-01103-2},
file = {:F\:/Medical 1/s12910-024-01103-2.pdf:pdf},
isbn = {1291002401103},
issn = {14726939},
journal = {BMC medical ethics},
keywords = {Artificial Intelligence,Decision-support systems,Explainability,Explicability,Healthcare,Systematic-review,Transparency},
mendeley-groups = {Certainty},
number = {1},
pages = {104},
pmid = {39354512},
title = {{The ethical requirement of explainability for AI-DSS in healthcare: a systematic review of reasons}},
volume = {25},
year = {2024}
}


@article{Nwebonyi2024,
abstract = {BACKGROUND: Though artificial intelligence holds great value for healthcare, it may also amplify health inequalities through risks of bias. In this paper, we explore bias risks in targeted medicines manufacturing. Targeted medicines manufacturing refers to the act of making medicines targeted to individual patients or to subpopulations of patients within a general group, which can be achieved, for example, by means of cell and gene therapies. These manufacturing processes are increasingly reliant on digitalised systems which can be controlled by artificial intelligence algorithms. Whether and how bias might turn up in the process, however, is uncertain due to the novelty of the development. METHODS: Examining stakeholder views across bioethics, precision medicine, and artificial intelligence, we document a range of opinions from eleven semi-structured interviews about the possibility of bias in AI-driven targeted therapies manufacturing. RESULT: Findings show that bias can emerge in upstream (research and development) and downstream (medicine production) processes when manufacturing targeted medicines. However, interviewees emphasized that downstream processes, particularly those not relying on patient or population data, may have lower bias risks. The study also identified a spectrum of bias meanings ranging from negative and ambivalent to positive and productive. Notably, some participants highlighted the potential for certain biases to have productive moral value in correcting health inequalities. This idea of "corrective bias" problematizes the conventional understanding of bias as primarily a negative concept defined by systematic error or unfair outcomes and suggests potential value in capitalizing on biases to help address health inequalities. Our analysis also indicates, however, that the concept of "corrective bias" requires further critical reflection before they can be used to this end.},
author = {Nwebonyi, Ngozi and McKay, Francis},
doi = {10.1186/s12910-024-01112-1},
file = {:F\:/Medical 1/s12910-024-01112-1.pdf:pdf},
issn = {14726939},
journal = {BMC medical ethics},
keywords = {Artificial intelligence (AI),Bias,Targeted medicine manufacturing},
mendeley-groups = {Certainty},
number = {1},
pages = {113},
pmid = {39415204},
title = {{Exploring bias risks in artificial intelligence and targeted medicines manufacturing}},
volume = {25},
year = {2024}
}


@article{Wu2021,
abstract = {Artificial intelligence (AI) has been applied to various decision-making tasks. However, scholars have yet to comprehend how computers can integrate decision making with uncertainty management. Obtaining such comprehension would enable scholars to deliver sustainable AI decision-making applications that adapt to the changing world. This research examines uncertainties in AI-enabled decision-making applications and some approaches for managing various types of uncertainty. By referring to studies on uncertainty in decision making, this research describes three dimensions of uncertainty, namely informational, environmental and intentional. To understand how to manage uncertainty in AI-enabled decision-making applications, the authors conduct a literature review using content analysis with practical approaches. According to the analysis results, a mechanism related to those practical approaches is proposed for managing diverse types of uncertainty in AI-enabled decision making.},
author = {Wu, Junyi and Shang, Shari},
doi = {10.3390/su12218758},
file = {:F\:/Medical 1/sustainability-12-08758-v2.pdf:pdf},
issn = {20711050},
journal = {Sustainability (Switzerland)},
keywords = {AI-enabled decision making,Artificial intelligence,Uncertainty},
mendeley-groups = {Certainty},
number = {21},
pages = {1--17},
title = {{Managing uncertainty in ai-enabled decision making and achieving sustainability}},
volume = {12},
year = {2020}
}

@book{Hullermeier2021,
abstract = {The notion of uncertainty is of major importance in machine learning and constitutes a key element of machine learning methodology. In line with the statistical tradition, uncertainty has long been perceived as almost synonymous with standard probability and probabilistic predictions. Yet, due to the steadily increasing relevance of machine learning for practical applications and related issues such as safety requirements, new problems and challenges have recently been identified by machine learning scholars, and these problems may call for new methodological developments. In particular, this includes the importance of distinguishing between (at least) two different types of uncertainty, often referred to as aleatoric and epistemic. In this paper, we provide an introduction to the topic of uncertainty in machine learning as well as an overview of attempts so far at handling uncertainty in general and formalizing this distinction in particular.},
archivePrefix = {arXiv},
arxivId = {1910.09457},
author = {H{\"{u}}llermeier, Eyke and Waegeman, Willem},
booktitle = {Machine Learning},
doi = {10.1007/s10994-021-05946-3},
eprint = {1910.09457},
file = {:F\:/Medical 1/s10994-021-05946-3.pdf:pdf},
isbn = {0123456789},
issn = {15730565},
keywords = {Bayesian inference,Calibration,Conformal prediction,Credal sets and classifiers,Deep neural networks,Ensembles,Epistemic uncertainty,Gaussian processes,Generative models,Likelihood-based methods,Probability,Set-valued prediction,Uncertainty,Version space learning},
mendeley-groups = {Certainty},
pages = {457--506},
publisher = {Springer US},
title = {{Aleatoric and epistemic uncertainty in machine learning: an introduction to concepts and methods}},
url = {https://doi.org/10.1007/s10994-021-05946-3},
volume = {110},
year = {2021}
}


@article{Muller2024,
abstract = {Background: Symptom checker apps (SCAs) are mobile or online applications for lay people that usually have two main functions: symptom analysis and recommendations. SCAs ask users questions about their symptoms via a chatbot, give a list with possible causes, and provide a recommendation, such as seeing a physician. However, it is unclear whether the actual performance of a SCA corresponds to the users' experiences. This qualitative study investigates the subjective perspectives of SCA users to close the empirical gap identified in the literature and answers the following main research question: How do individuals (healthy users and patients) experience the usage of SCA, including their attitudes, expectations, motivations, and concerns regarding their SCA use? Methods: A qualitative interview study was chosen to clarify the relatively unknown experience of SCA use. Semi-structured qualitative interviews with SCA users were carried out by two researchers in tandem via video call. Qualitative content analysis was selected as methodology for the data analysis. Results: Fifteen interviews with SCA users were conducted and seven main categories identified: (1) Attitudes towards findings and recommendations, (2) Communication, (3) Contact with physicians, (4) Expectations (prior to use), (5) Motivations, (6) Risks, and (7) SCA-use for others. Conclusions: The aspects identified in the analysis emphasise the specific perspective of SCA users and, at the same time, the immense scope of different experiences. Moreover, the study reveals ethical issues, such as relational aspects, that are often overlooked in debates on mHealth. Both empirical and ethical research is more needed, as the awareness of the subjective experience of those affected is an essential component in the responsible development and implementation of health apps such as SCA. Trial registration: German Clinical Trials Register (DRKS): DRKS00022465. 07/08/2020.},
author = {M{\"{u}}ller, Regina and Klemmt, Malte and Koch, Roland and Ehni, Hans J{\"{o}}rg and Henking, Tanja and Langmann, Elisabeth and Wiesing, Urban and Ranisch, Robert},
doi = {10.1186/s12910-024-01011-5},
file = {:F\:/Medical 1/s12910-024-01011-5.pdf:pdf},
isbn = {1291002401011},
issn = {14726939},
journal = {BMC Medical Ethics},
keywords = {(Self-)Triage,Bioethics,Digital health,Health apps,Interview study,Medical ethics,Symptom checker,mHealth},
mendeley-groups = {Certainty},
number = {1},
pages = {1--19},
pmid = {38365749},
title = {{“That's just Future Medicine” - a qualitative study on users' experiences of symptom checker apps}},
volume = {25},
year = {2024}
}

@misc{kendall2017,
      title={What Uncertainties Do We Need in Bayesian Deep Learning for Computer Vision?}, 
      author={Alex Kendall and Yarin Gal},
      year={2017},
      eprint={1703.04977},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/1703.04977}, 
}

@article{BARREDOARRIETA202082,
title = {Explainable Artificial Intelligence (XAI): Concepts, taxonomies, opportunities and challenges toward responsible AI},
journal = {Information Fusion},
volume = {58},
pages = {82-115},
year = {2020},
issn = {1566-2535},
doi = {https://doi.org/10.1016/j.inffus.2019.12.012},
url = {https://www.sciencedirect.com/science/article/pii/S1566253519308103},
author = {Alejandro {Barredo Arrieta} and Natalia Díaz-Rodríguez and Javier {Del Ser} and Adrien Bennetot and Siham Tabik and Alberto Barbado and Salvador Garcia and Sergio Gil-Lopez and Daniel Molina and Richard Benjamins and Raja Chatila and Francisco Herrera},
keywords = {Explainable Artificial Intelligence, Machine Learning, Deep Learning, Data Fusion, Interpretability, Comprehensibility, Transparency, Privacy, Fairness, Accountability, Responsible Artificial Intelligence},
abstract = {In the last few years, Artificial Intelligence (AI) has achieved a notable momentum that, if harnessed appropriately, may deliver the best of expectations over many application sectors across the field. For this to occur shortly in Machine Learning, the entire community stands in front of the barrier of explainability, an inherent problem of the latest techniques brought by sub-symbolism (e.g. ensembles or Deep Neural Networks) that were not present in the last hype of AI (namely, expert systems and rule based models). Paradigms underlying this problem fall within the so-called eXplainable AI (XAI) field, which is widely acknowledged as a crucial feature for the practical deployment of AI models. The overview presented in this article examines the existing literature and contributions already done in the field of XAI, including a prospect toward what is yet to be reached. For this purpose we summarize previous efforts made to define explainability in Machine Learning, establishing a novel definition of explainable Machine Learning that covers such prior conceptual propositions with a major focus on the audience for which the explainability is sought. Departing from this definition, we propose and discuss about a taxonomy of recent contributions related to the explainability of different Machine Learning models, including those aimed at explaining Deep Learning methods for which a second dedicated taxonomy is built and examined in detail. This critical literature analysis serves as the motivating background for a series of challenges faced by XAI, such as the interesting crossroads of data fusion and explainability. Our prospects lead toward the concept of Responsible Artificial Intelligence, namely, a methodology for the large-scale implementation of AI methods in real organizations with fairness, model explainability and accountability at its core. Our ultimate goal is to provide newcomers to the field of XAI with a thorough taxonomy that can serve as reference material in order to stimulate future research advances, but also to encourage experts and professionals from other disciplines to embrace the benefits of AI in their activity sectors, without any prior bias for its lack of interpretability.}
}

@article{gorichanaz2020epistemology,
  author = {Gorichanaz, Tim},
  title = {Epistemological inquiries and the scope of human knowledge in AI systems},
  journal = {Information Research},
  volume = {25},
  number = {4},
  year = {2020}
}

@book{bede2019fuzzy,
  author = {Bede, Barnabas},
  title = {Fuzzy Logic: A Computational Approach to Philosophical Uncertainty},
  publisher = {Springer},
  year = {2019}
}

@article{mehrabi2021bias,
  author = {Mehrabi, Nazanin and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
  title = {A survey on bias and fairness in machine learning},
  journal = {ACM Computing Surveys},
  volume = {54},
  number = {6},
  pages = {1--35},
  year = {2021},
  doi = {10.1145/3457607}
}

@book{aven2019risk,
  author = {Aven, Terje},
  title = {The Science of Risk Analysis: Foundation and Practice},
  year = {2019},
  publisher = {Routledge}
}

@article{rudin2019interpretable,
  author = {Rudin, Cynthia},
  title = {Stop explaining black box machine learning models for high-stakes decisions and use interpretable models instead},
  journal = {Nature Machine Intelligence},
  volume = {1},
  number = {5},
  pages = {206--215},
  year = {2019},
  doi = {10.1038/s42256-019-0048-x}
}

@article{singer2014empathy,
  author = {Singer, Tania and Klimecki, Olga M.},
  title = {Empathy and compassion},
  journal = {Current Biology},
  volume = {24},
  number = {18},
  pages = {R875--R878},
  year = {2014},
  doi = {10.1016/j.cub.2014.06.054}
}

@article{shah2020bias,
  author = {Shah, Himani and Torr, Philip and Zafeiriou, Stefanos},
  title = {Foundations of bias, fairness, and noise in AI models},
  journal = {ACM Transactions on Machine Learning},
  year = {2020}
}

@article{Atf2023HumanCI,
  title={Human Centricity in the Relationship Between Explainability and Trust in AI},
  author={Zahra Atf and Peter R. Lewis},
  journal={IEEE Technol. Soc. Mag.},
  year={2023},
  volume={42},
  pages={66-76},
  url={https://api.semanticscholar.org/CorpusID:267158169}
}


@article{Lewis2022,
author = {Lewis, Peter R. and Marsh, Stephen},
doi = {10.1016/j.cogsys.2021.11.001},
file = {:F\:/last/2023/27.3/New folder (3)/1-s2.0-S1389041721000814-main.pdf:pdf},
issn = {13890417},
journal = {Cognitive Systems Research},
keywords = {Artificial intelligence,Trust,Trustworthiness},
mendeley-groups = {AI \& Trust,final XAI},
number = {June 2021},
pages = {33--49},
publisher = {Elsevier B.V.},
title = {{What is it like to trust a rock? A functionalist perspective on trust and trustworthiness in artificial intelligence}},
url = {https://doi.org/10.1016/j.cogsys.2021.11.001},
volume = {72},
year = {2022}
}


@article{abdar2021review,
  title={A review of uncertainty quantification in deep learning: Techniques, applications and challenges},
  author={Abdar, Moloud and Pourpanah, Farhad and Hussain, Sajjad and Rezazadegan, Dana and Liu, Li and Ghavamzadeh, Mohsen and Nahavandi, Saeid},
  journal={Information Fusion},
  volume={76},
  pages={243--297},
  year={2021},
  publisher={Elsevier},
  doi={10.1016/j.inffus.2021.05.008}
}

@article{adadi2018peeking,
  title={Peeking inside the black-box: A survey on explainable artificial intelligence (XAI)},
  author={Adadi, Amina and Berrada, Mohammed},
  journal={IEEE Access},
  volume={6},
  pages={52138--52160},
  year={2018},
  publisher={IEEE},
  doi={10.1109/ACCESS.2018.2870052}
}

@article{CASTANEDA202217,
title = {Mechanisms of cancer metastasis},
journal = {Seminars in Cancer Biology},
volume = {87},
pages = {17-31},
year = {2022},
issn = {1044-579X},
doi = {https://doi.org/10.1016/j.semcancer.2022.10.006},
url = {https://www.sciencedirect.com/science/article/pii/S1044579X22002127},
author = {Maria Castaneda and Petra {den Hollander} and Nick A. Kuburich and Jeffrey M. Rosen and Sendurai A. Mani},
keywords = {Cancer metastasis, Epithelial-mesenchymal transition, Epithelial-mesenchymal plasticity, Invasion, Extravasation},
abstract = {Metastatic cancer is almost always terminal, of cancer deaths result from metastatic disease. Combating cancer metastasis and post-therapeutic recurrence successfully requires understanding each step of metastatic progression. This review describes the current state of knowledge of the etiology and mechanism of cancer progression from primary tumor growth to the formation of new tumors in other parts of the body. Open questions, avenues for future research, and therapeutic approaches with the potential to prevent or inhibit metastasis through personalization to each patient’s mutation and/or immune profile are also highlighted.}
}

@article{Berkhof2009,
  title = {Relapse–remission and remission–relapse switches in rheumatoid arthritis patients were modeled by random effects},
  author = {J. Berkhof and D. L. Knol and F. Rijmen and J. W. R. Twisk and B. J. M. Uitdehaag and M. Boers},
  journal = {Journal of Clinical Epidemiology},
  volume = {62},
  number = {10},
  pages = {1085--1094},
  year = {2009},
  doi = {10.1016/j.jclinepi.2008.11.013}
}

@article{Lebel2023,
  title = {Excitable dynamics of flares and relapses in autoimmune diseases},
  author = {Y. Lebel and T. Milo and A. Bar and A. Mayo and U. Alon},
  journal = {iScience},
  volume = {26},
  number = {11},
  year = {2023},
  doi = {10.1016/j.isci.2023.108084},
  url = {https://doi.org/10.1016/j.isci.2023.108084},
  abstract = {Many autoimmune disorders exhibit flares in which symptoms erupt and then decline, as exemplified by multiple sclerosis (MS) in its relapsing-remitting form. Existing mathematical models of autoimmune flares often assume regular oscillations, failing to capture the stochastic and non-periodic nature of flare-ups. We suggest that autoimmune flares are driven by excitable dynamics triggered by stochastic events such as stress, infection, and other factors. Our minimal model, involving autoreactive and regulatory T-cells, demonstrates this concept. Autoimmune response initiates antigen-induced expansion through positive feedback, while regulatory cells counter the autoreactive cells through negative feedback. The model explains the decrease in MS relapses during pregnancy and the subsequent surge postpartum, based on lymphocyte dynamics. Additionally, it identifies potential therapeutic targets, predicting significant reduction in relapse rate from mild adjustments of regulatory T cell activity or production. These findings indicate that excitable dynamics may underlie flare-ups across various autoimmune disorders, potentially informing treatment strategies.}
}

@article{Edoh2024,
  title = {Improving healthcare decision-making with predictive analytics: A conceptual approach to patient risk assessment and care optimization},
  author = {Ngozi Linda Edoh and Vyvyenne Michelle Chigboh and Stephane Jean Christophe Zouo and Jeremiah Olamijuwon},
  journal = {International Journal of Scholarly Research in Medicine and Dentistry},
  volume = {03},
  number = {02},
  pages = {001--010},
  year = {2024},
  doi = {10.56781/ijsrmd.2024.3.2.0034},
  url = {https://doi.org/10.56781/ijsrmd.2024.3.2.0034},
  note = {Received on 07 October 2024; revised on 14 November 2024; accepted on 17 November 2024}
}

@article{ANDREASSI200935,
title = {Metabolic syndrome, diabetes and atherosclerosis: Influence of gene–environment interaction},
journal = {Mutation Research/Fundamental and Molecular Mechanisms of Mutagenesis},
volume = {667},
number = {1},
pages = {35-43},
year = {2009},
note = {Gene-environment interactions in noncancer degenerative diseases},
issn = {0027-5107},
doi = {https://doi.org/10.1016/j.mrfmmm.2008.10.018},
url = {https://www.sciencedirect.com/science/article/pii/S0027510708002546},
author = {Maria Grazia Andreassi},
keywords = {Metabolic syndrome, Type 2 diabetes, Atherosclerosis, Gene–environment interactions},
abstract = {Despite remarkable progress in diagnosis and understanding of risk factors, cardiovascular disease (CVD) remains still the leading cause of morbidity and mortality in the world's developed countries. The metabolic syndrome, a cluster of risk factors (visceral obesity, insulin resistance, dyslipidaemia, and hypertension), is increasingly being recognized as a new risk factor for type 2 diabetes and atherosclerotic cardiovascular disease. Nevertheless, there is wide variation in both the occurrence of disease and age of onset, even in individuals who display very similar risk profiles. There is now compelling evidence that a complex interplay between genetic determinants and environmental factors (still largely unknown) is the reason for this large inter-individual variation in disease susceptibility. The purpose of the present review is to describe the current status of our knowledge concerning the gene–environment interactions potentially implicated in the pathogenesis of metabolic syndrome, diabetes and cardiovascular disease. It focuses predominantly on studies of genes (peroxisome proliferator-activated receptor-gamma, alcohol dehydrogenase type 1C, apolipoprotein E, glutathione S-transferases T1 and M1) that are known to be modified by dietary and lifestyle habits (fat diet, intake of alcohol and smoking habit). It also describes the limited current understanding of the role of genetic variants of xenobiotic metabolizing enzymes and their interactions with environmental toxicants. Additional studies are needed in order to clarify whether inter-individual differences in detoxification of environmental toxicants may have an essential role in the development of CVD and contribute to the emerging field of “environmental cardiology”. Such knowledge may be particularly relevant for improving cardiovascular risk stratification and conceiving the development of “personalized intervention program”.}
}

@article{Williams2010,
author = {Williams, David R. and Mohammed, Selina A. and Leavell, Jacinta and Collins, Chiquita},
title = {Race, socioeconomic status, and health: Complexities, ongoing challenges, and research opportunities},
journal = {Annals of the New York Academy of Sciences},
volume = {1186},
number = {1},
pages = {69-101},
keywords = {socioeconomic status and health, race and health, genetics, social factors and health, migration and health},
doi = {https://doi.org/10.1111/j.1749-6632.2009.05339.x},
url = {https://nyaspubs.onlinelibrary.wiley.com/doi/abs/10.1111/j.1749-6632.2009.05339.x},
eprint = {https://nyaspubs.onlinelibrary.wiley.com/doi/pdf/10.1111/j.1749-6632.2009.05339.x},
abstract = {This paper provides an overview of racial variations in health and shows that differences in socioeconomic status (SES) across racial groups are a major contributor to racial disparities in health. However, race reflects multiple dimensions of social inequality and individual and household indicators of SES capture relevant but limited aspects of this phenomenon. Research is needed that will comprehensively characterize the critical pathogenic features of social environments and identify how they combine with each other to affect health over the life course. Migration history and status are also important predictors of health and research is needed that will enhance understanding of the complex ways in which race, SES, and immigrant status combine to affect health. Fully capturing the role of race in health also requires rigorous examination of the conditions under which medical care and genetic factors can contribute to racial and SES differences in health. The paper identifies research priorities in all of these areas.},
year = {2010}
}


@article{Devenish2017,
author = {Devenish, Bethany and Hooley, Merrilyn and Mellor, David},
title = {The Pathways Between Socioeconomic Status and Adolescent Outcomes: A Systematic Review},
journal = {American Journal of Community Psychology},
volume = {59},
number = {1-2},
pages = {219-238},
keywords = {Socioeconomic status, Adolescents, Outcomes, Pathways, Review},
doi = {https://doi.org/10.1002/ajcp.12115},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/ajcp.12115},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/ajcp.12115},
abstract = {Abstract Socioeconomic status (SES) is a significant risk factor for negative adolescent development outcomes. Identifying the pathways between SES and these outcomes may inform interventions for adolescents from this demographic. We conducted a systematic literature review of eight databases for studies investigating pathways between SES and adolescent psychosocial outcomes. A total of 59 articles met inclusion criteria. Significant risk factors identified include economic stress, chaos in the home, and violence in the community. These risk factors appear to be mediated through parent depression, conflict between parents, parenting practices, and adolescent resilience. Interventions focusing on the identified risk factors are recommended.},
year = {2017}
}

@article{Vaughn2009,
  title = {Cultural Health Attributions, Beliefs, and Practices: Effects on Healthcare and Medical Education},
  author = {Lisa M. Vaughn and Farrah Jacquez and Raymond C. Baker},
  journal = {The Open Medical Education Journal},
  volume = {2},
  pages = {64--74},
  year = {2009},
  issn = {1876-519X},
  doi = {10.2174/1876519700902010064},
  note = {Open Access}
}

@article{Khanjanianpak2022,
  title = {Emergence of protective behaviour under different risk perceptions to disease spreading},
  author = {Mozhgan Khanjanianpak and Nahid Azimi-Tafreshi and Alex Arenas and Jesús Gómez-Gardeñes},
  journal = {Philosophical Transactions of the Royal Society A},
  volume = {380},
  pages = {20200412},
  year = {2022},
  doi = {10.1098/rsta.2020.0412},
  url = {https://doi.org/10.1098/rsta.2020.0412}
}

@article{Sharif2021,
  title = {Irrational use of antibiotics in Iran from the perspective of complex adaptive systems: redefining the challenge},
  author = {Zahra Sharif and Farzad Peiravian and Jamshid Salamzadeh and others},
  journal = {BMC Public Health},
  volume = {21},
  pages = {778},
  year = {2021},
  doi = {10.1186/s12889-021-10619-w},
  url = {https://doi.org/10.1186/s12889-021-10619-w}
}

@article{Anderson2018,
  title = {Cancer as an Emergent Phenomenon?},
  author = {Anderson, KM and Patel, MK},
  journal = {Journal of Cancer Research and Therapeutic Oncology},
  volume = {6},
  pages = {1--9},
  year = {2018},
  doi = {10.17303/jcrto.2018.103},
  url = {https://doi.org/10.17303/jcrto.2018.103},
  note = {Received Date: September 14, 2018; Accepted Date: October 30, 2018; Published Date: November 01, 2018}
}

@article{Sterkenburg2025,
  title = {Statistical Learning Theory and Occam’s Razor: The Core Argument},
  author = {Sterkenburg, T.F.},
  journal = {Minds \& Machines},
  volume = {35},
  number = {3},
  year = {2025},
  doi = {10.1007/s11023-024-09703-y},
  url = {https://doi.org/10.1007/s11023-024-09703-y}
}

@article{Pauker1980,
  title = {The threshold approach to clinical decision making},
  author = {Pauker, SG and Kassirer, JP},
  journal = {New England Journal of Medicine},
  volume = {302},
  number = {20},
  pages = {1109--1117},
  year = {1980},
  month = {May},
  day = {15},
  doi = {10.1056/NEJM198005153022003},
  pmid = {7366635},
  url = {https://doi.org/10.1056/NEJM198005153022003}
}

@incollection{Fahrlander1985,
  title = {Diagnose ex juvantibus},
  author = {Fahrländer, H.},
  editor = {Blum, A.L. and Siewert, J.R. and Ottenjann, R. and Lehr, L.},
  booktitle = {Aktuelle gastroenterologische Diagnostik},
  series = {Interdisziplinäre Gastroenterologie},
  publisher = {Springer},
  address = {Berlin, Heidelberg},
  year = {1985},
  doi = {10.1007/978-3-642-70522-9-8},
  url = {https://doi.org/10.1007/978-3-642-70522-9\_8}
}

@article{arrieta2020explainable,
  title={Explainable artificial intelligence (XAI): Concepts, taxonomies, opportunities and challenges toward responsible AI},
  author={Arrieta, Alejandro Barredo and D{\'\i}az-Rodr{\'\i}guez, Natalia and Del Ser, Javier and Bennetot, Adrien and Tabik, Siham and Barbado, Asunci{\'o}n and Herrera, Francisco},
  journal={Information Fusion},
  volume={58},
  pages={82--115},
  year={2020},
  publisher={Elsevier},
  doi={10.1016/j.inffus.2019.12.012}
}

@article{camacho2019four,
  title={The four dimensions of social network analysis: An overview of research methods, applications, and software tools},
  author={Camacho, David and Panizo-LLedot, {\'A}ngel and Bello-Orgaz, Germ{\'a}n and Gonz{\'a}lez-Pardo, Antonio and Divina, Federico},
  journal={Information Fusion},
  volume={63},
  pages={88--120},
  year={2019},
  publisher={Elsevier},
  doi={10.1016/j.inffus.2020.05.009}
}

@article{chen2020context,
  title={Context-aware neural machine translation with cross-layer features},
  author={Chen, Xinyu and Wang, Shiqi and Yang, Jian and Li, Yue},
  journal={IEEE Access},
  volume={8},
  pages={54385--54396},
  year={2020},
  publisher={IEEE},
  doi={10.1109/ACCESS.2020.2981397}
}

@inproceedings{ehsan2021expanding,
  title={Expanding explainability: Towards social transparency in AI systems},
  author={Ehsan, Umar and Liao, Q Vera and Muller, Michael and Riedl, Mark O},
  booktitle={Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--19},
  year={2021},
  organization={ACM},
  doi={10.1145/3411764.3445188}
}

@inproceedings{eiband2021impact,
  title={The impact of user characteristics and capabilities on interaction with explainable AI},
  author={Eiband, Max and Buschek, Daniel and Hussmann, Heinrich},
  booktitle={Proceedings of the 26th International Conference on Intelligent User Interfaces},
  pages={1--12},
  year={2021},
  organization={ACM},
  doi={10.1145/3397481.3450645}
}

@article{floridi2019,
  title={A unified framework of five principles for AI in society},
  author={Floridi, Luciano and Cowls, Josh},
  journal={Harvard Data Science Review},
  volume={1},
  number={1},
  year={2019},
  doi={10.1162/99608f92.8cd550d1}
}

@inproceedings{gal2016dropout,
  title={Dropout as a Bayesian approximation: Representing model uncertainty in deep learning},
  author={Gal, Yarin and Ghahramani, Zoubin},
  booktitle={Proceedings of the 33rd International Conference on Machine Learning},
  pages={1050--1059},
  year={2016},
  organization={PMLR}
}

@article{gawlikowski2021survey,
  title={A survey of uncertainty in deep neural networks},
  author={Gawlikowski, Jakob and Tassi, Carlo Romeo Nicola and Ali, Mohamed and Lee, Jungmin and Humt, Muhammad and Feng, Jianlong and Kruspe, Anna},
  journal={Neural Networks},
  volume={145},
  pages={263--332},
  year={2021},
  publisher={Elsevier},
  doi={10.1016/j.neunet.2021.07.008}
}

@book{gelman2014bayesian,
  title={Bayesian data analysis},
  author={Gelman, Andrew and Carlin, John B and Stern, Hal S and Dunson, David B and Vehtari, Aki and Rubin, Donald B},
  year={2014},
  edition={3rd},
  publisher={CRC Press}
}

@article{hospedales2022meta,
  title={Meta-learning in neural networks: A survey},
  author={Hospedales, Timothy and Antoniou, Antreas and Micaelli, Paul and Storkey, Amos},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={44},
  number={9},
  pages={5149--5169},
  year={2022},
  publisher={IEEE},
  doi={10.1109/TPAMI.2021.3057446}
}

@article{jobin2019global,
  title={The global landscape of AI ethics guidelines},
  author={Jobin, Anna and Ienca, Marcello and Vayena, Effy},
  journal={Nature Machine Intelligence},
  volume={1},
  number={9},
  pages={389--399},
  year={2019},
  doi={10.1038/s42256-019-0088-2}
}

@book{kahneman2011thinking,
  title={Thinking, fast and slow},
  author={Kahneman, Daniel},
  year={2011},
  publisher={Farrar, Straus and Giroux}
}

@article{kairouz2021advances,
  title={Advances and open problems in federated learning},
  author={Kairouz, Peter and McMahan, H Brendan and Avent, Brendan and Bellet, Aur{\'e}lien and Bennis, Mehdi and Bhagoji, Arjun N and Zhao, Sen},
  journal={Foundations and Trends® in Machine Learning},
  volume={14},
  number={1--2},
  pages={1--210},
  year={2021},
  doi={10.1561/2200000083}
}


@inproceedings{kendall2017uncertainties,
  title={What uncertainties do we need in Bayesian deep learning for computer vision?},
  author={Kendall, Alex and Gal, Yarin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5574--5584},
  year={2017}
}

@book{kochenderfer2022decision,
  title={Decision making under uncertainty: Theory and application},
  author={Kochenderfer, Mykel J and Amato, Christopher and Chowdhary, Girish and How, Jonathan P and Reynolds, H John and Thornton, Jason R and Vian, John},
  year={2022},
  edition={2nd},
  publisher={MIT Press}
}

@inproceedings{lakshminarayanan2017simple,
  title={Simple and scalable predictive uncertainty estimation using deep ensembles},
  author={Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6402--6413},
  year={2017}
}

@article{liu2021,
  title={Context-aware machine learning for intelligent systems: A survey},
  author={Liu, Xiang and Sun, Chang and Lin, Li and Wang, Hui},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={33},
  number={7},
  pages={2956--2971},
  year={2021},
  doi={10.1109/TKDE.2019.2961675}
}

@article{mehrabi2021survey,
  title={A survey on bias and fairness in machine learning},
  author={Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
  journal={ACM Computing Surveys},
  volume={54},
  number={6},
  pages={1--35},
  year={2021},
  doi={10.1145/3457607}
}



@inproceedings{muller2021shifting,
  title={Shifting expectations: Understanding user reactions to changes in AI system performance},
  author={Muller, Michael and Liao, Q Vera and Gruen, Daniel},
  booktitle={Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems},
  pages={1--14},
  year={2021},
  organization={ACM},
  doi={10.1145/3411764.3445141}
}

@inproceedings{ovadia2019can,
  title={Can you trust your model's uncertainty? Evaluating predictive uncertainty under dataset shift},
  author={Ovadia, Yaniv and Fertig, Emily and Ren, Jie and Nado, Zachary and Sculley, D and Nowozin, Sebastian and Snoek, Jasper},
  booktitle={Advances in Neural Information Processing Systems},
  pages={13991--14002},
  year={2019}
}

@article{qi2020data,
  title={Data uncertainty in deep learning: A survey},
  author={Qi, Jian and Luo, Hao and Xu, Hong and Xiong, Zhiqiang},
  journal={IEEE Access},
  volume={8},
  pages={128022--128034},
  year={2020},
  publisher={IEEE},
  doi={10.1109/ACCESS.2020.3007104}
}

@article{shorten2019survey,
  title={A survey on image data augmentation for deep learning},
  author={Shorten, Connor and Khoshgoftaar, Taghi M},
  journal={Journal of Big Data},
  volume={6},
  number={1},
  pages={1--48},
  year={2019},
  doi={10.1186/s40537-019-0197-0}
}

@article{situ2021context,
  title={Context-aware conversational AI: A survey},
  author={Situ, Hao and Wang, Yuguang and Zhang, Deqing},
  journal={Artificial Intelligence Review},
  volume={54},
  number={4},
  pages={3149--3192},
  year={2021},
  doi={10.1007/s10462-020-09933-7}
}

@inproceedings{suresh2021framework,
  title={A framework for understanding unintended consequences of machine learning},
  author={Suresh, Harini and Guttag, John V},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={1},
  pages={930--938},
  year={2021}
}

@inproceedings{yang2020unremarkable,
  title={Unremarkable AI: Fitting intelligent decision support into critical, clinical decision-making processes},
  author={Yang, Qian and Steinfeld, Aaron and Zimmerman, John},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--12},
  year={2020},
  organization={ACM},
  doi={10.1145/3313831.3376638}
}

@inproceedings{yin2019understanding,
  title={Understanding the effect of accuracy on trust in machine learning models},
  author={Yin, Ming and Wortman Vaughan, Jennifer and Wallach, Hanna},
  booktitle={Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems},
  pages={1--12},
  year={2019},
  organization={ACM},
  doi={10.1145/3290605.3300509}
}

@inproceedings{zhou2020uncertainty,
  title={Uncertainty estimation and sample selection for crowd counting},
  author={Zhou, Zhiqiang and Siddiquee, M M Rahman and Tajbakhsh, Nima and Liang, Jianming},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10117--10126},
  year={2020},
  doi={10.1109/CVPR42600.2020.01013}
}

@article{Ong2025,
abstract = {Sustainability commonly refers to entities, such as individuals, companies, and institutions, having a non-detrimental (or even positive) impact on the environment, society, and the economy. With sustainability becoming a synonym of acceptable and legitimate behaviour, it is being increasingly demanded and regulated. Several frameworks and standards have been proposed to measure the sustainability impact of corporations, including United Nations' sustainable development goals and the recently introduced global sustainability reporting framework, amongst others. However, the concept of corporate sustainability is complex due to the diverse and intricate nature of firm operations (i.e. geography, size, business activities, interlinks with other stakeholders). As a result, corporate sustainability assessments are plagued by subjectivity both within data that reflect corporate sustainability efforts (i.e. corporate sustainability disclosures) and the analysts evaluating them. This subjectivity can be distilled into distinct challenges, such as incompleteness, ambiguity, unreliability and sophistication on the data dimension, as well as limited resources and potential bias on the analyst dimension. Put together, subjectivity hinders effective cost attribution to entities non-compliant with prevailing sustainability expectations, potentially rendering sustainability efforts and its associated regulations futile. To this end, we argue that Explainable Natural Language Processing (XNLP) can significantly enhance corporate sustainability analysis. Specifically, linguistic understanding algorithms (lexical, semantic, syntactic), integrated with XAI capabilities (interpretability, explainability, faithfulness), can bridge gaps in analyst resources and mitigate subjectivity problems within data.},
author = {Ong, Keane and Mao, Rui and Satapathy, Ranjan and Filho, Ricardo Shirota and Cambria, Erik and Sulaeman, Johan and Mengaldo, Gianmarco},
doi = {10.1016/j.inffus.2024.102726},
file = {:C\:/Users/RHfix/Desktop/1-s2.0-S1566253524005049-main.pdf:pdf},
issn = {15662535},
journal = {Information Fusion},
keywords = {Corporate sustainability,Explainable artificial intelligence,Explainable natural language processing,Sustainability analysis,Sustainability disclosure},
mendeley-groups = {Certainty},
number = {September 2024},
pages = {102726},
publisher = {Elsevier B.V.},
title = {{Explainable natural language processing for corporate sustainability analysis}},
url = {https://doi.org/10.1016/j.inffus.2024.102726},
volume = {115},
year = {2025}
}
@article{Baghirov2024,
author = {Baghirov, E.},
doi = {10.1016/j.csa.2024.100072},
file = {:C\:/Users/RHfix/Desktop/1-s2.0-S2772918424000389-main.pdf:pdf},
issn = {27729184},
journal = {Cyber Security and Applications},
keywords = {"Explainable AI","LIME","LightGBM","Malware analysis","Malware detection","SHAP"},
mendeley-groups = {Certainty},
number = {September 2024},
pages = {100072},
publisher = {Elsevier B.V.},
title = {{A Comprehensive Investigation into Robust Malware Detection with Explainable AI}},
url = {https://doi.org/10.1016/j.csa.2024.100072},
volume = {3},
year = {2024}
}

@misc{duan2024shiftingattentionrelevancepredictive,
      title={Shifting Attention to Relevance: Towards the Predictive Uncertainty Quantification of Free-Form Large Language Models}, 
      author={Jinhao Duan and Hao Cheng and Shiqi Wang and Alex Zavalny and Chenan Wang and Renjing Xu and Bhavya Kailkhura and Kaidi Xu},
      year={2024},
      eprint={2307.01379},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2307.01379}, 
}

@misc{li2024,
      title={Think Twice Before Trusting: Self-Detection for Large Language Models through Comprehensive Answer Reflection}, 
      author={Moxin Li and Wenjie Wang and Fuli Feng and Fengbin Zhu and Qifan Wang and Tat-Seng Chua},
      year={2024},
      eprint={2403.09972},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2403.09972}, 
}

@misc{li2024thinktwicetrustingselfdetection,
      title={Think Twice Before Trusting: Self-Detection for Large Language Models through Comprehensive Answer Reflection}, 
      author={Moxin Li and Wenjie Wang and Fuli Feng and Fengbin Zhu and Qifan Wang and Tat-Seng Chua},
      year={2024},
      eprint={2403.09972},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2403.09972}, 
}

@article{Malinin2021,
abstract = {Uncertainty estimation is important for ensuring safety and robustness of AI systems. While most research in the area has focused on unstructured prediction tasks, limited work has investigated general uncertainty estimation approaches for structured prediction. Thus, this work aims to investigate uncertainty estimation for autoregressive structured prediction tasks within a single unified and interpretable probabilistic ensemble-based framework. We consider uncertainty estimation for sequence data at the token-level and complete sequence-level; interpretations for, and applications of, various measures of uncertainty; and discuss both the theoretical and practical challenges associated with obtaining them. This work also provides baselines for token-level and sequence-level error detection, and sequence-level out-of-domain input detection on the WMT'14 English-French and WMT'17 English-German translation and LibriSpeech speech recognition datasets.},
archivePrefix = {arXiv},
arxivId = {2002.07650},
author = {Malinin, Andrey and Gales, Mark},
eprint = {2002.07650},
file = {:F\:/Medical 1/Paper 45.pdf:pdf},
journal = {ICLR 2021 - 9th International Conference on Learning Representations},
mendeley-groups = {000000},
pages = {1--31},
title = {{Uncertainty Estimation in Autoregressive Structured Prediction}},
year = {2021}
}
@misc{wang2024wordsequenceentropyuncertaintyestimation,
      title={Word-Sequence Entropy: Towards Uncertainty Estimation in Free-Form Medical Question Answering Applications and Beyond}, 
      author={Zhiyuan Wang and Jinhao Duan and Chenxi Yuan and Qingyu Chen and Tianlong Chen and Yue Zhang and Ren Wang and Xiaoshuang Shi and Kaidi Xu},
      year={2024},
      eprint={2402.14259},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2402.14259}, 
}

@misc{han2024miningcausalityaiassistedsearch,
      title={Mining Causality: AI-Assisted Search for Instrumental Variables}, 
      author={Sukjin Han},
      year={2024},
      eprint={2409.14202},
      archivePrefix={arXiv},
      primaryClass={econ.EM},
      url={https://arxiv.org/abs/2409.14202}, 
}


@misc{peng2024uncertaintyawareexplainablerecommendationlarge,
      title={Uncertainty-Aware Explainable Recommendation with Large Language Models}, 
      author={Yicui Peng and Hao Chen and Chingsheng Lin and Guo Huang and Jinrong Hu and Hui Guo and Bin Kong and Shu Hu and Xi Wu and Xin Wang},
      year={2024},
      eprint={2402.03366},
      archivePrefix={arXiv},
      primaryClass={cs.IR},
      url={https://arxiv.org/abs/2402.03366}, 
}

@misc{xie2024preliminarystudyo1medicine,
      title={A Preliminary Study of o1 in Medicine: Are We Closer to an AI Doctor?}, 
      author={Yunfei Xie and Juncheng Wu and Haoqin Tu and Siwei Yang and Bingchen Zhao and Yongshuo Zong and Qiao Jin and Cihang Xie and Yuyin Zhou},
      year={2024},
      eprint={2409.15277},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2409.15277}, 
}

@article{Huang2024,
abstract = {Large Language Models (LLMs) obtain their instruction-following ability through instruction tuning. While the quality of instruction data is considered critical for a successful LLM, the selection of high-quality datasets for finetuning still lacks clear guidelines and quantitative analyses. In this work, we introduce three analytical views for instruction mining: diversity, complexity, and accuracy, which can aid in selecting an optimal subset of instruction data for fine-tuning. Based on these views, we propose a multi-view fusion framework for efficient instruction selection, including diversity sampling based on LoRA representation distribution, complexity scoring based on uncertainty quantification, and accuracy scoring based on reward modeling. We perform the framework on various open-sourced instruction datasets, and achieved enhanced performance of LLMs with a carefully curated subset, underscoring the effectiveness of our proposed framework.},
author = {Huang, Hui and Xu, Bing and Liang, Xinnian and Chen, Kehai and Yang, Muyun and Zhao, Tiejun and Zhu, Conghui},
doi = {10.1016/j.inffus.2024.102480},
file = {:F\:/Medical 1/paper 11.pdf:pdf},
issn = {15662535},
journal = {Information Fusion},
keywords = {Instruction mining,Instruction tuning,Large language model},
mendeley-groups = {000000},
number = {May},
pages = {102480},
publisher = {Elsevier B.V.},
title = {{Multi-view fusion for instruction mining of large language model}},
url = {https://doi.org/10.1016/j.inffus.2024.102480},
volume = {110},
year = {2024}
}
@article{Mahjour2024,
abstract = {ChatGPT, a prominent large language model (LLM), is being increasingly used across a wide range of scientific fields. Geosystem engineers and researchers are also posed to leverage ChatGPT to find solutions to challenges encountered in various topics. This study evaluates the accuracy and reproducibility of ChatGPT in responding to different qualitative and quantitative questions, with a particular focus on risk and uncertainty (R\& U) in both the Greenfield and Brownfield domains as an important area of interest. The results show the importance of prompting to considerably improve the ChatGPT's response accuracy and reproducibility. The findings highlight that the greater the comprehensiveness of the prompts, the higher the accuracy and reproducibility of the responses to the questions. The study also acknowledges the potential limitations associated with the sources of information and the contextual influences on the reliability of the response.},
author = {Mahjour, Seyed Kourosh and Soltanmohammadi, Ramin and Heidaryan, Ehsan and Faroughi, Salah A.},
doi = {10.1016/j.geoen.2024.212889},
file = {:F\:/Medical 1/Paper 12.pdf:pdf},
issn = {29498910},
journal = {Geoenergy Science and Engineering},
keywords = {ChatGPT,Geosystems,Greenfield \& Brownfield,Prompting,Risk \& uncertainty},
mendeley-groups = {000000},
number = {May},
pages = {212889},
publisher = {Elsevier B.V.},
title = {{Geosystems risk and uncertainty: The application of ChatGPT with targeted prompting}},
url = {https://doi.org/10.1016/j.geoen.2024.212889},
volume = {238},
year = {2024}
}
@article{Seedat2024,
abstract = {Machine Learning (ML) in low-data settings remains an underappreciated yet crucial problem. Hence, data augmentation methods to increase the sample size of datasets needed for ML are key to unlocking the transformative potential of ML in data-deprived regions and domains. Unfortunately, the limited training set constrains traditional tabular synthetic data generators in their ability to generate a large and diverse augmented dataset needed for ML tasks. To address this challenge, we introduce CLLM, which leverages the prior knowledge of Large Language Models (LLMs) for data augmentation in the low-data regime. However, not all the data generated by LLMs will improve downstream utility, as for any generative model. Consequently, we introduce a principled curation mechanism, leveraging learning dynamics, coupled with confidence and uncertainty metrics, to obtain a high-quality dataset. Empirically, on multiple real-world datasets, we demonstrate the superior performance of CLLM in the low-data regime compared to conventional generators. Additionally, we provide insights into the LLM generation and curation mechanism, shedding light on the features that enable them to output high-quality augmented datasets.},
archivePrefix = {arXiv},
arxivId = {2312.12112},
author = {Seedat, Nabeel and Huynh, Nicolas and van Breugel, Boris and van der Schaar, Mihaela},
eprint = {2312.12112},
file = {:F\:/Medical 1/Paper 13.pdf:pdf},
issn = {26403498},
journal = {Proceedings of Machine Learning Research},
mendeley-groups = {000000},
number = {Ml},
pages = {44060--44092},
title = {{Curated LLM: Synergy of LLMs and Data Curation for tabular augmentation in low-data regimes}},
volume = {235},
year = {2024}
}
@article{Yin2024,
abstract = {We study how to characterize and predict the truthfulness of texts generated from large language models (LLMs), which serves as a crucial step in building trust between humans and LLMs. Although several approaches based on entropy or verbalized uncertainty have been proposed to calibrate model predictions, these methods are often intractable, sensitive to hyperparameters, and less reliable when applied in generative tasks with LLMs. In this paper, we suggest investigating internal activations and quantifying LLM's truthfulness using the local intrinsic dimension (LID) of model activations. Through experiments on four question answering (QA) datasets, we demonstrate the effectiveness of our proposed method. Additionally, we study intrinsic dimensions in LLMs and their relations with model layers, autoregressive language modeling, and the training of LLMs, revealing that intrinsic dimensions can be a powerful approach to understanding LLMs. Code is available at: https://github.com/fanyin3639/LID-HallucinationDetection.},
archivePrefix = {arXiv},
arxivId = {2402.18048},
author = {Yin, Fan and Srinivasa, Jayanth and Chang, Kai Wei},
eprint = {2402.18048},
file = {:F\:/Medical 1/Paper 14.pdf:pdf},
issn = {26403498},
journal = {Proceedings of Machine Learning Research},
mendeley-groups = {000000},
pages = {57069--57084},
title = {{Characterizing Truthfulness in Large Language Model Generations with Local Intrinsic Dimension}},
volume = {235},
year = {2024}
}
@article{Osman2024,
abstract = {Data integration is considered a classic research field and a pressing need within the information science community. Ontologies play a critical role in such processes by providing well-consolidated support to link and semantically integrate datasets via interoperability. This paper approaches data integration from an application perspective by looking at ontology matching techniques. As the manual matching of different sources of information becomes unrealistic once the system scales up, the automation of the matching process becomes a compelling need. Therefore, we have conducted experiments on actual non-semantically enriched relational data with the support of existing tools (pre-LLM technology) for automatic ontology matching from the scientific community. Even considering a relatively simple case study—i.e., the spatio–temporal alignment of macro indicators—outcomes clearly show significant uncertainty resulting from errors and inaccuracies along the automated matching process. More concretely, this paper aims to test on real-world data a bottom-up knowledge-building approach, discuss the lessons learned from the experimental results of the case study, and draw conclusions about uncertainty and uncertainty management in an automated ontology matching process. While the most common evaluation metrics clearly demonstrate the unreliability of fully automated matching solutions, properly designed semi-supervised approaches seem to be mature for more generalized application.},
author = {Osman, In{\`{e}}s and Pileggi, Salvatore Flavio and Yahia, Sadok Ben},
doi = {10.3390/app14114679},
file = {:F\:/Medical 1/Paper 15.pdf:pdf},
issn = {20763417},
journal = {Applied Sciences (Switzerland)},
keywords = {data integration,ontology matching,uncertainty},
mendeley-groups = {000000},
number = {11},
title = {{Uncertainty in Automated Ontology Matching: Lessons from an Empirical Evaluation}},
volume = {14},
year = {2024}
}
@article{Kim2024,
abstract = {Widely deployed large language models (LLMs) can produce convincing yet incorrect outputs, potentially misleading users who may rely on them as if they were correct. To reduce such overreliance, there have been calls for LLMs to communicate their uncertainty to end users. However, there has been little empirical work examining how users perceive and act upon LLMs' expressions of uncertainty. We explore this question through a large-scale, pre-registered, human-subject experiment (N=404) in which participants answer medical questions with or without access to responses from a fictional LLM-infused search engine. Using both behavioral and self-reported measures, we examine how different natural language expressions of uncertainty impact participants' reliance, trust, and overall task performance. We find that first-person expressions (e.g., "I'm not sure, but...") decrease participants' confidence in the system and tendency to agree with the system's answers, while increasing participants' accuracy. An exploratory analysis suggests that this increase can be attributed to reduced (but not fully eliminated) overreliance on incorrect answers. While we observe similar effects for uncertainty expressed from a general perspective (e.g., "It's not clear, but..."), these effects are weaker and not statistically significant. Our findings suggest that using natural language expressions of uncertainty may be an effective approach for reducing overreliance on LLMs, but that the precise language used matters. This highlights the importance of user testing before deploying LLMs at scale.},
archivePrefix = {arXiv},
arxivId = {2405.00623},
author = {Kim, Sunnie S.Y. and Liao, Q. Vera and Vorvoreanu, Mihaela and Ballard, Stephanie and Vaughan, Jennifer Wortman},
doi = {10.1145/3630106.3658941},
eprint = {2405.00623},
file = {:F\:/Medical 1/Paper 16.pdf:pdf},
isbn = {9798400704505},
journal = {2024 ACM Conference on Fairness, Accountability, and Transparency, FAccT 2024},
keywords = {Human-AI interaction,Large language models,Overreliance,Trust in AI,Uncertainty expression},
mendeley-groups = {000000},
pages = {822--835},
title = {{"I'm Not Sure, But...": Examining the Impact of Large Language Models' Uncertainty Expression on User Reliance and Trust}},
year = {2024}
}
@article{Cai2024,
abstract = {Histopathological whole-slide image (WSI) segmentation is essential for precise tissue characterization in medical diagnostics. However, traditional approaches require labor-intensive pixel-level annotations. To this end, we study weakly supervised semantic segmentation (WSSS) which uses patch-level classification labels, reducing annotation efforts significantly. However, the complexity of WSIs and the challenge of sparse classification labels hinder effective dense pixel predictions. Moreover, due to the multi-label nature of WSI, existingapproachesofsingle-labelcontrastivelearningdesignedfortherepresentationofsingle-category, neglecting the presence of other relevant categories and thus fail to adapt to WSI tasks. This paper presents a novel multilabel contrastive learning method for WSSS by incorporating class-specific embedding extraction with LLM features guidance. Specifically, we propose to obtain class-specific embeddings by utilizing classifier weights, followed by a dot-product-based attention fusion method that leverages LLM features to enrich their semantics, facilitating contrastive learning between different classes from single image. Besides, we propose a Robust Learning approach that leverages multi-layer features to evaluate the uncertainty of pseudo-labels, thereby mitigating the impact of noisy pseudo-labels on the learning process of segmentation. Extensive experiments have been conducted on two Histopathological image segmentation datasets, i.e. LUAD dataset and BCSS dataset, demonstrating the effectiveness of our methods with leading performance.},
author = {Cai, Wentian and Li, Yijiang and Chen, Yandan and Lin, Jing and Huang, Zihao and Gao, Ping and Gadekallu, Thippa Reddy and Wang, Wei and Gao, Ying},
doi = {10.1109/JBHI.2024.3450013},
file = {:F\:/Medical 1/Paper 17.pdf:pdf},
issn = {21682208},
journal = {IEEE Journal of Biomedical and Health Informatics},
keywords = {LLMs,Weakly supervised learning,contrastive learning,medical image segmentation},
mendeley-groups = {000000},
pages = {1--11},
pmid = {39236138},
publisher = {IEEE},
title = {{Enhancing Weakly Supervised Semantic Segmentation with Multi-label Contrastive Learning and LLM Features Guidance}},
volume = {PP},
year = {2024}
}
@article{Bakman2024,
abstract = {Generative Large Language Models (LLMs) have recently been widely utilized for their unprecedented capabil-ities across many tasks. Considering their use in high-stakes environments and for mission-critical applications, the fact that LLMs often can generate inaccurate or misleading results can be potentially harmful, which motivates us to study the correctness of generative LLM outputs. Uncertainty Estimation (UE) in generative LLMs is a developing area, with state-of-the-art probability-based techniques frequently using length-normalized scoring. As an alternative to length-normalized scoring in UE, in this work, we propose Meaning-Aware Response Scoring (MARS). The key idea of MARS is to consider the semantic contribution of each token of the generated sequence to the context of the question during UE. Through extensive experiments on three question-answering datasets across five pretrained LLMs, we show that utilizing MARS during UE results in a universal and significant improvement in UE performance.},
author = {Bakman, Yavuz Faruk and Yaldiz, Duygu Nur and Buyukates, Baturalp and Avestimehr, Salman and Tao, Chenyang and Dimitriadis, Dimitrios},
doi = {10.1109/ISIT57864.2024.10619136},
file = {:F\:/Medical 1/Paper 18.pdf:pdf},
isbn = {9798350382846},
issn = {21578095},
journal = {IEEE International Symposium on Information Theory - Proceedings},
mendeley-groups = {000000},
pages = {2033--2037},
publisher = {IEEE},
title = {{Predicting Uncertainty of Generative LLMs with MARS: Meaning-Aware Response Scoring}},
year = {2024}
}
@article{Polak2024,
abstract = {There has been a growing effort to replace manual extraction of data from research papers with automated data extraction based on natural language processing, language models, and recently, large language models (LLMs). Although these methods enable efficient extraction of data from large sets of research papers, they require a significant amount of up-front effort, expertise, and coding. In this work, we propose the ChatExtract method that can fully automate very accurate data extraction with minimal initial effort and background, using an advanced conversational LLM. ChatExtract consists of a set of engineered prompts applied to a conversational LLM that both identify sentences with data, extract that data, and assure the data's correctness through a series of follow-up questions. These follow-up questions largely overcome known issues with LLMs providing factually inaccurate responses. ChatExtract can be applied with any conversational LLMs and yields very high quality data extraction. These results suggest that approaches similar to ChatExtract, due to their simplicity, transferability, and accuracy are likely to become powerful tools for data extraction in the near future. Finally, databases for critical cooling rates of metallic glasses and yield strengths of high entropy alloys are developed using ChatExtract.},
archivePrefix = {arXiv},
arxivId = {2303.05352},
author = {Polak, Maciej P. and Morgan, Dane},
doi = {10.1038/s41467-024-45914-8},
eprint = {2303.05352},
file = {:F\:/Medical 1/Paper 19.pdf:pdf},
isbn = {4146702445},
issn = {20411723},
journal = {Nature Communications},
mendeley-groups = {000000},
number = {1},
pages = {1--11},
pmid = {38383556},
publisher = {Springer US},
title = {{Extracting accurate materials data from research papers with conversational language models and prompt engineering}},
volume = {15},
year = {2024}
}
@article{Farquhar2024,
abstract = {Large language model (LLM) systems, such as ChatGPT1 or Gemini2, can show impressive reasoning and question-answering capabilities but often ‘hallucinate' false outputs and unsubstantiated answers3,4. Answering unreliably or without the necessary information prevents adoption in diverse fields, with problems including fabrication of legal precedents5 or untrue facts in news articles6 and even posing a risk to human life in medical domains such as radiology7. Encouraging truthfulness through supervision or reinforcement has been only partially successful8. Researchers need a general method for detecting hallucinations in LLMs that works even with new and unseen questions to which humans might not know the answer. Here we develop new methods grounded in statistics, proposing entropy-based uncertainty estimators for LLMs to detect a subset of hallucinations—confabulations—which are arbitrary and incorrect generations. Our method addresses the fact that one idea can be expressed in many ways by computing uncertainty at the level of meaning rather than specific sequences of words. Our method works across datasets and tasks without a priori knowledge of the task, requires no task-specific data and robustly generalizes to new tasks not seen before. By detecting when a prompt is likely to produce a confabulation, our method helps users understand when they must take extra care with LLMs and opens up new possibilities for using LLMs that are otherwise prevented by their unreliability.},
author = {Farquhar, Sebastian and Kossen, Jannik and Kuhn, Lorenz and Gal, Yarin},
doi = {10.1038/s41586-024-07421-0},
file = {:F\:/Medical 1/Paper 20.pdf:pdf},
issn = {14764687},
journal = {Nature},
mendeley-groups = {000000},
number = {8017},
pages = {625--630},
pmid = {38898292},
publisher = {Springer US},
title = {{Detecting hallucinations in large language models using semantic entropy}},
url = {http://dx.doi.org/10.1038/s41586-024-07421-0},
volume = {630},
year = {2024}
}
@article{DeGroat2024,
abstract = {Personalized interventions are deemed vital given the intricate characteristics, advancement, inherent genetic composition, and diversity of cardiovascular diseases (CVDs). The appropriate utilization of artificial intelligence (AI) and machine learning (ML) methodologies can yield novel understandings of CVDs, enabling improved personalized treatments through predictive analysis and deep phenotyping. In this study, we proposed and employed a novel approach combining traditional statistics and a nexus of cutting-edge AI/ML techniques to identify significant biomarkers for our predictive engine by analyzing the complete transcriptome of CVD patients. After robust gene expression data pre-processing, we utilized three statistical tests (Pearson correlation, Chi-square test, and ANOVA) to assess the differences in transcriptomic expression and clinical characteristics between healthy individuals and CVD patients. Next, the recursive feature elimination classifier assigned rankings to transcriptomic features based on their relation to the case–control variable. The top ten percent of commonly observed significant biomarkers were evaluated using four unique ML classifiers (Random Forest, Support Vector Machine, Xtreme Gradient Boosting Decision Trees, and k-Nearest Neighbors). After optimizing hyperparameters, the ensembled models, which were implemented using a soft voting classifier, accurately differentiated between patients and healthy individuals. We have uncovered 18 transcriptomic biomarkers that are highly significant in the CVD population that were used to predict disease with up to 96 accuracy. Additionally, we cross-validated our results with clinical records collected from patients in our cohort. The identified biomarkers served as potential indicators for early detection of CVDs. With its successful implementation, our newly developed predictive engine provides a valuable framework for identifying patients with CVDs based on their biomarker profiles.},
author = {DeGroat, William and Abdelhalim, Habiba and Patel, Kush and Mendhe, Dinesh and Zeeshan, Saman and Ahmed, Zeeshan},
doi = {10.1038/s41598-023-50600-8},
file = {:F\:/Medical 1/Paper 21.pdf:pdf},
isbn = {0123456789},
issn = {20452322},
journal = {Scientific Reports},
mendeley-groups = {000000},
number = {1},
pages = {1--13},
pmid = {38167627},
publisher = {Nature Publishing Group UK},
title = {{Discovering biomarkers associated and predicting cardiovascular disease with high accuracy using a novel nexus of machine learning techniques for precision medicine}},
url = {https://doi.org/10.1038/s41598-023-50600-8},
volume = {14},
year = {2024}
}
@article{Maloney2024,
abstract = {English speakers use probabilistic phrases such as likely to communicate information about the probability or likelihood of events. Communication is successful to the extent that the listener grasps what the speaker means to convey and, if communication is successful, individuals can potentially coordinate their actions based on shared knowledge about uncertainty. We first assessed human ability to estimate the probability and the ambiguity (imprecision) of twenty-three probabilistic phrases in a coordination game in two different contexts, investment advice and medical advice. We then had GPT-4 (OpenAI), a Large Language Model, complete the same tasks as the human participants. We found that GPT-4's estimates of probability both in the Investment and Medical Contexts were as close or closer to that of the human participants as the human participants' estimates were to one another. However, further analyses of residuals disclosed small but significant differences between human and GPT-4 performance. Human probability estimates were compressed relative to those of GPT-4. Estimates of probability for both the human participants and GPT-4 were little affected by context. We propose that evaluation methods based on coordination games provide a systematic way to assess what GPT-4 and similar programs can and cannot do.},
author = {Maloney, Laurence T. and {Dal Martello}, Maria F. and Fei, Vivian and Ma, Valerie},
doi = {10.1038/s41598-024-56740-9},
file = {:F\:/Medical 1/Paper 22.pdf:pdf},
isbn = {0123456789},
issn = {20452322},
journal = {Scientific Reports},
keywords = {Ambiguity,GPT-4,LLM,Pragmatics,Probabilistic phrases,Probability},
mendeley-groups = {000000},
number = {1},
pages = {1--11},
pmid = {38514688},
publisher = {Nature Publishing Group UK},
title = {{A comparison of human and GPT-4 use of probabilistic phrases in a coordination game}},
url = {https://doi.org/10.1038/s41598-024-56740-9},
volume = {14},
year = {2024}
}
@article{Hao2024,
abstract = {Large language models (LLMs) are becoming a significant source of content generation in social networks, which is a typical complex adaptive system (CAS). However, due to their hallucinatory nature, LLMs produce false information that can spread through social networks, which will impact the stability of the whole society. The uncertainty of LLMs false information spread within social networks is attributable to the diversity of individual behaviors, intricate interconnectivity, and dynamic network structures. Quantifying the uncertainty of false information spread by LLMs in social networks is beneficial for preemptively devising strategies to defend against threats. To address these challenges, we propose an LLMs hallucination-aware dynamic modeling method via agent-based probability distributions, spread popularity and community affiliation, to quantify the uncertain spreading of LLMs hallucination in social networks. We set up the node attributes and behaviors in the model based on real-world data. For evaluation, we consider the spreaders, informed people, discerning and unwilling non-spreaders as indicators, and quantified the spreading under different LLMs task situations, such as QA, dialogue, and summarization, as well as LLMs versions. Furthermore, we conduct experiments using real-world LLM hallucination data combined with social network features to ensure the validity of the proposed quantifying scheme.},
author = {Hao, Guozhi and Wu, Jun and Pan, Qianqian and Morello, Rosario},
doi = {10.1038/s41598-024-66708-4},
file = {:F\:/Medical 1/Paper 23.pdf:pdf},
isbn = {4159802466708},
issn = {20452322},
journal = {Scientific Reports},
mendeley-groups = {000000},
number = {1},
pages = {1--13},
pmid = {39014013},
publisher = {Nature Publishing Group UK},
title = {{Quantifying the uncertainty of LLM hallucination spreading in complex adaptive social networks}},
url = {https://doi.org/10.1038/s41598-024-66708-4},
volume = {14},
year = {2024}
}
@article{Yang2024,
abstract = {To complete tasks in dynamic environments, robots need to timely update their plans to react to environment changes. Traditional stripe-like or learning-based planners struggle to achieve this due to their high reliance on meticulously predefined planning rules or labeled data. Fortunately, recent works find that Large Language Models (LLMs) can be effectively prompted to solve planning problems. Thus, we investigate the strategies for LLMs to master reactive planning problems without complex definitions and extra training. We propose Text2Reaction, an LLM-based framework enabling robots to continuously reason and update plans according to the latest environment changes. Inspired from human's step-by-step re-planning process, we present the Re-planning Prompt, which informs LLMs the basic principles of re-planning and fosters the gradual development of a current plan to a new one in a three-hop reasoning manner-cause analysis, consequence inference, and plan adjustment. In addition, Text2Reaction is designed to first generate an initial plan based on the task description before execution, allowing for subsequent iterative updates of this plan. We demonstrate the superior performance of Text2Reaction over prior works in reacting to various environment changes and completing varied tasks. In addition, we validate the reliability of our re-planning prompt through ablation experiments and its capability when deployed in real-world robots, enabling continuous reasoning in the face of diverse changes until the user instructions are successfully completed.},
author = {Yang, Zejun and Ning, Li and Wang, Haitao and Jiang, Tianyu and Zhang, Shaolin and Cui, Shaowei and Jiang, Hao and Li, Chunpeng and Wang, Shuo and Wang, Zhaoqi},
doi = {10.1109/LRA.2024.3371223},
file = {:F\:/Medical 1/Paper 24.pdf:pdf},
issn = {23773766},
journal = {IEEE Robotics and Automation Letters},
keywords = {AI-based methods,Planning under uncertainty,learning from demonstration},
mendeley-groups = {000000},
number = {5},
pages = {4003--4010},
title = {{Text2Reaction : Enabling Reactive Task Planning Using Large Language Models}},
volume = {9},
year = {2024}
}
@article{Bond2024,
abstract = {There is considerable uncertainty about the role that Artificial Intelligence (AI) might play in Environmental Impact Assessment (EIA), including into research. AI large language model (LLM) chatbots have the potential to increase the efficiency of EIA research, but their outputs can create concerns. This paper investigates the potential time savings achievable using LLM chatbots to undertake a critical review of literature focussing on the use of AI in EIA. Using a combination of ChatGPT and Elicit, literature was reviewed to identify 12 key issues associated with the use of AI in EIA and this paper was prepared in three and a half days from initial conception. A protocol is developed to assist researchers in fact checking evidence delivered through Elicit (or other machine learning tools) which serves as a novel outcome of this research. Using comments from three peer reviewers allowed some more objective reflection on the credibility of the LLM chatbot-derived output, on the appropriateness of the time savings, and on the future research needed on the application of LLM chatbots in this context.},
author = {Bond, Alan and Cilliers, Dirk and Retief, Francois and Alberts, Reece and Roos, Claudine and Moolman, Jurie},
doi = {10.1080/14615517.2024.2320591},
file = {:F\:/Medical 1/Paper 25.pdf:pdf},
issn = {14615517},
journal = {Impact Assessment and Project Appraisal},
keywords = {Artificial Intelligence (AI),Environmental Impact Assessment (EIA),ethics,future challenges,issues},
mendeley-groups = {000000},
number = {2},
pages = {189--199},
publisher = {Taylor \& Francis},
title = {{Using an Artificial intelligence chatbot to critically review the scientific literature on the use of Artificial intelligence in Environmental Impact Assessment}},
url = {https://doi.org/10.1080/14615517.2024.2320591},
volume = {42},
year = {2024}
}
@article{AltntasAykan2024,
author = {{Altıntaş Aykan}, Duygun and Aykan, Ahmet {\c{C}}ağrı and {\c{C}}elik, Enes and {\"{O}}zt{\"{u}}rk, Bayram},
doi = {10.1111/bcp.16265},
file = {:F\:/Medical 1/Paper 26.pdf:pdf},
issn = {13652125},
journal = {British Journal of Clinical Pharmacology},
keywords = {adiposity,antihypertensive drugs,clinical pharmacology,skinfold thickness},
mendeley-groups = {000000},
number = {August},
pages = {1--7},
pmid = {39351823},
title = {{Assessment of the influence of body fat indices on antihypertensive drug responses}},
year = {2024}
}
@article{Croissant2024,
abstract = {The development of believable, natural, and interactive digital artificial agents is a field of growing interest. Theoretical uncertainties and technical barriers present considerable challenges to the field, particularly with regards to developing agents that effectively simulate human emotions. Large language models (LLMs) might address these issues by tapping common patterns in situational appraisal. In three empirical experiments, this study tests the capabilities of LLMs to solve emotional intelligence tasks and to simulate emotions. It presents and evaluates a new Chain-of-Emotion architecture for emotion simulation within video games, based on psychological appraisal research. Results show that it outperforms control LLM architectures on a range of user experience and content analysis metrics. This study therefore provides early evidence of how to construct and test affective agents based on cognitive processes represented in language models.},
archivePrefix = {arXiv},
arxivId = {2309.05076},
author = {Croissant, Maximilian and Frister, Madeleine and Schofield, Guy and McCall, Cade},
doi = {10.1371/journal.pone.0301033},
eprint = {2309.05076},
file = {:F\:/Medical 1/Paper 27.pdf:pdf},
isbn = {1111111111},
issn = {19326203},
journal = {PLoS ONE},
mendeley-groups = {000000},
number = {5 May},
pages = {1--21},
pmid = {38728280},
title = {{An appraisal-based chain-of-emotion architecture for affective language model game agents}},
url = {http://dx.doi.org/10.1371/journal.pone.0301033},
volume = {19},
year = {2024}
}
@article{Collins2024,
abstract = {There is much excitement about the opportunity to harness the power of large language models (LLMs) when building problem-solving assistants. However, the standard methodology of evaluating LLMs relies on static pairs of inputs and outputs; this is insufficient for making an informed decision about which LLMs are best to use in an interactive setting, and how that varies by setting. Static assessment therefore limits how we understand language model capabilities. We introduce CheckMate, an adaptable prototype platform for humans to interact with and evaluate LLMs. We conduct a study with CheckMate to evaluate three language models (InstructGPT, ChatGPT, and GPT-4) as assistants in proving undergraduate-level mathematics, with a mixed cohort of participants from undergraduate students to professors of mathematics. We release the resulting interaction and rating dataset, MathConverse. By analyzing MathConverse, we derive a taxonomy of human query behaviors and uncover that despite a generally positive correlation, there are notable instances of divergence between correctness and perceived helpfulness inLLMgenerations, among other findings. Further, we garner a more granular understanding of GPT-4 mathematical problemsolving through a series of case studies, contributed by experienced mathematicians.We conclude with actionable takeaways for ML practitioners and mathematicians: models that communicate uncertainty, respond well to user corrections, and can provide a concise rationale for their recommendations, may constitute better assistants. Humans should inspect LLM output carefully given their current shortcomings and potential for surprising fallibility.},
archivePrefix = {arXiv},
arxivId = {2306.01694},
author = {Collins, Katherine M. and Jiang, Albert Q. and Frieder, Simon and Wong, Lionel and Zilka, Miri and Bhatt, Umang and Lukasiewicz, Thomas and Wu, Yuhuai and Tenenbaum, Joshua B. and Hart, William and Gowers, Timothy and Li, Wenda and Weller, Adrian and Jamnik, Mateja},
doi = {10.1073/pnas.2318124121},
eprint = {2306.01694},
file = {:F\:/Medical 1/Paper 28.pdf:pdf},
issn = {10916490},
journal = {Proceedings of the National Academy of Sciences of the United States of America},
keywords = {AI,human-computer interaction,language models,theorem proving},
mendeley-groups = {000000},
number = {24},
pages = {1--11},
pmid = {38830100},
title = {{Evaluating language models for mathematics through interactions}},
volume = {121},
year = {2024}
}
@article{RadhaKrishnan2024,
abstract = {Drug–drug interactions (DDIs) present a significant health burden, compounded by clinician time constraints and poor patient health literacy. We assessed the ability of ChatGPT (generative artificial intelligence-based large language model) to predict DDIs in a real-world setting. Demographics, diagnoses and prescribed medicines for 120 hospitalized patients were input through three standardized prompts to ChatGPT version 3.5 and compared against pharmacist DDI evaluation to estimate diagnostic accuracy. Area under receiver operating characteristic and inter-rater reliability (Cohen's and Fleiss' kappa coefficients) were calculated. ChatGPT's responses differed based on prompt wording style, with higher sensitivity for prompts mentioning ‘drug interaction'. Confusion matrices displayed low true positive and high true negative rates, and there was minimal agreement between ChatGPT and pharmacists (Cohen's kappa values 0.077–0.143). Low sensitivity values suggest a lack of success in identifying DDIs by ChatGPT, and further development is required before it can reliably assess potential DDIs in real-world scenarios.},
author = {{Radha Krishnan}, Ramya Padmavathy and Hung, Euniss Hinyo and Ashford, Megan and Edillo, Clark Ethan and Gardner, Charlise and Hatrick, Hector Blake and Kim, Byungjun and Lai, Angel Wing Yan and Li, Xinran and Zhao, Yvonne Xinyi and Raubenheimer, Jacques Eugene},
doi = {10.1111/bcp.16275},
file = {:F\:/Medical 1/Paper 29.pdf:pdf},
issn = {13652125},
journal = {British Journal of Clinical Pharmacology},
keywords = {ChatGPT,artificial intelligence (AI),drug–drug interaction (DDI),large language model (LLM),patient health literacy},
mendeley-groups = {000000},
number = {June},
pages = {1--6},
title = {{Evaluating the capability of ChatGPT in predicting drug–drug interactions: Real-world evidence using hospitalized patient data}},
year = {2024}
}
@misc{lin2022teachingmodelsexpressuncertainty,
      title={Teaching Models to Express Their Uncertainty in Words}, 
      author={Stephanie Lin and Jacob Hilton and Owain Evans},
      year={2022},
      eprint={2205.14334},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2205.14334}, 
}

@article{Fan2024,
abstract = {Game theory, as an analytical tool, is frequently utilized to analyze human behavior in social science research. With the high alignment between the behavior of Large Language Models (LLMs) and humans, a promising research direction is to employ LLMs as substitutes for humans in game experiments, enabling social science research. However, despite numerous empirical researches on the combination of LLMs and game theory, the capability boundaries of LLMs in game theory remain unclear. In this research, we endeavor to systematically analyze LLMs in the context of game theory. Specifically, rationality, as the fundamental principle of game theory, serves as the metric for evaluating players' behavior — building a clear desire, refining belief about uncertainty, and taking optimal actions. Accordingly, we select three classical games (dictator game, Rock-Paper-Scissors, and ring-network game) to analyze to what extent LLMs can achieve rationality in these three aspects. The experimental results indicate that even the current state-of-the-art LLM (GPT-4) exhibits substantial disparities compared to humans in game theory. For instance, LLMs struggle to build desires based on uncommon preferences, fail to refine belief from many simple patterns, and may overlook or modify refined belief when taking actions. Therefore, we consider that introducing LLMs into game experiments in the field of social science should be approached with greater caution.},
archivePrefix = {arXiv},
arxivId = {2312.05488},
author = {Fan, Caoyun and Chen, Jindou and Jin, Yaohui and He, Hao},
doi = {10.1609/aaai.v38i16.29751},
eprint = {2312.05488},
file = {:F\:/Medical 1/Paper 33.pdf:pdf},
issn = {23743468},
journal = {Proceedings of the AAAI Conference on Artificial Intelligence},
keywords = {Game Theory and Economic Paradigms (GTEP): GTEP: Applications,Game Theory and Economic Paradigms (GTEP): GTEP: Game Theory,Natural Language Processing (NLP): NLP: (Large) Language Models},
mendeley-groups = {000000},
number = {16},
pages = {17960--17967},
title = {{Can Large Language Models Serve as Rational Players in Game Theory? A Systematic Analysis}},
volume = {38},
year = {2024}
}
@misc{lin2024generatingconfidenceuncertaintyquantification,
      title={Generating with Confidence: Uncertainty Quantification for Black-box Large Language Models}, 
      author={Zhen Lin and Shubhendu Trivedi and Jimeng Sun},
      year={2024},
      eprint={2305.19187},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2305.19187}, 
}
@misc{kadavath2022languagemodelsmostlyknow,
      title={Language Models (Mostly) Know What They Know}, 
      author={Saurav Kadavath and Tom Conerly and Amanda Askell and Tom Henighan and Dawn Drain and Ethan Perez and Nicholas Schiefer and Zac Hatfield-Dodds and Nova DasSarma and Eli Tran-Johnson and Scott Johnston and Sheer El-Showk and Andy Jones and Nelson Elhage and Tristan Hume and Anna Chen and Yuntao Bai and Sam Bowman and Stanislav Fort and Deep Ganguli and Danny Hernandez and Josh Jacobson and Jackson Kernion and Shauna Kravec and Liane Lovitt and Kamal Ndousse and Catherine Olsson and Sam Ringer and Dario Amodei and Tom Brown and Jack Clark and Nicholas Joseph and Ben Mann and Sam McCandlish and Chris Olah and Jared Kaplan},
      year={2022},
      eprint={2207.05221},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2207.05221}, 
}

@misc{chen2023quantifyinguncertaintyanswerslanguage,
      title={Quantifying Uncertainty in Answers from any Language Model and Enhancing their Trustworthiness}, 
      author={Jiuhai Chen and Jonas Mueller},
      year={2023},
      eprint={2308.16175},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2308.16175}, 
}

@article{Sen2024,
abstract = {Workers, especially those involved in jobs requiring extended standing or repetitive movements, often face significant health challenges due to Musculoskeletal Disorders (MSDs). To mitigate MSD risks, enhancing workplace ergonomics is vital, which includes forecasting long-term employee postures, educating workers about related occupational health risks, and offering relevant recommendations. However, research gaps remain, such as the lack of a sustainable AI/ML pipeline that combines sensor-based, uncertainty-aware posture prediction with large language models for natural language communication of occupational health risks and recommendations. We introduce ERG-AI, a machine learning pipeline designed to predict extended worker postures using data from multiple wearable sensors. Alongside providing posture prediction and uncertainty estimates, ERG-AI also provides personalized health risk assessments and recommendations by generating prompts based on its performance and prompting Large Language Model (LLM) APIs, like GPT-4, to obtain user-friendly output. We used the Digital Worker Goldicare dataset to assess ERG-AI, which includes data from 114 home care workers who wore five tri-axial accelerometers in various bodily positions for a cumulative 2913 hours. The evaluation focused on the quality of posture prediction under uncertainty, energy consumption and carbon footprint of ERG-AI and the effectiveness of personalized recommendations rendered in easy-to-understand language.},
author = {Sen, Sagar and Gonzalez, Victor and Husom, Erik Johannes and Tverdal, Simeon and Tokas, Shukun and Tj{\o}svoll, Svein O.},
doi = {10.1007/s10489-024-05796-1},
file = {:F\:/Medical 1/Paper 39.pdf:pdf},
issn = {15737497},
journal = {Applied Intelligence},
keywords = {Human ergonomics,Large language models,Machine learning pipeline,Musculoskeletal disorders,Uncertainty estimation},
mendeley-groups = {000000},
pages = {12128--12155},
title = {{ERG-AI: enhancing occupational ergonomics with uncertainty-aware ML and LLM feedback}},
year = {2024}
}
@article{Manakul2023,
abstract = {Generative Large Language Models (LLMs) such as GPT-3 are capable of generating highly fluent responses to a wide variety of user prompts. However, LLMs are known to hallucinate facts and make non-factual statements which can undermine trust in their output. Existing fact-checking approaches either require access to the output probability distribution (which may not be available for systems such as ChatGPT) or external databases that are interfaced via separate, often complex, modules. In this work, we propose "SelfCheckGPT", a simple sampling-based approach that can be used to fact-check the responses of black-box models in a zero-resource fashion, i.e. without an external database. SelfCheckGPT leverages the simple idea that if an LLM has knowledge of a given concept, sampled responses are likely to be similar and contain consistent facts. However, for hallucinated facts, stochastically sampled responses are likely to diverge and contradict one another. We investigate this approach by using GPT-3 to generate passages about individuals from the WikiBio dataset, and manually annotate the factuality of the generated passages. We demonstrate that SelfCheckGPT can: i) detect non-factual and factual sentences; and ii) rank passages in terms of factuality. We compare our approach to several baselines and show that our approach has considerably higher AUC-PR scores in sentence-level hallucination detection and higher correlation scores in passage-level factuality assessment compared to grey-box methods.},
archivePrefix = {arXiv},
arxivId = {2303.08896},
author = {Manakul, Potsawee and Liusie, Adian and Gales, Mark J.F.},
doi = {10.18653/v1/2023.emnlp-main.557},
eprint = {2303.08896},
file = {:F\:/Medical 1/Paper 40.pdf:pdf},
isbn = {9798891760608},
journal = {EMNLP 2023 - 2023 Conference on Empirical Methods in Natural Language Processing, Proceedings},
mendeley-groups = {000000},
pages = {9004--9017},
title = {{SELFCHECKGPT: Zero-Resource Black-Box Hallucination Detection for Generative Large Language Models}},
year = {2023}
}
@article{Kuhn2023,
abstract = {We introduce a method to measure uncertainty in large language models. For tasks like question answering, it is essential to know when we can trust the natural language outputs of foundation models. We show that measuring uncertainty in natural language is challenging because of 'semantic equivalence'-different sentences can mean the same thing. To overcome these challenges we introduce semantic entropy-an entropy which incorporates linguistic invariances created by shared meanings. Our method is unsupervised, uses only a single model, and requires no modifications to 'off-the-shelf' language models. In comprehensive ablation studies we show that the semantic entropy is more predictive of model accuracy on question answering data sets than comparable baselines.},
archivePrefix = {arXiv},
arxivId = {2302.09664},
author = {Kuhn, Lorenz and Gal, Yarin and Farquhar, Sebastian},
eprint = {2302.09664},
file = {:F\:/Medical 1/Paper 41.pdf:pdf},
journal = {11th International Conference on Learning Representations, ICLR 2023},
mendeley-groups = {000000},
pages = {1--19},
title = {{Semantic Uncertainty: Linguistic Invariances for Uncertainty Estimation in Natural Language Generation}},
year = {2023}
}

@misc{peng2024uncertaintyawareexplainablerecommendationlarge,
      title={Uncertainty-Aware Explainable Recommendation with Large Language Models}, 
      author={Yicui Peng and Hao Chen and Chingsheng Lin and Guo Huang and Jinrong Hu and Hui Guo and Bin Kong and Shu Hu and Xi Wu and Xin Wang},
      year={2024},
      eprint={2402.03366},
      archivePrefix={arXiv},
      primaryClass={cs.IR},
      url={https://arxiv.org/abs/2402.03366}, 
}

@article{Savage2025,
  author    = {Thomas Savage and John Wang and Robert Gallo and Abdessalem Boukil and Vishwesh Patel and Seyed Amir Ahmad Safavi-Naini and Ali Soroush and Jonathan H. Chen},
  title     = {Large language model uncertainty proxies: discrimination and calibration for medical diagnosis and treatment},
  journal   = {Journal of the American Medical Informatics Association},
  volume    = {32},
  number    = {1},
  pages     = {139--149},
  year      = {2025},
  month     = jan,
  doi       = {10.1093/jamia/ocae254},
  url       = {https://doi.org/10.1093/jamia/ocae254}
}


@article{Lin2023,
abstract = {Deep learning methods have achieved an excellent performance in medical image segmentation. However, the practical application of deep learning-based segmentation models is limited in clinical settings due to the lack of reliable information about the segmentation quality. In this article, we propose a novel quality control algorithm based on fuzzy uncertainty to quantify the quality of the predicted segmentation results as part of the model inference process. First, test-time augmentation and Monte Carlo dropout are applied simultaneously to capture both the data and model uncertainties of the trained image segmentation model. Then, a fuzzy set is generated to describe the captured uncertainty with the assistance of the linear Euclidean distance transform algorithm. Finally, the fuzziness of the generated fuzzy set is adopted to calculate an image-level segmentation uncertainty and, therefore, to infer the segmentation quality. Extensive experiments using five medical image segmentation applications on the detection of skin lesion, nuclei, lung, breast, and cell are conducted to evaluate the proposed algorithm. The experimental results show that the estimated image-level uncertainties using the proposed method have strong correlations with the segmentation qualities measured by the Dice coefficient, resulting in absolute Pearson correlation coefficients of 0.60-0.92. Our method outperforms other five state-of-the-art quality control methods in classifying the segmentation results into good and poor quality groups (area under the receiver operating curve of greater than 0.92, while other methods are below 0.85).},
author = {Lin, Qiao and Chen, Xin and Chen, Chao and Garibaldi, Jonathan M.},
doi = {10.1109/TFUZZ.2022.3228332},
file = {:C\:/Users/RHfix/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Lin et al. - 2023 - A Novel Quality Control Algorithm for Medical Image Segmentation Based on Fuzzy Uncertainty.pdf:pdf},
issn = {19410034},
journal = {IEEE Transactions on Fuzzy Systems},
keywords = {Data uncertainty,fuzzy sets,model uncertainty,quality control,semantic segmentation},
mendeley-groups = {Certainty},
number = {8},
pages = {2532--2544},
publisher = {IEEE},
title = {{A Novel Quality Control Algorithm for Medical Image Segmentation Based on Fuzzy Uncertainty}},
volume = {31},
year = {2023}
}


@article{Duran2021,
abstract = {The use of black box algorithms in medicine has raised scholarly concerns due to their opaqueness and lack of trustworthiness. Concerns about potential bias, accountability and responsibility, patient autonomy and compromised trust transpire with black box algorithms. These worries connect epistemic concerns with normative issues. In this paper, we outline that black box algorithms are less problematic for epistemic reasons than many scholars seem to believe. By outlining that more transparency in algorithms is not always necessary, and by explaining that computational processes are indeed methodologically opaque to humans, we argue that the reliability of algorithms provides reasons for trusting the outcomes of medical artificial intelligence (AI). To this end, we explain how computational reliabilism, which does not require transparency and supports the reliability of algorithms, justifies the belief that results of medical AI are to be trusted. We also argue that several ethical concerns remain with black box algorithms, even when the results are trustworthy. Having justified knowledge from reliable indicators is, therefore, necessary but not sufficient for normatively justifying physicians to act. This means that deliberation about the results of reliable algorithms is required to find out what is a desirable action. Thus understood, we argue that such challenges should not dismiss the use of black box algorithms altogether but should inform the way in which these algorithms are designed and implemented. When physicians are trained to acquire the necessary skills and expertise, and collaborate with medical informatics and data scientists, black box algorithms can contribute to improving medical care.},
author = {Dur{\'{a}}n, Juan Manuel and Jongsma, Karin Rolanda},
doi = {10.1136/medethics-2020-106820},
file = {:C\:/Users/RHfix/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Dur{\'{a}}n, Jongsma - 2021 - Who is afraid of black box algorithms On the epistemological and ethical basis of trust in medical AI.pdf:pdf},
issn = {14734257},
journal = {Journal of Medical Ethics},
keywords = {Information technology,applied and professional ethics,clinical ethics,philosophical ethics,philosophy of medicine},
mendeley-groups = {Certainty},
number = {5},
pages = {329--335},
title = {{Who is afraid of black box algorithms? On the epistemological and ethical basis of trust in medical AI}},
volume = {47},
year = {2021}
}
@misc{donakanti2024reimaginingselfadaptationagelarge,
      title={Reimagining Self-Adaptation in the Age of Large Language Models}, 
      author={Raghav Donakanti and Prakhar Jain and Shubham Kulkarni and Karthik Vaidhyanathan},
      year={2024},
      eprint={2404.09866},
      archivePrefix={arXiv},
      primaryClass={cs.SE},
      url={https://arxiv.org/abs/2404.09866}, 
}

@article{Lin2023,
abstract = {Deep learning methods have achieved an excellent performance in medical image segmentation. However, the practical application of deep learning-based segmentation models is limited in clinical settings due to the lack of reliable information about the segmentation quality. In this article, we propose a novel quality control algorithm based on fuzzy uncertainty to quantify the quality of the predicted segmentation results as part of the model inference process. First, test-time augmentation and Monte Carlo dropout are applied simultaneously to capture both the data and model uncertainties of the trained image segmentation model. Then, a fuzzy set is generated to describe the captured uncertainty with the assistance of the linear Euclidean distance transform algorithm. Finally, the fuzziness of the generated fuzzy set is adopted to calculate an image-level segmentation uncertainty and, therefore, to infer the segmentation quality. Extensive experiments using five medical image segmentation applications on the detection of skin lesion, nuclei, lung, breast, and cell are conducted to evaluate the proposed algorithm. The experimental results show that the estimated image-level uncertainties using the proposed method have strong correlations with the segmentation qualities measured by the Dice coefficient, resulting in absolute Pearson correlation coefficients of 0.60-0.92. Our method outperforms other five state-of-the-art quality control methods in classifying the segmentation results into good and poor quality groups (area under the receiver operating curve of greater than 0.92, while other methods are below 0.85).},
author = {Lin, Qiao and Chen, Xin and Chen, Chao and Garibaldi, Jonathan M.},
doi = {10.1109/TFUZZ.2022.3228332},
file = {:C\:/Users/RHfix/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/Lin et al. - 2023 - A Novel Quality Control Algorithm for Medical Image Segmentation Based on Fuzzy Uncertainty.pdf:pdf},
issn = {19410034},
journal = {IEEE Transactions on Fuzzy Systems},
keywords = {Data uncertainty,fuzzy sets,model uncertainty,quality control,semantic segmentation},
mendeley-groups = {Certainty},
number = {8},
pages = {2532--2544},
publisher = {IEEE},
title = {{A Novel Quality Control Algorithm for Medical Image Segmentation Based on Fuzzy Uncertainty}},
volume = {31},
year = {2023}
}


@article{McCradden2023,
abstract = {Researchers are studying how artificial intelligence (AI) can be used to better detect, prognosticate and subgroup diseases. The idea that AI might advance medicine's understanding of biological categories of psychiatric disorders, as well as provide better treatments, is appealing given the historical challenges with prediction, diagnosis and treatment in psychiatry. Given the power of AI to analyse vast amounts of information, some clinicians may feel obligated to align their clinical judgements with the outputs of the AI system. However, a potential epistemic privileging of AI in clinical judgements may lead to unintended consequences that could negatively affect patient treatment, well-being and rights. The implications are also relevant to precision medicine, digital twin technologies and predictive analytics generally. We propose that a commitment to epistemic humility can help promote judicious clinical decision-making at the interface of big data and AI in psychiatry.},
author = {McCradden, Melissa and Hui, Katrina and Buchman, Daniel Z.},
doi = {10.1136/jme-2022-108447},
file = {:C\:/Users/RHfix/AppData/Local/Mendeley Ltd./Mendeley Desktop/Downloaded/McCradden, Hui, Buchman - 2023 - Evidence, ethics and the promise of artificial intelligence in psychiatry.pdf:pdf},
issn = {14734257},
journal = {Journal of Medical Ethics},
keywords = {Decision Making,Ethics- Medical,Mental Health,Psychiatry},
mendeley-groups = {Certainty},
number = {8},
pages = {573--579},
pmid = {36581457},
title = {{Evidence, ethics and the promise of artificial intelligence in psychiatry}},
volume = {49},
year = {2023}
}


@article{kahneman1979prospect,
  title={Prospect theory: An analysis of decision under risk},
  author={Kahneman, Daniel and Tversky, Amos},
  journal={Econometrica},
  volume={47},
  number={2},
  pages={263--291},
  year={1979},
  publisher={JSTOR}
}
@inproceedings{harsha2024quantifying,
  title={Quantifying Uncertainty in Natural Language Explanations of Large Language Models},
  author={Harsha Tanneru and others},
  booktitle={Proceedings of Machine Learning Research (PMLR)},
  year={2024},
  url={https://proceedings.mlr.press/v238/harsha-tanneru24a.html}
}

@article{rethinking2024uncertainty,
  title={Rethinking the Uncertainty: A Critical Review and Analysis in the Era of Large Language Models},
  author={Author Unknown},
  journal={arXiv preprint arXiv:2410.20199},
  year={2024},
  url={https://arxiv.org/abs/2410.20199}
}

@article{Xiao2022,
  author    = {Zhiyong Xiao and Yixin Su and Zhaohong Deng and Weidong Zhang},
  title     = {Efficient Combination of CNN and Transformer for Dual-Teacher Uncertainty-guided Semi-supervised Medical Image Segmentation},
  journal   = {Computer Methods and Programs in Biomedicine},
  volume    = {226},
  year      = {2022},
  month     = nov,
  doi       = {10.1016/j.cmpb.2022.107099},
  issn      = {1872-7565},
  pmid      = {36116398},
  publisher = {Elsevier Ireland Ltd},
  keywords  = {Deep learning, Image segmentation, Magnetic resonance imaging (MRI), Semi-supervised learning, Transformer}
}

@article{Yan2023,
   abstract = {Background: Cardiovascular disease is one of the leading causes of death worldwide. However, according to studies, 90\% of cardiovascular diseases can be prevented. Cardiovascular function parameters are an important basis for the diagnosis of cardiovascular diseases. The pulse wave also contains a wealth of physiological and pathological information, which can reflect the trend of cardiac function parameters at an early stage, so the measurement and analysis of the pulse wave signal becomes more and more important. The wearable pulse signal acquisition device has gradually become a new trend. In the mobile health scenario, convenient use is the prerequisite for long-term and rapid health monitoring. The data containing diverse pulse wave signals is the basis for obtaining more comprehensive and accurate human physiopathological information. Accurate data analysis and processing is the key to realizing the important goal of cardiovascular health monitoring. Objective: Based on the concept of mobile health care, wearable devices are developed to obtain physiological signals. The zero-dimensional model and the optimization algorithm are combined to complete the uncertainty quantification of the microcirculation parameters. Then, a feature set containing the cardiovasvular parameters can be constructed. The machine learning algorithm can be used to build a model that can accurately realize cardiovascular disease identification. Methods: This paper adopts laboratory-developed equipment to acquire the wrist pulse wave and fingertip volume pulse wave. A total of 323 samples were collected from healthy populations, hypertensive patients and patients with coronary heart disease (CHD). The pulse blood flow model in fingertip microcirculation is established, and the uncertainty quantification of model parameters is completed based on slime mold algorithm (SMA). After comparing and analyzing the performance of four algorithms on pulse wave classification, the identification model of cardiovascular diseases is established based on the microcirculatory characteristic parameter set and random forest algorithm (RF). Results: RF showed good classification performance among the four classification algorithms. The identification accuracy of the model built on the microcirculatory characteristic parameter set and RF algorithm all reached more than 88\%. The highest recognition accuracy was 95.51\% for coronary heart disease samples, 92.11\% for healthy samples, and 88.55\% for hypertensive samples. It can be seen that the model based on RF algorithm has a good ability to distinguish the characteristic parameters in different cardiovascular health states. Conclusions: The wearable device designed in this paper can facilitate the daily health monitoring of cardiovascular disease. By using the combination of the physical model and machine learning model, the uncertainty quantification of microcirculation parameters and the identification of cardiovascular disease was finally completed. The recognition model based on machine learning provides a new idea and method for the research of cardiovascular health monitoring through pulse waves.},
   author = {Jianjun Yan and Shiyu Cai and Xianglei Cai and Guangyao Zhu and Wei Zhou and Rui Guo and Haixia Yan and Yiqin Wang},
   doi = {10.1016/j.cmpb.2023.107674},
   issn = {18727565},
   journal = {Computer Methods and Programs in Biomedicine},
   keywords = {Cardiovascular disease recognition,Pulse wave,Random forest algorithm,Slime mold algorithm,Uncertainty quantification},
   month = {10},
   pmid = {37343374},
   publisher = {Elsevier Ireland Ltd},
   title = {Uncertainty quantification of microcirculatory characteristic parameters for recognition of cardiovascular diseases},
   volume = {240},
   year = {2023},
}
@article{Silk2022,
   abstract = {Scientific advice to the UK government throughout the COVID-19 pandemic has been informed by ensembles of epidemiological models provided by members of the Scientific Pandemic Influenza group on Modelling. Among other applications, the model ensembles have been used to forecast daily incidence, deaths and hospitalizations. The models differ in approach (e.g. deterministic or agent-based) and in assumptions made about the disease and population. These differences capture genuine uncertainty in the understanding of disease dynamics and in the choice of simplifying assumptions underpinning the model. Although analyses of multi-model ensembles can be logistically challenging when time-frames are short, accounting for structural uncertainty can improve accuracy and reduce the risk of over-confidence in predictions. In this study, we compare the performance of various ensemble methods to combine short-term (14-day) COVID-19 forecasts within the context of the pandemic response. We address practical issues around the availability of model predictions and make some initial proposals to address the shortcomings of standard methods in this challenging situation.},
   author = {Daniel S. Silk and Veronica E. Bowman and Daria Semochkina and Ursula Dalrymple and Dave C. Woods},
   doi = {10.1177/09622802221109523},
   issn = {14770334},
   issue = {9},
   journal = {Statistical Methods in Medical Research},
   keywords = {COVID-19,disease forecasting,model combination,model stacking,uncertainty quantification},
   month = {9},
   pages = {1778-1789},
   pmid = {35799481},
   publisher = {SAGE Publications Ltd},
   title = {Uncertainty quantification for epidemiological forecasts of COVID-19 through combinations of model predictions},
   volume = {31},
   year = {2022},
}
@article{Jones2025,
   abstract = {Computational models that can predict growth and remodeling of the heart could have important clinical applications. However, the time it takes to calibrate and run current models while considering data uncertainty and variability makes them impractical for routine clinical use. This study aims to address this need by creating a computational framework to efficiently predict cardiac growth probability. We utilized a biophysics model to rapidly simulate cardiac growth following mitral valve regurgitation (MVR). Here we developed a two-tiered Bayesian History Matching approach augmented with Gaussian process emulators for efficient calibration of model parameters to align with growth outcomes within a 95\% confidence interval. We first generated a synthetic data set to assess the accuracy of our framework, and the effect of changes in data uncertainty on growth predictions. We then calibrated our model to match baseline and chronic canine MVR data and used an independent data set to successfully validate the ability of our calibrated model to accurately predict cardiac growth probability. The combined biophysics and machine learning modeling framework we proposed in this study can be easily translated to predict patient-specific cardiac growth.},
   author = {Clara E. Jones and Pim J.A. Oomen},
   doi = {10.1016/j.compbiomed.2024.109323},
   issn = {18790534},
   journal = {Computers in Biology and Medicine},
   keywords = {Biophysics modeling,Cardiac mechanics,Growth \& remodeling,Machine learning,Mitral regurgitation},
   month = {1},
   publisher = {Elsevier Ltd},
   title = {Synergistic biophysics and machine learning modeling to rapidly predict cardiac growth probability},
   volume = {184},
   year = {2025},
}


@ARTICLE{Wickstrøm2021,
  author={Wickstrøm, Kristoffer and Mikalsen, Karl Øyvind and Kampffmeyer, Michael and Revhaug, Arthur and Jenssen, Robert},
  journal={IEEE Journal of Biomedical and Health Informatics}, 
  title={Uncertainty-Aware Deep Ensembles for Reliable and Explainable Predictions of Clinical Time Series}, 
  year={2021},
  volume={25},
  number={7},
  pages={2435-2444},
  keywords={Time series analysis;Uncertainty;Task analysis;Predictive models;Computational modeling;Bioinformatics;Biomedical measurement;Deep learning;ensembles;interpretability;time series;uncertainty},
  doi={10.1109/JBHI.2020.3042637},
}

@article{Molchanova2025,
   abstract = {This paper explores uncertainty quantification (UQ) as an indicator of the trustworthiness of automated deep-learning (DL) tools in the context of white matter lesion (WML) segmentation from magnetic resonance imaging (MRI) scans of multiple sclerosis (MS) patients. Our study focuses on two principal aspects of uncertainty in structured output segmentation tasks. First, we postulate that a reliable uncertainty measure should indicate predictions likely to be incorrect with high uncertainty values. Second, we investigate the merit of quantifying uncertainty at different anatomical scales (voxel, lesion, or patient). We hypothesize that uncertainty at each scale is related to specific types of errors. Our study aims to confirm this relationship by conducting separate analyses for in-domain and out-of-domain settings. Our primary methodological contributions are (i) the development of novel measures for quantifying uncertainty at lesion and patient scales, derived from structural prediction discrepancies, and (ii) the extension of an error retention curve analysis framework to facilitate the evaluation of UQ performance at both lesion and patient scales. The results from a multi-centric MRI dataset of 444 patients demonstrate that our proposed measures more effectively capture model errors at the lesion and patient scales compared to measures that average voxel-scale uncertainty values. We provide the UQ protocols code at https://github.com/Medical-Image-Analysis-Laboratory/MSWMLuncs.},
   author = {Nataliia Molchanova and Vatsal Raina and Andrey Malinin and Francesco La Rosa and Adrien Depeursinge and Mark Gales and Cristina Granziera and Henning Müller and Mara Graziani and Meritxell Bach Cuadra},
   doi = {10.1016/j.compbiomed.2024.109336},
   issn = {18790534},
   journal = {Computers in Biology and Medicine},
   keywords = {Deep learning,Instancescale uncertainty,Magnetic resonance imaging,Multiple sclerosis,Patientscale uncertainty,Uncertainty quantification,White matter lesion segmentation},
   month = {1},
   publisher = {Elsevier Ltd},
   title = {Structural-based uncertainty in deep learning across anatomical scales: Analysis in white matter lesion segmentation},
   volume = {184},
   year = {2025},
}


@article{Bahaj2025,
   abstract = {Objective: This study aims at automatically quantifying and modelling the uncertainty of facts in biomedical knowledge graphs (BKGs) based on their textual supporting evidence using deep learning techniques. Materials and Methods: A sentence transformer is employed to extract deep features of sentences used to classify sentence factuality using a naive Bayes classifier. For each fact and its supporting evidence in a source KG, the deep feature extractor and the classifier are used to quantify the factuality of each sentence which are then transformed to numerical values in [0,1] before being averaged to get the confidence score of the fact. Results: The fact classification feature extractor enhances the separability of classes in the embedding space. This helped the fact classification model to achieve a better performance than existing factuality classification with hand-crafted features. Uncertainty quantification and modelling were demonstrated on SemMedDB by creating USemMedDB, showing KGB2U's ability to process large BKGs. A subset of USemMedDB facts is modelled to demonstrate the correlation between the structure of the uncertain BKG and the confidence scores. The best-trained model is used to predict confidence scores of existing and unseen facts. The top-ranked unseen facts were grounded using scientific evidence showing KGB2U's ability to discover new knowledge. Conclusion: Supporting literature of BKG facts can be used to automatically quantify their uncertainty. Additionally, the resulting uncertain biomedical KGs can be used for knowledge discovery. BKG2U interface and source code are available at http://biofunk.datanets.org/ and https://github.com/BahajAdil/KBG2U respectively.},
   author = {Adil Bahaj and Mounir Ghogho},
   doi = {10.1016/j.compbiomed.2024.109355},
   issn = {18790534},
   journal = {Computers in Biology and Medicine},
   keywords = {Biomedical knowledge graphs,Knowledge graph embedding,Precision medicine,Uncertain knowledge graphs},
   month = {1},
   publisher = {Elsevier Ltd},
   title = {A step towards quantifying, modelling and exploring uncertainty in biomedical knowledge graphs},
   volume = {184},
   year = {2025},
}

@article{Flaig2022,
   abstract = {Background: Recent epidemics and measures taken to control them-through vaccination or other actions-have highlighted the role and importance of uncertainty in public health. There is generally a trade-off between information collection and other uses of resources. Whether this trade-off is solved explicitly or implicitly, the concept of value of information is central in order to inform policy makers in an uncertain environment. Method: We use a deterministic SIR disease emergence and transmission model with vaccination that can be administered as one or two doses. The disease parameters and vaccine characteristics are uncertain. We study the trade-offs between information acquisition and two other measures: bringing vaccination forward, and acquiring more vaccine doses. To do this, we quantify the expected value of perfect information (EVPI) under different constraints faced by public health authorities, i.e. the time of the vaccination campaign implementation and the number of vaccine doses available. Results: We discuss the appropriateness of different responses under uncertainty. We show that in some cases, vaccinating later or with less vaccine doses but more information about the epidemic and the efficacy of control strategies may bring better results than vaccinating earlier or with more doses and less information respectively. Conclusion: In the present methodological paper, we show in an abstract setting how clearly defining and treating the trade-off between information acquisition and the relaxation of constraints can improve public health decision making.},
   author = {Julien Flaig and Nicolas Houy},
   doi = {10.1177/0272989X231158295ï},
   issue = {3},
   journal = {Medical Decision Making},
   pages = {350-361},
   title = {Optimal Epidemic Control under Uncertainty: Tradeoffs between Information Collection and Other Actions Optimal epidemic control under uncertainty: trade-offs between information collection and other actions},
   volume = {2023},
   url = {https://doi.org/10.1101/2022.03.28.22273039},
   year = {2022},
}

@misc{Meyer2021,
   abstract = {Various convolutional neural network (CNN) based concepts have been introduced for the prostate's automatic segmentation and its coarse subdivision into transition zone (TZ) and peripheral zone (PZ). However, when targeting a fine-grained segmentation of TZ, PZ, distal prostatic urethra (DPU) and the anterior fibromuscular stroma (AFS), the task becomes more challenging and has not yet been solved at the level of human performance. One reason might be the insufficient amount of labeled data for supervised training. Therefore, we propose to apply a semi-supervised learning (SSL) technique named uncertainty-aware temporal self-learning (UATS) to overcome the expensive and time-consuming manual ground truth labeling. We combine the SSL techniques temporal ensembling and uncertainty-guided self-learning to benefit from unlabeled images, which are often readily available. Our method significantly outperforms the supervised baseline and obtained a Dice coefficient (DC) TZ, PZ, DPU and AFS, respectively. The obtained results are in the range of human inter-rater performance for all structures. Moreover, we investigate the method's robustness against noise and demonstrate the generalization capability for varying ratios of labeled data and on other challenging tasks, namely the hippocampus and skin lesion segmentation. UATS achieved superiority segmentation quality compared to the supervised baseline, particularly for minimal amounts of labeled data.},
   author = {Anneke Meyer and Suhita Ghosh and Daniel Schindele and Martin Schostak and Sebastian Stober and Christian Hansen and Marko Rak},
   keywords = {Biomedical Segmentation,Prostate Zones,Semi-Supervised Deep Learning},
   title = {Uncertainty-Aware Temporal Self-Learning (UATS): Semi-Supervised Learning for Segmentation of Prostate Zones and Beyond},
   year = {2021},
}


@article{Salvador2023,
  author    = {Salvador, M. and Regazzoni, F. and Dede', L. and Quarteroni, A.},
  title     = {Fast and robust parameter estimation with uncertainty quantification for the cardiac function},
  journal   = {Computer Methods and Programs in Biomedicine},
  volume    = {231},
  pages     = {107402},
  year      = {2023},
  month     = apr,
  doi       = {10.1016/j.cmpb.2023.107402},
  pmid      = {36773593},
  note      = {Epub 2023 Feb 4}
}

@article{Du2025,
   abstract = {Automatic segmentation of polyps from colonoscopy images plays a critical role in the early diagnosis and treatment of colorectal cancer. Nevertheless, some bottlenecks still exist. In our previous work, we mainly focused on polyps with intra-class inconsistency and low contrast, using ICGNet to solve them. Due to the different equipment, specific locations and properties of polyps, the color distribution of the collected images is inconsistent. ICGNet was designed primarily with reverse-contour guide information and local–global context information, ignoring this inconsistent color distribution, which leads to overfitting problems and makes it difficult to focus only on beneficial image content. In addition, a trustworthy segmentation model should not only produce high-precision results but also provide a measure of uncertainty to accompany its predictions so that physicians can make informed decisions. However, ICGNet only gives the segmentation result and lacks the uncertainty measure. To cope with these novel bottlenecks, we further extend the original ICGNet to a comprehensive and effective network (UM-Net) with two main contributions that have been proved by experiments to have substantial practical value. Firstly, we employ a color transfer operation to weaken the relationship between color and polyps, making the model more concerned with the shape of the polyps. Secondly, we provide the uncertainty to represent the reliability of the segmentation results and use variance to rectify uncertainty. Our improved method is evaluated on five polyp datasets, which shows competitive results compared to other advanced methods in both learning ability and generalization capability. The source code is available at https://github.com/dxqllp/UM-Net.},
   author = {Xiuquan Du and Xuebin Xu and Jiajia Chen and Xuejun Zhang and Lei Li and Heng Liu and Shuo Li},
   doi = {10.1016/j.media.2024.103347},
   issn = {13618423},
   journal = {Medical Image Analysis},
   keywords = {Colonoscopy image,Color transfer,Polyp segmentation,Uncertainty},
   month = {1},
   publisher = {Elsevier B.V.},
   title = {UM-Net: Rethinking ICGNet for polyp segmentation with uncertainty modeling},
   volume = {99},
   year = {2025},
}

@article{Koume2025,
   abstract = {Objective: A major concern for cancer survivors after treatment is the Fear of Cancer Recurrence (FCR), which is the fear that cancer will reappear or progress. This fear can be exacerbated by medical uncertainty about the future, leading to harmful obsession and having a negative impact on quality of life. This study aims to develop a predictive Machine Learning (ML) model using healthcare reimbursement data to better predict FCR and understand the factors influencing FCR in women with breast cancer five years after their diagnosis. Materials and Methods: We used data from the VICAN (VIe après le CANcer) survey to propose an interpretable model to identify patients at risk of developing clinical FCR. The reimbursement data for each patient were analyzed beyond the first two years of treatment, excluding the initial phase influenced by the cancer curative therapeutic process. Data experiments were conducted, including the use of algorithms such as Random Forest, Support Vector Machines, Gradient Boosting, eXtreme Gradient Boosting, and Multilayer Perceptron. The AUC was used to choose the optimal model. Results: The dataset is composed of 918 patients classified regarding FCR. The experimental design incorporated classification levels of medications, biological and medical procedures. Subsequently, data was generated for two experiments, facilitating examination at the ultimate healthcare classification level in Experiment 1, while Experiment 2 targeted the penultimate classification level. Overall, the best-performing model achieved an AUC of 66\% This demonstrates some effectiveness of the algorithms in detecting patients at risk of developing clinical FCR and encourages further investigations to enhance the model's performance and assess its generalizability. Conclusion: ML applied to reimbursement data has shown promise in predicting FCR, aiding in the identification of patients at risk of developing it. The results pave the way for personalized prevention and intervention strategies, representing a significant advancement in postcancer care focusing on the needs of survivors.},
   author = {Mamoudou Koume and Lorène Seguin and Julien Mancini and Marc Karim Bendiane and Anne Déborah Bouhnik and Raquel Urena},
   doi = {10.1016/j.ijmedinf.2024.105705},
   issn = {18728243},
   journal = {International Journal of Medical Informatics},
   keywords = {Breast cancer,Fear of cancer recurrence,Healthcare reimbursement data,Machine learning},
   month = {1},
   publisher = {Elsevier Ireland Ltd},
   title = {Predicting Fear of Breast Cancer Recurrence in women five years after diagnosis using Machine Learning and healthcare reimbursement data from the French nationwide VICAN survey},
   volume = {193},
   year = {2025},
}

@misc{Dimitriou2023,
   abstract = { The validation of mathematical models of tumour growth is frequently hampered by the lack of sufficient experimental data, resulting in qualitative rather than quantitative studies. Recent approaches to this problem have attempted to extract information about tumour growth by integrating multiscale experimental measurements, such as longitudinal cell counts and gene expression data. In the present study, we investigated the performance of several mathematical models of tumour growth, including classical logistic, fractional and novel multiscale models, in terms of quantifying in-vitro tumour growth in the presence and absence of therapy. We further examined the effect of genes associated with changes in chemosensitivity in cell death rates. State-of-the-art Bayesian inference, likelihood maximisation and uncertainty quantification techniques allowed a thorough evaluation of model performance. The results suggest that the classical single-cell population model (SCPM) was the best fit for the untreated and low-dose treatment conditions, while the multiscale model with a cell death rate symmetric with the expression profile of OCT4 (SymSCPM) yielded the best fit for the high-dose treatment data. Further identifiability analysis showed that the multiscale model was both structurally and practically identifiable under the condition of known OCT4 expression profiles. Overall, the present study demonstrates that model performance can be improved by incorporating multiscale measurements of tumour growth. },
   author = {Nikolaos M. Dimitriou and Ece Demirag and Katerina Strati and Georgios D. Mitsis},
   doi = {10.1101/2023.04.12.536622},
   institution = {bioRxiv},
   month = {4},
   title = {A calibration and uncertainty quantification analysis of classical, fractional and multiscale logistic models of tumour growth},
   url = {http://biorxiv.org/lookup/doi/10.1101/2023.04.12.536622},
   year = {2023},
}

@article{Fazekas2023,
  author    = {Fazekas, B. and Lachinov, D. and Aresta, G. and Mai, J. and Schmidt-Erfurth, U. and Bogunovic, H.},
  title     = {Segmentation of Bruch's Membrane in Retinal OCT With AMD Using Anatomical Priors and Uncertainty Quantification},
  journal   = {IEEE Journal of Biomedical and Health Informatics},
  volume    = {27},
  number    = {1},
  pages     = {41--52},
  year      = {2023},
  month     = jan,
  doi       = {10.1109/JBHI.2022.3217962},
  pmid      = {36306300},
  note      = {Epub 2023 Jan 4}
}



@article{Bhutto2024,
  author    = {Bhutto, D. F. and Zhu, B. and Liu, J. Z. and Koonjoo, N. and Li, H. B. and Rosen, B. R. and Rosen, M. S.},
  title     = {Uncertainty Estimation and Out-of-Distribution Detection for Deep Learning-Based Image Reconstruction Using the Local Lipschitz},
  journal   = {IEEE Journal of Biomedical and Health Informatics},
  year      = {2024},
  volume    = {28},
  number    = {9},
  pages     = {5422--5434},
  doi       = {10.1109/JBHI.2024.3404883},
  note      = {Epub 2024 Sep 5},
  pmid      = {38787662}
}

@article{Khawaled2024,
  author    = {Khawaled, S. and Freiman, M.},
  title     = {NPB-REC: A non-parametric Bayesian deep-learning approach for undersampled MRI reconstruction with uncertainty estimation},
  journal   = {Artificial Intelligence in Medicine},
  volume    = {149},
  pages     = {102798},
  year      = {2024},
  month     = mar,
  doi       = {10.1016/j.artmed.2024.102798},
  note      = {Epub 2024 Feb 5},
  pmid      = {38462289}
}


@article{Campos2023,
   abstract = {Introduction: Family members of patients admitted to an Intensive Care Unit present high uncertainty level due to not knowing what is happening and to not having clear details about the related events; therefore, interventions are required to allow modulating those levels. Objective: To evaluate the effect of an educational Nursing intervention compared to conventional care on the uncertainty of family members of patients hospitalized in an ICU. Materials and methods: An experimental study with a sample comprised by 132 relatives of patients admitted to an ICU, randomly distributed in four Solomon groups (33 in each group). The Nursing intervention based on the concepts of the Uncertainty in Illness Theory was applied to both experimental groups and devised under the Whittemore and Grey parameters with three moments: assessment; education about the relative's hospitalization in the ICU; and accompaniment. This was done with pre-assessments for two groups and post-assessments for the four groups, using the PPUS-FM Uncertainty Scale. The data were analyzed by means of descriptive statistics and respective non-parametric analyses. The study took into account the ethical principles in research. Results: The family members in the experimental groups presented a lower final uncertainty level when compared to the control groups, with a difference of 73.04 points with p-value of 0.001. Discussion: Standardized interventions and under a theoretical model allow reducing uncertainty in relatives of patients in ICUs. Conclusions: The Nursing intervention based on the Uncertainty theory allows reducing uncertainty in relatives of patients hospitalized in an Intensive Care Unit.},
   author = {Diego Omar Pérez Campos and Alejandra Fuentes-Ramírez},
   doi = {10.15649/cuidarte.3220},
   issn = {23463414},
   issue = {1},
   journal = {Revista Cuidarte},
   keywords = {Critical Care,Family,Life Change Events,Nursing Care,Uncertainty},
   pages = {15-27},
   publisher = {Universidad de Santander},
   title = {Effect of a Nursing intervention on the uncertainty of family members in Intensive Care},
   volume = {15},
   year = {2023},
}

@article{Kucukgoz2025,
   abstract = {Full-thickness macular holes are a relatively common and visually disabling condition with a prevalence of approximately 0.5 in the over-40-year-old age group. If left untreated, the hole typically enlarges, reducing visual acuity (VA) below the definition of blindness in the eye affected. They are now routinely treated with surgery, which can close the hole and improve vision in most cases. The extent of improvement, however, is variable and dependent on the size of the hole and other features which can be discerned in spectral-domain optical coherence tomography imaging, which is now routinely available in eye clinics globally. Artificial intelligence (AI) models have been developed to enable surgical decision-making and have achieved relatively high predictive performance. However, their black-box behavior is opaque to users and uncertainty associated with their predictions is not typically stated, leading to a lack of trust among clinicians and patients. In this paper, we describe an uncertainty-aware regression model (U-ARM) for predicting VA for people undergoing macular hole surgery using preoperative spectral-domain optical coherence tomography images, achieving an MAE of 6.07, RMSE of 9.11 and R2 of 0.47 in internal tests, and an MAE of 6.49, RMSE of 9.49, and R2 of 0.42 in external tests. In addition to predicting VA following surgery, U-ARM displays its associated uncertainty, a p-value of <0.005 in internal and external tests, showing the predictions are not due to random chance. We then qualitatively evaluated the performance of U-ARM. Lastly, we demonstrate out-of-sample data performance, generalizing well to data outside the training distribution, low-quality images, and unseen instances not encountered during training. The results show that U-ARM outperforms commonly used methods in terms of prediction and reliability. U-ARM is thus a promising approach for clinical settings and can improve the reliability of AI models in predicting VA.},
   author = {Burak Kucukgoz and Ke Zou and Declan C. Murphy and David H. Steel and Boguslaw Obara and Huazhu Fu},
   doi = {10.1016/j.compmedimag.2024.102461},
   issn = {18790771},
   journal = {Computerized Medical Imaging and Graphics},
   keywords = {Evidential deep regression,Image analysis,Machine learning,Optical coherence tomography,Uncertainty,Visual acuity measurement},
   month = {1},
   publisher = {Elsevier Ltd},
   title = {Uncertainty-aware regression model to predict post-operative visual acuity in patients with macular holes},
   volume = {119},
   year = {2025},
}

@article{Nurhidayah2023,
   abstract = {Background: Parents of newly diagnosed cancer children often experience significant concerns about the implications of the diagnosis. They find themselves in challenging decision-making situations, navigating through uncertain conditions following the disclosure. Uncertainty is a prevailing issue in healthcare, yet its interpretation and application within the context of health and nursing practice exhibit multiple meanings and variations. Objective: This study aimed to clarify the concept of parental uncertainty arising from having children with cancer. Methods: The concept analysis followed the steps outlined by Walker and Avant. A thorough literature search was conducted using the Embase, CINAHL, and MEDLINE databases to identify articles published between 1980 and 2022. Results: The literature search yielded 147 articles from various disciplines, including health, nursing, medicine, psycho-oncology, and management. After analysis, 20 articles were selected for inclusion. This study identified four key attributes of parental uncertainty associated with having a child with cancer: (1) emotional disturbance, (2) unpredictability, (3) insufficient information, and (4) problems with decision-making. The antecedents of parental uncertainty encompassed the complexity of the disease, the diagnostic and treatment processes, the hospital environment, communication, and support from credible authorities. The consequences of parental uncertainty included the pursuit of new information, parental adaptability to their role, and parental distress. Conclusion: Understanding the four attributes of parental uncertainty, along with their antecedents and consequences, can facilitate the future development and operational translation of the concept of uncertainty in nursing practice. This concept is valuable in the evidence-based provision of nursing care to parents of children with cancer, enabling comprehensive recognition and assessment of parental uncertainty and the implementation of appropriate interventions that are sensitive to parental experiences. Ultimately, this approach promotes the adaptation of both the child and the parent.},
   author = {Ikeu Nurhidayah and Nani Nurhaeni and Allenidekania Allenidekania and Dewi Gayatri and Yeni Rustina},
   doi = {10.33546/bnj.2612},
   issn = {24774073},
   issue = {3},
   journal = {Belitung Nursing Journal},
   keywords = {cancer,children,concept analysis,parents,uncertainty},
   month = {5},
   pages = {218-226},
   publisher = {Belitung Raya Publisher - Belitung Raya Foundation},
   title = {Uncertainty of parents due to having children with cancer: A concept analysis},
   volume = {9},
   year = {2023},
}


@article{Huang2025,
   abstract = {Deep learning has been extensively applied in medical image reconstruction, where Convolutional Neural Networks (CNNs) and Vision Transformers (ViTs) represent the predominant paradigms, each possessing distinct advantages and inherent limitations: CNNs exhibit linear complexity with local sensitivity, whereas ViTs demonstrate quadratic complexity with global sensitivity. The emerging Mamba has shown superiority in learning visual representation, which combines the advantages of linear scalability and global sensitivity. In this study, we introduce MambaMIR, an Arbitrary-Masked Mamba-based model with wavelet decomposition for joint medical image reconstruction and uncertainty estimation. A novel Arbitrary Scan Masking (ASM) mechanism “masks out” redundant information to introduce randomness for further uncertainty estimation. Compared to the commonly used Monte Carlo (MC) dropout, our proposed MC-ASM provides an uncertainty map without the need for hyperparameter tuning and mitigates the performance drop typically observed when applying dropout to low-level tasks. For further texture preservation and better perceptual quality, we employ the wavelet transformation into MambaMIR and explore its variant based on the Generative Adversarial Network, namely MambaMIR-GAN. Comprehensive experiments have been conducted for multiple representative medical image reconstruction tasks, demonstrating that the proposed MambaMIR and MambaMIR-GAN outperform other baseline and state-of-the-art methods in different reconstruction tasks, where MambaMIR achieves the best reconstruction fidelity and MambaMIR-GAN has the best perceptual quality. In addition, our MC-ASM provides uncertainty maps as an additional tool for clinicians, while mitigating the typical performance drop caused by the commonly used dropout.},
   author = {Jiahao Huang and Liutao Yang and Fanwen Wang and Yinzhe Wu and Yang Nan and Weiwen Wu and Chengyan Wang and Kuangyu Shi and Angelica I. Aviles-Rivero and Carola Bibiane Schönlieb and Daoqiang Zhang and Guang Yang},
   doi = {10.1016/j.media.2024.103334},
   issn = {13618423},
   journal = {Medical Image Analysis},
   keywords = {Deep Learning,Mamba,Medical image reconstruction,Uncertainty,Wavelet},
   month = {1},
   publisher = {Elsevier B.V.},
   title = {Enhancing global sensitivity and uncertainty quantification in medical image reconstruction with Monte Carlo arbitrary-masked mamba},
   volume = {99},
   year = {2025},
}


@article{Shen2023,
   abstract = {Background: One of the most prevalent psychological signs of breast cancer is uncertainty, which is more prevalent in Chinese patients during the preoperative period. Despite the numerous factors contributing to preoperative uncertainty, there is limited relevant research conducted in China. Objective: This study aimed to describe the current state of preoperative uncertainty and to investigate the relationship between anxiety, illness perception, social support, and preoperative uncertainty in patients with breast cancer in Wenzhou, China. Methods: This cross-sectional research used a simple random sampling technique to select 122 participants from a university hospital in Wenzhou, China, from July 2022 to December 2022, employing validated instruments. Descriptive statistics and Pearson’s correlation coefficient were utilized to analyze the data. Results: The average preoperative uncertainty scores of the patients fell within a moderate range (M = 61.92, SD = 7.51). Significant correlations were found between anxiety (r = 0.638, p <0.01), illness perception (r = 0.704, p <0.01), social support (r = -0.481, p <0.01), and preoperative uncertainty. Conclusions: The results can assist healthcare professionals, especially nurses, in recognizing the factors contributing to uncertainty before surgery in patients with breast cancer. This knowledge enables them to promptly address and minimize this issue, leading to improved outcomes.},
   author = {Huaiyu Shen and Khemaradee Masingboon and Niphawan Samartkit},
   doi = {10.33546/bnj.2648},
   issn = {24774073},
   issue = {3},
   journal = {Belitung Nursing Journal},
   keywords = {China,anxiety,breast neoplasms,illness perception,nurses,social support,uncertainty},
   month = {5},
   pages = {236-243},
   publisher = {Belitung Raya Publisher - Belitung Raya Foundation},
   title = {Factors related to preoperative uncertainty among patients with breast cancer in Wenzhou, China: A cross-sectional study},
   volume = {9},
   year = {2023},
}


@article{Bora2024,
   abstract = {Background: The inconsistent course of schizophrenia causes a long-term experience of uncertainty for individuals and their families. In Turkey, no studies yet exist that have attempted to address this constant uncertainty that is experienced by caregivers of schizophrenic patients. Aims: To evaluate the effects of the Uncertainty Management Psychoeducation Program on reducing uncertainty and intolerance to uncertainty, improving psychological well-being, and coping styles in caregivers of patients with schizophrenia. Method: Single-blinded randomized controlled trial. Caregivers of schizophrenia inpatients were recruited from the psychiatry clinic of a university-affiliated hospital. Data were collected between April 2019 and August 2020. Eligible individuals were randomly allocated to one of the two groups: intervention or control. The intervention group had five individual psychoeducation sessions: “Recognizing Uncertainty,” “Cognitively Reframing Uncertainty,” “Solving Uncertainty-Related Issues,” “Dealing with Uncertainty Using Communication Skills,” and the “Closing Session.” Participants in the control group received the usual care. Uncertainty, intolerance to uncertainty, psychological well-being, and stress coping strategies were measured at two points: at baseline and immediately following the intervention. Hypotheses were tested using the Mann–Whitney U and Wilcoxon tests. Results: A total of 54 participants were recruited. The intervention group’s ratings for “seeking social support” and “optimistic approach” were higher than the control group’s ratings. Significant within-group changes in terms of “uncertainty” and “optimistic approach” were reported for the intervention group in the post-intervention. In the control group, significant changes were seen in terms of “uncertainty” and “psychological well-being” over time. Conclusion: The Uncertainty Management Psychoeducation Program was found to be effective in reducing the level of uncertainty, increasing their optimistic approach, and seeking social support of caregivers of schizophrenic patients.},
   author = {Sultan Taş Bora and Kadriye Buldukoğlu and Donald Etheridge Bailey},
   doi = {10.1177/10783903221141890},
   issn = {15325725},
   issue = {3},
   journal = {Journal of the American Psychiatric Nurses Association},
   keywords = {family caregivers,psychiatric nursing,psychoeducation,reconceptualized uncertainty in illness theory,schizophrenia},
   month = {5},
   pages = {590-602},
   pmid = {36475415},
   publisher = {SAGE Publications Inc.},
   title = {Effectiveness of an Uncertainty Management Psychoeducation Program for Schizophrenia Caregivers: A Randomized Controlled Trial},
   volume = {30},
   year = {2024},
}

@misc{lanfredi2024enhancingchestxraydatasets,
      title={Enhancing chest X-ray datasets with privacy-preserving large language models and multi-type annotations: a data-driven approach for improved classification}, 
      author={Ricardo Bigolin Lanfredi and Pritam Mukherjee and Ronald Summers},
      year={2024},
      eprint={2403.04024},
      archivePrefix={arXiv},
      primaryClass={eess.IV},
      url={https://arxiv.org/abs/2403.04024}, 
}

@misc{Chen2025,
   abstract = {Deep learning technologies have dramatically reshaped the field of medical image registration over the past decade. The initial developments, such as regression-based and U-Net-based networks, established the foundation for deep learning in image registration. Subsequent progress has been made in various aspects of deep learning-based registration, including similarity measures, deformation regularizations, network architectures, and uncertainty estimation. These advancements have not only enriched the field of image registration but have also facilitated its application in a wide range of tasks, including atlas construction, multi-atlas segmentation, motion estimation, and 2D–3D registration. In this paper, we present a comprehensive overview of the most recent advancements in deep learning-based image registration. We begin with a concise introduction to the core concepts of deep learning-based image registration. Then, we delve into innovative network architectures, loss functions specific to registration, and methods for estimating registration uncertainty. Additionally, this paper explores appropriate evaluation metrics for assessing the performance of deep learning models in registration tasks. Finally, we highlight the practical applications of these novel techniques in medical imaging and discuss the future prospects of deep learning-based image registration.},
   author = {Junyu Chen and Yihao Liu and Shuwen Wei and Zhangxing Bian and Shalini Subramanian and Aaron Carass and Jerry L. Prince and Yong Du},
   doi = {10.1016/j.media.2024.103385},
   issn = {13618423},
   journal = {Medical Image Analysis},
   keywords = {Deep neural networks,Image registration,Medical imaging},
   month = {2},
   publisher = {Elsevier B.V.},
   title = {A survey on deep learning in medical image registration: New technologies, uncertainty, evaluation metrics, and beyond},
   volume = {100},
   year = {2025},
}

@article{Praud2025,
   author = {Delphine Praud and Amina Amadou and Thomas Coudon and Margaux Duboeuf and Benoît Mercoeur and Elodie Faure and Lény Grassot and Aurélie MN. Danjou and Pietro Salizzoni and Florian Couvidat and Laure Dossus and Gianluca Severi and Francesca Romana Mancini and Béatrice Fervers},
   doi = {10.1016/j.ijheh.2024.114489},
   issn = {14384639},
   journal = {International Journal of Hygiene and Environmental Health},
   month = {1},
   pages = {114489},
   title = {Association between chronic long-term exposure to airborne dioxins and breast cancer},
   volume = {263},
   url = {https://linkinghub.elsevier.com/retrieve/pii/S1438463924001706},
   year = {2025},
}

@article{ChenEtal2025,
   abstract = {Background: Sample size calculation and power estimate are an integral part of clinical trials. With accelerated development to address the unmet medical needs, the fast-paced development may lead to uncertainties in initial planning and assumptions of clinical trials. Promising zone design presents sponsors an opportunity to re-estimate the sample size based on the interim data to mitigate risks, reduce uncertainties, and increase probability of trial success. Methods: This paper aims to use the GRAPHITE trial (NCT03657160) as a real data application to showcase the practical considerations in implementation of promising zone design for interim sample size re-estimation (SSR), in light of sample size adaptation rules, maximum sample size allowed, multiplicity adjustment, and sponsor access to interim results. GRAPHITE is a phase 3 trial with vedolizumab for prophylaxis of acute graft vs host disease (aGvHD) after allogeneic hematopoietic stem cell transplant (allo-HSCT). The primary efficacy endpoint is lower intestinal aGVHD-free survival by Day +180 after allo-HSCT. A simulation study was conducted to demonstrate the evaluation of operating characteristics by various true underlying treatment effects at the design stage. Conclusion: The application of promising zone design for interim SSR is novel and has successfully helped the sponsor achieve the balance between minimizing the risks and maintaining scientific integrity. This work aims to highlight the necessity of empirical guidance to gain better insights for clinical researchers in practice and is expected to facilitate the understanding and implementation of promising zone design for interim SSR in phase 3 trials.},
   author = {Jingjing Chen and Yohei Takanami and Johan Jansson and Guillermo Rossiter},
   doi = {10.1016/j.cct.2024.107765},
   issn = {15592030},
   journal = {Contemporary Clinical Trials},
   keywords = {Futility analysis,Graft vs host disease,Interim sample size re-estimation,Promising zone design,Vedolizumab},
   month = {1},
   publisher = {Elsevier Inc.},
   title = {Practical considerations of promising zone design for interim sample size Re-estimation: An application to GRAPHITE for graft vs host disease},
   volume = {148},
   year = {2025},
}

@article{Trowman2021,
   abstract = {As health technology assessment (HTA) seeks to combine complex sets of evidence, values, and perspectives to support open, accountable, and transparent decision making, uncertainty is inherent. Uncertainty is present in the clinical and economic inputs that inform HTA and is a critical factor during context-specific deliberations where the evidence is weighed and decisions are made, taking uncertainty into account through either financial or evidence-generation mechanisms. The presence and impact of uncertainty must also be communicated to all relevant stakeholders during the HTA output stage. This article summarizes the 2021 HTAi Global Policy Forum discussion on “Considering and Communicating Uncertainty in HTA” that debated some of the key challenges and opportunities regarding uncertainty in HTA. Through a combination of small and large group discussions, core themes related to the topic of uncertainty in HTA were identified. These discussions revealed that: utilization of a life cycle/HTA management approach helps manage uncertainty; genuine stakeholder input and engagement (and not just consultation) can clarify uncertainty; tolerance of risk, the relationship of risk to uncertainty, and the context in which uncertainty is considered is critical; transparent and early dialogues could be increased to further reduce the uncertainty during HTA; and communicating uncertainty in HTA outputs is critical. The paper ends with suggested next steps that HTA agencies and stakeholders (such as industry, patients, regulators, payers, and others) might take to move the field forward. The paper promotes further discussion on aspects of uncertainty that should be more openly discussed, debated, and addressed.},
   author = {Rebecca Trowman and Alicia Powers and Daniel A. Ollendorf},
   doi = {10.1017/S0266462321000453},
   issn = {14716348},
   issue = {1},
   journal = {International Journal of Technology Assessment in Health Care},
   keywords = {Context,Life cycle,Stakeholder engagement,Transparency,Uncertainty},
   pmid = {34261561},
   publisher = {Cambridge University Press},
   title = {Considering and communicating uncertainty in health technology assessment},
   volume = {37},
   year = {2021},
}

@article{Karthik2025,
   abstract = {In the realm of pulmonary medicine, prognostic assessment of Idiopathic Pulmonary Fibrosis (IPF) poses a significant challenge, necessitating advancements in predictive analytics. This study introduces a pioneering predictive model that synergistically utilizes Convolutional Neural Networks (CNNs) and Long Short-Term Memory (LSTM) networks to analyze CT scans and clinical data, offering a dynamic prediction of IPF progression. The model's methodology is rooted in the integration of detailed spatial features and temporal clinical patterns to forecast disease trajectory with heightened accuracy. A novel aspect of this model is its built-in mechanism for uncertainty quantification, enhancing the interpretability of its prognostic output. Through validation, the proposed model demonstrated a mean Out-of-Fold (OOF) validation score 6.9679 and accuracy of 95\% notably superior to traditional methods, alongside a conservative yet precise approach to uncertainty estimation. The findings represent a substantial improvement in predictive capabilities, emphasizing the model's potential to inform clinical decision-making and facilitate personalized treatment strategies. The implications of this research extend beyond IPF, providing a framework for future explorations into machine learning applications in complex disease prognostics.},
   author = {A. Karthik and Sridhar Patthi and B. Uma Maheswari and J. Sirisha Devi and Abhaya Kumar Pradhan and L. Balaji and G. Nallasivan and A. Rajaram},
   doi = {10.1016/j.bspc.2024.106811},
   issn = {17468108},
   journal = {Biomedical Signal Processing and Control},
   keywords = {Convolutional neural networks,Disease progression,Idiopathic pulmonary fibrosis,Long short-term memory networks,Machine learning,Predictive modeling,Uncertainty quantification},
   month = {2},
   publisher = {Elsevier Ltd},
   title = {Advancing idiopathic pulmonary fibrosis prognosis through integrated CNN-LSTM predictive modeling and uncertainty quantification},
   volume = {100},
   year = {2025},
}

@article{Wang2025,
   abstract = {Background and Objective: Epicardial Adipose Tissue (EAT) is regarded as an independent risk factor for cardiovascular disease, and an increase in its volume is closely associated with disorders such as coronary artery atherosclerosis. Traditional manual and semi-automatic methods for EAT segmentation rely on subjective judgment, resulting in uncertainty and unreliability, which limits their application in clinical practice. Therefore, this study aims to develop a fully automatic segmentation and quantification method to improve the accuracy of EAT assessment. Methods: A Boundary-Enhanced Multi-scale U-Net network with a Convolutional Transformer (BMT-UNet) is developed to segment the pericardium. The BMT-UNet comprises Boundary-Enhanced (BE) modules, Multi-Scale (MS) modules, and a Convolutional Transformer (ConvT) module. The MS and BE modules in the encoding part are designed to capture detailed boundary features and accurately delineate the pericardium boundary by combining multi-scale features with morphological operations, leveraging their complementarity. The ConvT module integrates global contextual information, thereby enhancing overall segmentation accuracy and addressing the issue of internal holes in the segmented pericardial images. The volume of EAT is automatically quantified using standard fat thresholds with a range of −190 to −30 HU. Results: For a Coronary Computed Tomography Angiography (CCTA) dataset which contained 50 patient respectively. The linear regression coefficient between the EAT volume segmented and the actual volume is 0.982, and the Pearson correlation coefficient is 0.99. Bland-Altman analysis further confirmed the high consistency between the automated and manual methods. These results demonstrate a significant improvement over existing methods, particularly in terms of segmentation precision and reliability, which are critical for clinical application. Conclusions: This work develops an automated method for quantifying EAT in Computed Tomography (CT) images, and the results agreed closely with expert evaluations. Code is available at: https://github.com/wy-9903/BMT-UNet.},
   author = {Ying Wang and Ankang Wang and Lu Wang and Wenjun Tan and Lisheng Xu and Jinsong Wang and Songang Li and Jinshuai Liu and Yu Sun and Benqiang Yang and Steve Greenwald},
   doi = {10.1016/j.bspc.2024.107167},
   issn = {17468108},
   journal = {Biomedical Signal Processing and Control},
   keywords = {Computed tomography,Deep neural network,Epicardial adipose tissue,Pericardium segmentation},
   month = {2},
   publisher = {Elsevier Ltd},
   title = {Automated pericardium segmentation and epicardial adipose tissue quantification from computed tomography images},
   volume = {100},
   year = {2025},
}

@article{Haq2025,
   abstract = {Introduction: Ultrasonography is among the most regularly used methods for earlier detection of breast cancer. Automatic and precise segmentation of breast masses in breast ultrasound (US) images is essential but still a challenge due to several causes of uncertainties, like the high variety of tumor shapes and sizes, obscure tumor borders, very low SNR, and speckle noise. Method: To deal with these uncertainties, this work presents an effective and automated GAN based approach for tumor segmentation in breast US named MAR-GAN, to extract rich, informative features from US images. In MAR-GAN the capabilities of the traditional encoder-decoder generator were enhanced by multiple modifications. Multi-scale residual blocks were used to retrieve additional aspects of the tumor area for a more precise description. A novel boundary and foreground attention (BFA) module is proposed to increase attention for the tumor region and boundary curve. The squeeze and excitation (SE) and the adaptive context selection (ACS) modules were added to increase representational capability on encoder side and facilitates better selection and aggregation of contextual information on the decoder side respectively. The L1-norm and structural similarity index metric (SSIM) were added into the MAR-GAN's loss function to capture rich local context information from the tumors’ surroundings.},
   author = {Imran Ul Haq and Haider Ali and Yuefeng Li and Zhe Liu},
   doi = {10.1016/j.bspc.2024.107171},
   issn = {17468108},
   journal = {Biomedical Signal Processing and Control},
   keywords = {Breast cancer,GAN,Multi-attention,Segmentation,Ultrasound},
   month = {2},
   publisher = {Elsevier Ltd},
   title = {MAR-GAN: Multi attention residual generative adversarial network for tumor segmentation in breast ultrasounds},
   volume = {100},
   year = {2025},
}

@article{Darley2023,
   abstract = {Objective: Digital health technology is valued as a tool to provide person-centred care and improve health outcomes amongst people with cancer and their family caregivers. Although the evidence to date shows encouraging effectiveness, there is limited knowledge regarding the lived experience and personal meaning of using supportive technology during cancer treatment. The aim of this study was to explore the lived experiences of people with colorectal cancer receiving chemotherapy using digital health symptom management technology and their family caregivers. Methods: A longitudinal and multi-perspective interpretative phenomenological analytical approach was adopted including three people with newly diagnosed colorectal cancer and four family caregivers. Findings: Three superordinate themes and related subthemes were identified. The first theme (The 3 Cs of symptom management technology) centred on the continuity of care that participants felt while using the technology. The second theme (Digital health technology as a psychosocial support) offered insights into the psychological benefits using technology incurred as they navigated their cancer diagnosis including sense of control and psychological safety. The final theme (Impact of digital health technology on family caregivers) details the supportive effect the technology had on family caregivers’ role, responsibilities and well-being during the cancer experience. Conclusion: Digital health technology can act as a bridge from uncertainty to an understanding regarding a cancer diagnosis and its treatment. Digital health technology can support peoples’ understanding of cancer and enhance self-management practices, while being a psychological support in navigating the uncertain and often worrying period of receiving cancer treatment.},
   author = {Andrew Darley and Barbara Coughlan and Roma Maguire and Lisa McCann and Eileen Furlong},
   doi = {10.1177/20552076231152163},
   issn = {20552076},
   journal = {Digital Health},
   keywords = {Digital health,cancer,family caregiving,interpretative phenomenology,qualitative research},
   month = {1},
   publisher = {SAGE Publications Inc.},
   title = {A bridge from uncertainty to understanding: The meaning of symptom management digital health technology during cancer treatment},
   volume = {9},
   year = {2023},
}


@article{Akkuş2023,
   abstract = {Disease-related uncertainty and the factors associated with uncertainty in patients with cancer have not been adequately investigated. This study aimed to determine the relationship between intolerance of uncertainty and attitudes toward complementary and alternative medicine (CAM) in patients with cancer. This cross-sectional descriptive study included 351 patients treated in the oncology clinic of a university hospital. and showed a weak negative correlation. The patients in our study showed high intolerance of uncertainty and a moderately positive attitude toward CAM, and most patients did not notify health care professionals of their CAM use. Therefore, we recommend assessing intolerance of uncertainty and CAM use in this patient group. By identifying patients experiencing uncertainty and seeking different treatment, nurses can support patients physiologically, psychologically, and socially, and can explain the effects of CAM use.},
   author = {Yeliz Akkuş and Tuǧba Menekli},
   doi = {10.1097/HNP.0000000000000600},
   issn = {15505138},
   issue = {5},
   journal = {Holistic Nursing Practice},
   keywords = {cancer,complementary and alternative medicine,uncertainty},
   month = {9},
   pages = {277-284},
   pmid = {37595120},
   publisher = {Lippincott Williams and Wilkins},
   title = {Determining the Relationship Between Intolerance of Uncertainty and Attitudes Toward Complementary and Alternative Medicine in Patients With Cancer},
   volume = {37},
   year = {2023},
}

@article{Dijk2024,
   abstract = {Background: The COVID-19 pandemic underscored the criticality and complexity of decision making for novel treatment approval and further research. Our study aims to assess potential decision-making methodologies, an evaluation vital for refining future public health crisis responses. Methods: We compared 4 decision-making approaches to drug approval and research: the Food and Drug Administration’s policy decisions, cumulative meta-analysis, a prospective value-of-information (VOI) approach (using information available at the time of decision), and a reference standard (retrospective VOI analysis using information available in hindsight). Possible decisions were to reject, accept, provide emergency use authorization, or allow access to new therapies only in research settings. We used monoclonal antibodies provided to hospitalized COVID-19 patients as a case study, examining the evidence from September 2020 to December 2021 and focusing on each method’s capacity to optimize health outcomes and resource allocation. Results: Our findings indicate a notable discrepancy between policy decisions and the reference standard retrospective VOI approach with expected losses up to $269 billion USD, suggesting suboptimal resource use during the wait for emergency use authorization. Relying solely on cumulative meta-analysis for decision making results in the largest expected loss, while the policy approach showed a loss up to $16 billion and the prospective VOI approach presented the least loss (up to $2 billion). Conclusion: Our research suggests that incorporating VOI analysis may be particularly useful for research prioritization and treatment implementation decisions during pandemics. While the prospective VOI approach was favored in this case study, further studies should validate the ideal decision-making method across various contexts. This study’s findings not only enhance our understanding of decision-making strategies during a health crisis but also provide a potential framework for future pandemic responses. This study reviews discrepancies between a reference standard (retrospective VOI, using hindsight information) and 3 conceivable real-time approaches to research-treatment decisions during a pandemic, suggesting suboptimal use of resources. Of all prospective decision-making approaches considered, VOI closely mirrored the reference standard, yielding the least expected value loss across our study timeline. This study illustrates the possible benefit of VOI results and the need for evidence accumulation accompanied by modeling in health technology assessment for emerging therapies.},
   author = {Stijntje W. Dijk and Eline Krijkamp and Natalia Kunst and Jeremy A. Labrecque and Cary P. Gross and Aradhana Pandit and Chia Ping Lu and Loes E. Visser and John B. Wong and M. G.Myriam Hunink},
   doi = {10.1177/0272989X241255047},
   issn = {1552681X},
   issue = {5},
   journal = {Medical Decision Making},
   keywords = {COVID-19,antibodies,cost-benefit analysis,decision support techniques,drug approval,meta-analysis,monoclonal,policy analyses},
   month = {7},
   pages = {512-528},
   pmid = {38828516},
   publisher = {SAGE Publications Inc.},
   title = {Making Drug Approval Decisions in the Face of Uncertainty: Cumulative Evidence versus Value of Information},
   volume = {44},
   year = {2024},
}


@article{Vreman2022,
   abstract = {This study outlines the ways in which different health technology assessment (HTA) organizations deal with uncertainty in relative effectiveness assessments (REAs), using the GRADE framework as a common reference. Guidelines regarding REA and uncertainty assessment methods and three most recent HTA reports (as of April 2020) of seven HTA organizations in Germany, England and Wales, France, the Netherlands, Europe (EUnetHTA), the USA, and Canada were included. First, it was analyzed how each organization addressed uncertainty on the following levels of evidence: (i) individual studies, (ii) body of evidence for one outcome, (iii) body of evidence across all outcomes, and (iv) added net benefit. Second, the extent to which HTA organizations considered the eight domains of certainty of evidence defined by GRADE was assessed. For individual studies, checklists were the most common approach to express uncertainty (4/7 organizations). Uncertainty in the body of evidence for all outcomes and in added benefit was combined in a single conclusion by five organizations. All organizations reported on at least 4/5 downgrading domains of GRADE, while the three upgrading domains were reported less. The operationalization of the assessment of multiple domains was unclear due to vague or absent guidelines. HTA organizations consider most domains of the GRADE framework, but approaches to assess uncertainty within REAs on different levels of evidence differ substantially between organizations. More alignment and guidance on the best methods to deal with uncertainty within HTA could lead to more clarity for stakeholders and to more aligned reimbursement recommendations.},
   author = {Rick A. Vreman and George Strigkos and Hubert G.M. Leufkens and Holger J. Schünemann and Aukje K. Mantel-Teeuwisse and Wim G. Goettsch},
   doi = {10.1017/S026646232100177X},
   issn = {14716348},
   issue = {1},
   journal = {International Journal of Technology Assessment in Health Care},
   keywords = {Added benefit,Clinical benefit,Evidence,Grade,Health technology assessment,Relative effectiveness,Risk of bias,Uncertainty,Value},
   month = {1},
   pmid = {35094740},
   publisher = {Cambridge University Press},
   title = {Addressing uncertainty in relative effectiveness assessments by HTA organizations},
   volume = {38},
   year = {2022},
}


@article{Rothenberger2025,
   author = {Sean M. Rothenberger and Jiacheng Zhang and Michael Markl and Bruce A. Craig and Pavlos P. Vlachos and Vitaliy L. Rayz},
   doi = {10.1002/mrm.30287},
   issn = {0740-3194},
   issue = {1},
   journal = {Magnetic Resonance in Medicine},
   month = {1},
   pages = {397-410},
   title = {4D flow MRI velocity uncertainty quantification},
   volume = {93},
   url = {https://onlinelibrary.wiley.com/doi/10.1002/mrm.30287},
   year = {2025},
}


@article{McGowan2025,
   author = {Samuel K. McGowan and Maria-Jose Corrales-Martinez and Teva Brender and Alexander K. Smith and Shannen Kim and Krista L. Harrison and Hunter Mills and Albert Lee and David Bamman and Julien Cobert},
   doi = {10.1177/0272989X241293446},
   issn = {0272-989X},
   issue = {1},
   journal = {Medical Decision Making},
   month = {1},
   pages = {34-44},
   title = {Unclear Trajectory and Uncertain Benefit: Creating a Lexicon for Clinical Uncertainty in Patients with Critical or Advanced Illness Using a Delphi Consensus Process},
   volume = {45},
   url = {https://journals.sagepub.com/doi/10.1177/0272989X241293446},
   year = {2025},
}


@article{Wiedmann2024,
   abstract = {Objective This study examined the application, feasibility, and validity of supervised learning models for text classification in appraisals for rare disease treatments (RDTs) in relation to uncertainty, and analyzed differences between appraisals based on the classification results. Methods We analyzed appraisals for RDTs (n = 94) published by the National Institute for Health and Care Excellence (NICE) between January 2011 and May 2023. We used Naïve Bayes, Lasso, and Support Vector Machine models in a binary text classification task (classifying paragraphs as either referencing uncertainty in the evidence base or not). To illustrate the results, we tested hypotheses in relation to the appraisal guidance, advanced therapy medicinal product (ATMP) status, disease area, and age group. Results The best performing (Lasso) model achieved 83.6 percent classification accuracy (sensitivity = 74.4 percent, specificity = 92.6 percent). Paragraphs classified as referencing uncertainty were significantly more likely to arise in highly specialized technology (HST) appraisals compared to appraisals from the technology appraisal (TA) guidance (adjusted odds ratio = 1.44, 95 percent CI 1.09, 1.90, p = 0.004). There was no significant association between paragraphs classified as referencing uncertainty and appraisals for ATMPs, non-oncology RDTs, and RDTs indicated for children only or adults and children. These results were robust to the threshold value used for classifying paragraphs but were sensitive to the choice of classification model. Conclusion Using supervised learning models for text classification in NICE appraisals for RDTs is feasible, but the results of downstream analyses may be sensitive to the choice of classification model.},
   author = {Lea Wiedmann and Jack Blumenau and Orlagh Carroll and John Cairns},
   doi = {10.1017/S0266462323002805},
   issn = {14716348},
   issue = {1},
   journal = {International Journal of Technology Assessment in Health Care},
   keywords = {National Institute for Health and Care Excellence,health technology assessment,rare diseases,supervised learning,uncertainty},
   month = {1},
   pmid = {38178720},
   publisher = {Cambridge University Press},
   title = {Using automated text classification to explore uncertainty in NICE appraisals for drugs for rare diseases},
   volume = {40},
   year = {2024},
}

@article{Mennin2023,
   abstract = {Rationale: Question Storming offers a method that enables one to hold the condition of uncertainty in reflection without the need for resolution. Global interdependencies and unprecedented access to information, social mediaand multiple forms of communications challenge our ability to see, understandand influence change effectively and efficiently. The tension and need to cope effectively with massive uncertainties cannot be resolved with current methods leading to a necessity for people to seek new ways to transform their understanding and explore new options for action. Problem-solving and facilitation of the past are not flexible or rapid enough to meet the current demands of decision making and action taking in the face of massive uncertainties. As a result, people face ‘wicked unsolvable’ issues in their personal and professional lives. Aims and Objectives: An international group of scholar-practitioners has adapted and tested an enquiry process. Question Storming—The Power of Questions is based on principles of complex adaptive systems, human systems dynamics, and self-organization. Method: A three-step method of inquiry and reflection opens new possibilities. Results and Conclusions: Question Storming has helped people see their wicked issues from new perspectives, understand them in useful ways and generate new options for action. This paper introduces Question Storming—the Power of Questions as a practical method for group inquiry in the presence of individual and group uncertainties/wicked issues. The Container, Difference, Exchange (CDE) model and Pattern Logic are presented to explain the paradigm-shifting dynamics experienced by participants, both individuals and members of the group. It concludes with emerging questions for future consideration. Question Storming generates a divergent problem space that decreases constraint and increases degrees of freedom to allow practical exploration of new and often surprising options for action.},
   author = {Stewart Mennin and Glenda H. Eoyang},
   doi = {10.1111/jep.13704},
   issn = {13652753},
   issue = {4},
   journal = {Journal of Evaluation in Clinical Practice},
   keywords = {CDE model,Pattern Logic,complex adaptive system,human systems dynamics,inquiry,wicked problems},
   month = {6},
   pages = {650-656},
   pmid = {35604003},
   publisher = {John Wiley and Sons Inc},
   title = {Question storming: The power of Questions—A method to increase options for action in uncertainty},
   volume = {29},
   year = {2023},
}

@article{Palmer2023,
   abstract = {The coronavirus disease 2019 (COVID-19) pandemic and resulting instructions to stay home and social distance enhanced concerns of the impact of social isolation on the physical and mental well-being of older adults. Eighteen community-dwelling older adults participated in interviews describing their experiences early in the COVID-19 pandemic. Participants experienced loss of activities, routines, and social connection, and feelings of worry and uncertainty. Nevertheless, participants were hopeful about the future and demonstrated resilience in overcoming boredom as they became intentional in finding new activities and using technology to maintain connection with others. Older adults may need support in such situations to manage boredom and uncertainty and avoid social isolation.},
   author = {Janice L. Palmer and Devita T. Stallings and Jee Hye Yoo and Rebecca A. Lorenz and Helen W. Lach},
   doi = {10.3928/00989134-20230512-04},
   issn = {00989134},
   issue = {6},
   journal = {Journal of Gerontological Nursing},
   pages = {27-32},
   pmid = {37256759},
   publisher = {Slack Incorporated},
   title = {Experiences of Older Adults During COVID-19: Loss, Boredom, Uncertainty, Worry, and Resilience},
   volume = {49},
   year = {2023},
}


@article{Kang2024,
   abstract = {Despite the success of deep learning methods in multi-modality segmentation tasks, they typically produce a deterministic output, neglecting the underlying uncertainty. The absence of uncertainty could lead to over-confident predictions with catastrophic consequences, particularly in safety-critical clinical applications. Recently, uncertainty estimation has attracted increasing attention, offering a measure of confidence associated with machine decisions. Nonetheless, existing uncertainty estimation approaches primarily focus on single-modality networks, leaving the uncertainty of multi-modality networks a largely under-explored domain. In this study, we present the first exploration of multi-modality uncertainties in the context of tumor segmentation on PET/CT. Concretely, we assessed four well-established uncertainty estimation approaches across various dimensions, including segmentation performance, uncertainty quality, comparison to single-modality uncertainties, and correlation to the contradictory information between modalities. Through qualitative and quantitative analyses, we gained valuable insights into what benefits multi-modality uncertainties derive, what information multi-modality uncertainties capture, and how multi-modality uncertainties correlate to information from single modalities. Drawing from these insights, we introduced a novel uncertainty-driven loss, which incentivized the network to effectively utilize the complementary information between modalities. The proposed approach outperformed the backbone network by 4.53 and 2.92 Dices in percentages on two PET/CT datasets while achieving lower uncertainties. This study not only advanced the comprehension of multi-modality uncertainties but also revealed the potential benefit of incorporating them into the segmentation network. The code is available at https://github.com/HUST-Tan/MMUE.},
   author = {Susu Kang and Yixiong Kang and Shan Tan},
   doi = {10.1109/JBHI.2024.3397332},
   issn = {21682208},
   journal = {IEEE Journal of Biomedical and Health Informatics},
   keywords = {PET/CT,Tumor segmentation,deep learning,multi-modality,uncertainty estimation},
   pmid = {38776203},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {Exploring and Exploiting Multi-modality Uncertainty for Tumor Segmentation on PET/CT},
   year = {2024},
}

@article{Popat2023,
   abstract = {Two significant obstacles exist preventing the widespread usage of Deep Learning (DL) models for predicting healthcare outcomes in general and mental health conditions in particular. Firstly, DL models do not quantify the uncertainty in their predictions, so clinicians are unsure of which predictions they can trust. Secondly, DL models do not triage, i.e., separate which cases could be best handled by the human or the model. This paper attempts to address these obstacles using Bayesian Deep Learning (BDL), which extends DL probabilistically and allows us to quantify the model’s uncertainty, which we use to improve human–model collaboration. We implement a range of state-of-the-art DL models for Natural Language Processing and apply a range of BDL methods to these models. Taking a step closer to the real-life scenarios of human–AI collaboration, we propose a Referral Learning methodology for the models that make predictions for certain instances while referring the rest of the instances to a human expert for further assessment. The study demonstrates that models can significantly enhance their performance by seeking human assistance in cases where the model exhibits high uncertainty, which is closely linked to misclassifications. Referral Learning offers two options: (1) supporting humans in cases where the model predicts with certainty, and (2) triaging cases where the model evaluated when it had a better chance of being right than the human by evaluating human disagreement. The latter method combines model uncertainty from BDL and human disagreement from multiple annotations, resulting in improved triaging capabilities.},
   author = {Ram Popat and Julia Ive},
   doi = {10.3389/fdgth.2023.1188338},
   issn = {2673253X},
   journal = {Frontiers in Digital Health},
   keywords = {Bayesian Deep Learning,human uncertainty,human–machine collaboration,mental health conditions,uncertainty},
   publisher = {Frontiers Media SA},
   title = {Embracing the uncertainty in human–machine collaboration to support clinical decision-making for mental health conditions},
   volume = {5},
   year = {2023},
}

@ARTICLE{9263102,
  author={Cicalese, Pietro Antonio and Mobiny, Aryan and Shahmoradi, Zahed and Yi, Xiongfeng and Mohan, Chandra and Van Nguyen, Hien},
  journal={IEEE Journal of Biomedical and Health Informatics}, 
  title={Kidney Level Lupus Nephritis Classification Using Uncertainty Guided Bayesian Convolutional Neural Networks}, 
  year={2021},
  volume={25},
  number={2},
  pages={315-324},
  keywords={Uncertainty;Bayes methods;Solid modeling;Kidney;Diseases;Task analysis;Biopsy;Bayesian deep network;lupus glomerulonephritis;lupus nephritis;model uncertainty;physician-friendly machine learning},
  doi={10.1109/JBHI.2020.3039162}}



@article{Sabeti2021,
   abstract = {Acute respiratory distress syndrome (ARDS) is a fulminant inflammatory lung injury that develops in patients with critical illnesses, affecting 200,000 patients in the United States annually. However, a recent study suggests that most patients with ARDS are diagnosed late or missed completely and fail to receive life-saving treatments. This is primarily due to the dependency of current diagnosis criteria on chest X-ray, which is not necessarily available at the time of diagnosis. In machine learning, such an information is known as Privileged Information-information that is available at training but not at testing. However, in diagnosing ARDS, privileged information (chest X-rays) are sometimes only available for a portion of the training data. To address this issue, the Learning Using Partially Available Privileged Information (LUPAPI) paradigm is proposed. As there are multiple ways to incorporate partially available privileged information, three models built on classical SVM are described. Another complexity of diagnosing ARDS is the uncertainty in clinical interpretation of chest X-rays. To address this, the LUPAPI framework is then extended to incorporate label uncertainty, resulting in a novel and comprehensive machine learning paradigm-Learning Using Label Uncertainty and Partially Available Privileged Information (LULUPAPI). The proposed frameworks use Electronic Health Record (EHR) data as regular information, chest X-rays as partially available privileged information, and clinicians' confidence levels in ARDS diagnosis as a measure of label uncertainty. Experiments on an ARDS dataset demonstrate that both the LUPAPI and LULUPAPI models outperform SVM, with LULUPAPI performing better than LUPAPI.},
   author = {Elyas Sabeti and Joshua Drews and Narathip Reamaroon and Elisa Warner and Michael W. Sjoding and Jonathan Gryak and Kayvan Najarian},
   doi = {10.1109/JBHI.2020.3008601},
   issn = {21682208},
   issue = {3},
   journal = {IEEE Journal of Biomedical and Health Informatics},
   keywords = {ARDS,EHR data,SVM,chest X-ray,label uncertainty,partially available privileged information},
   month = {3},
   pages = {784-796},
   pmid = {32750956},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {Learning Using Partially Available Privileged Information and Label Uncertainty: Application in Detection of Acute Respiratory Distress Syndrome},
   volume = {25},
   year = {2021},
}

@article{Zahari2024,
   abstract = {In radiology, particularly in lung cancer diagnosis, diagnostic errors and cognitive biases pose substantial challenges. These issues, including perceptual errors, interpretive mistakes, and cognitive biases such as anchoring and premature closure, are often unnoticed by experienced radiologists. To address these challenges, we propose the Multi-Eyes principle approach, which utilises multiple deep learning models to reduce bias and potentially improve diagnostic accuracy. Inspired by the Four-Eyes principle in business and cybersecurity, this methodology employs various 3D and 2D (for validation) deep learning architectures and three uncertainty quantification techniques: Monte Carlo Dropout, Deep Ensemble, and Ensemble Monte Carlo Dropout. Each model functions as an independent reviewer, similar to blind reviews. With entropy selected as the uncertainty measurement, it is averaged, followed by ensemble averaging of predictions. The effectiveness of this approach was demonstrated using the LIDC-IDRI dataset for lung cancer classification. Statistical analysis of the uncertainty's distribution reveals that with more models, uncertainty in incorrect predictions becomes more peaked and left skewed, indicating consensus on uncertainty levels. This results in accuracy and F1 score improvements, even with the best performing model, addressing overconfidence in single-model systems. These findings highlight the potential of the Multi-Eyes principle to significantly improve diagnostic performance in computer-aided diagnostic systems. Future research may explore different uncertainty quantification methods and feedback mechanisms for further advancement.},
   author = {Rahimi Zahari and Julie Cox and Boguslaw Obara},
   doi = {10.1109/JBHI.2024.3446040},
   issn = {21682208},
   journal = {IEEE Journal of Biomedical and Health Informatics},
   keywords = {Deep ensemble,Monte Carlo dropout,lung cancer,multi-eyes,uncertainty quantification},
   publisher = {Institute of Electrical and Electronics Engineers Inc.},
   title = {Mitigating Diagnostic Errors in Lung Cancer Classification: A Multi-Eyes Principle to Uncertainty Quantification},
   year = {2024},
}


@article{Zhang2023,
   abstract = {The uncertainty in predictions from deep neural network analysis of medical imaging is challenging to assess but potentially important to include in subsequent decision-making. Using data from diabetic retinopathy detection, we present an empirical evaluation of the role of model calibration in uncertainty-based referral, an approach that prioritizes referral of observations based on the magnitude of a measure of uncertainty. We consider several configurations of network architecture, methods for uncertainty estimation, and training data size. We identify a strong relationship between the effectiveness of uncertainty-based referral and having a well-calibrated model. This is especially relevant as complex deep neural networks tend to have high calibration errors. Finally, we show that post-calibration of the neural network helps uncertainty-based referral with identifying hard-to-classify observations.},
   author = {Ruotao Zhang and Constantine Gatsonis and Jon Arni Steingrimsson},
   doi = {10.1177/09622802231158811},
   issn = {14770334},
   issue = {5},
   journal = {Statistical Methods in Medical Research},
   keywords = {Deep learning,calibration,diabetic retinopathy,domain adaptation,post-calibration,uncertainty estimation},
   month = {5},
   pages = {927-943},
   pmid = {37011026},
   publisher = {SAGE Publications Ltd},
   title = {Role of calibration in uncertainty-based referral for deep learning},
   volume = {32},
   year = {2023},
}


@misc{Teng2024,
   abstract = {Background and Objective: Medical image segmentation is a vital aspect of medical image processing, allowing healthcare professionals to conduct precise and comprehensive lesion analyses. Traditional segmentation methods are often labor intensive and influenced by the subjectivity of individual physicians. The advent of artificial intelligence (AI) has transformed this field by reducing the workload of physicians, and improving the accuracy and efficiency of disease diagnosis. However, conventional AI techniques are not without challenges. Issues such as inexplicability, uncontrollable decision-making processes, and unpredictability can lead to confusion and uncertainty in clinical decision-making. This review explores the evolution of AI in medical image segmentation, focusing on the development and impact of explainable AI (XAI) and trustworthy AI (TAI). Methods: This review synthesizes existing literature on traditional segmentation methods, AI-based approaches, and the transition from conventional AI to XAI and TAI. The review highlights the key principles and advancements in XAI that aim to address the shortcomings of conventional AI by enhancing transparency and interpretability. It further examines how TAI builds on XAI to improve the reliability, safety, and accountability of AI systems in medical image segmentation. Key Content and Findings: XAI has emerged as a solution to the limitations of conventional AI by providing greater transparency and interpretability, allowing healthcare professionals to better understand and trust AI-driven decisions. However, XAI itself faces challenges, including those related to safety, robustness, and value alignment. TAI has been developed to overcome these challenges, offering a more reliable framework for AI applications in medical image segmentation. By integrating the principles of XAI with enhanced safety and dependability, TAI addresses the critical need for TAI systems in clinical settings. Conclusions: TAI presents a promising future for medical image segmentation, combining the benefits of AI with improved reliability and safety. Thus, TAI is a more viable and dependable option for healthcare applications, and could ultimately lead to better clinical outcomes for patients, and advance the field of medical image processing.},
   author = {Zixuan Teng and Lan Li and Ziqing Xin and Dehui Xiang and Jiang Huang and Hailing Zhou and Fei Shi and Weifang Zhu and Jing Cai and Tao Peng and Xinjian Chen},
   doi = {10.21037/qims-24-723},
   issn = {22234306},
   issue = {12},
   journal = {Quantitative Imaging in Medicine and Surgery},
   keywords = {Medical image segmentation,artificial intelligence (AI),explainable AI (XAI),trustworthy AI (TAI)},
   month = {12},
   pages = {9620-9652},
   publisher = {AME Publishing Company},
   title = {A literature review of artificial intelligence (AI) for medical image segmentation: from AI and explainable AI to trustworthy AI},
   volume = {14},
   year = {2024},
}


@article{MathiszigLee2022,
 
   author = {Jakob F. Mathiszig-Lee and Finneas J.R. Catling and S. Ramani Moonesinghe and Stephen J. Brett},
   doi = {10.1038/s41746-022-00616-7},
   issn = {23986352},
   issue = {1},
   journal = {npj Digital Medicine},
   month = {12},
   publisher = {Nature Research},
   title = {Highlighting uncertainty in clinical risk prediction using a model of emergency laparotomy mortality risk},
   volume = {5},
   year = {2022},
}


@article{Xue2024,
   abstract = {To conduct a computational investigation to explore the influence of clinical reference uncertainty on magnetic resonance imaging (MRI) radiomics feature selection, modelling, and performance. This study used two sets of publicly available prostate cancer MRI = radiomics data (Dataset 1: n = 260; Dataset 2: n = 100) with Gleason score clinical references. Each dataset was divided into training and holdout testing datasets at a ratio of 7:3 and analysed independently. The clinical references of the training set were permuted at different levels  and repeated 20 times. Four feature selection algorithms and two classifiers were used to construct the models. Cross-validation was employed for training, while a separate hold-out testing set was used for evaluation. The Jaccard similarity coefficient was used to evaluate feature selection, while the area under the curve (AUC) and accuracy were used to assess model performance. An analysis of variance test with Bonferroni correction was conducted to compare the metrics of each model. The consistency of the feature selection performance decreased substantially with the clinical reference permutation. The performances of the models were also associated with larger uncertainties and an increasing number of permuted clinical references. Clinical reference uncertainty can substantially influence MRI radiomic feature selection and modelling. The high accuracy of clinical references should be helpful in building reliable and robust radiomic models. Careful interpretation of the model performance is necessary, particularly for high-dimensional data.},
   author = {Cindy Xue and Jing Yuan and Gladys G. Lo and Darren M.C. Poon and Winnie C.W. Chu},
   doi = {10.1186/s42492-024-00180-9},
   issn = {25244442},
   issue = {1},
   journal = {Visual Computing for Industry, Biomedicine, and Art},
   keywords = {Clinical reference,Magnetic resonance imaging,Prostate cancer,Radiomics,Reliability},
   month = {12},
   publisher = {Springer},
   title = {Computational analysis of variability and uncertainty in the clinical reference on magnetic resonance imaging radiomics: modelling and performance},
   volume = {7},
   year = {2024},
}

@article{Bartolucci2021,
   abstract = {For the analysis of COVID-19 pandemic data, we propose Bayesian multinomial and Dirichlet-multinomial autoregressive models for time-series of counts of patients in mutually exclusive and exhaustive observational categories, defined according to the severity of the patient status and the required treatment. Categories include hospitalized in regular wards (H) and in intensive care units (ICU), together with deceased (D) and recovered (R). These models explicitly formulate assumptions on the transition probabilities between these categories across time, thanks to a flexible formulation based on parameters that a priori follow normal distributions, possibly truncated to incorporate specific hypotheses having an epidemiological interpretation. The posterior distribution of model parameters and the transition matrices are estimated by a Markov chain Monte Carlo algorithm that also provides predictions and allows us to compute the reproduction number (Formula presented.). All estimates and predictions are endowed with an accuracy measure obtained thanks to the Bayesian approach. We present results concerning data collected during the first wave of the pandemic in Italy and Lombardy and study the effect of nonpharmaceutical interventions. Suitable discrepancy measures defined to check and compare models show that the Dirichlet-multinomial model has an adequate fit and provides good predictive performance in particular for H and ICU patients.},
   author = {Francesco Bartolucci and Fulvia Pennoni and Antonietta Mira},
   doi = {10.1002/sim.9129},
   issn = {10970258},
   issue = {24},
   journal = {Statistics in Medicine},
   keywords = {Dirichlet-multinomial distribution,epidemic modeling,model diagnostics,multinomial distribution,pandemic predictions,reproduction number},
   month = {10},
   pages = {5351-5372},
   pmid = {34374438},
   publisher = {John Wiley and Sons Ltd},
   title = {A multivariate statistical approach to predict COVID-19 count data with epidemiological interpretation and uncertainty quantification},
   volume = {40},
   year = {2021},
}


@article{Heinze2018,
  title = {Variable selection - A review and recommendations for the practicing statistician},
  author = {Heinze, G. and Wallisch, C. and Dunkler, D.},
  journal = {Biometrical Journal},
  volume = {60},
  number = {3},
  pages = {431--449},
  year = {2018},
  month = {May},
  doi = {10.1002/bimj.201700067},
  pmid = {29292533},
  pmcid = {PMC5969114},
  note = {Epub 2018 Jan 2}
}

@article{Yan2024,
   abstract = {The statistical methodology for model-based dose finding under model uncertainty has attracted increasing attention in recent years. While the underlying principles are simple and easy to understand, developing and implementing an efficient approach for binary responses can be a formidable task in practice. Motivated by the statistical challenges encountered in a phase II dose finding study, we explore several key design and analysis issues related to the hybrid testing-modeling approaches for binary responses. The issues include candidate model selection and specifications, optimal design and efficient sample size allocations, and, notably, the methods for dose-response testing and estimation. Specifically, we consider a class of generalized linear models suited for the candidate set and establish D-optimal designs for these models. Additionally, we propose using permutation-based tests for dose-response testing to avoid asymptotic normality assumptions typically required for contrast-based tests. We perform trial simulations to enhance our understanding of these issues.},
   author = {Zhiwu Yan and Min Yang},
   doi = {10.1002/sim.10082},
   issn = {10970258},
   issue = {12},
   journal = {Statistics in Medicine},
   keywords = {MCP-Mod,dose finding,model uncertainty,optimal design,permutation test},
   month = {5},
   pages = {2472-2485},
   pmid = {38605556},
   publisher = {John Wiley and Sons Ltd},
   title = {Statistical considerations in model-based dose finding for binary responses under model uncertainty},
   volume = {43},
   year = {2024},
}


@article{Ko2024,
   abstract = {The objective of this study was to explore the mediation effects of coping strategies on the relationship between uncertainty and quality of life in Korean women with gynecological cancer. Mishel's Uncertainty in Illness Theory and Lazarus and Folkman's Stress and Coping Theory were used to guide the study. Three coping strategies (problem-focused, active emotional, and avoidant emotional) partially mediated the relationship between uncertainty and quality of life. This work provides evidence that reducing uncertainty has significant effects on coping strategies and positively affects the quality of life in women with gynecological cancer.},
   author = {Eungil Ko and Yaelim Lee},
   doi = {10.1097/ANS.0000000000000507},
   issn = {15505014},
   issue = {3},
   journal = {Advances in Nursing Science},
   keywords = {adaptation,genital neoplasms,oncology nursing,quality of life,uncertainty},
   month = {7},
   pages = {E84-E95},
   pmid = {37498078},
   publisher = {Lippincott Williams and Wilkins},
   title = {The Effects of Coping Strategies Between Uncertainty and Quality of Life of Korean Women With Gynecological Cancer: Evaluation of Uncertainty in Illness Theory and Stress and Coping Theory},
   volume = {47},
   year = {2024},
}


@article{Meghan2024,
   abstract = {Background Individuals with a strong family history of pancreatic cancer or a known hereditary cancer syndrome that is associated with pancreatic cancer are considered at high risk for developing pancreatic cancer. Living with a high risk for often fatal cancer is accompanied by high levels of uncertainty. Uncertainty is also independently associated with negative health outcomes. By understanding issues, sources, and responses to uncertainty, targeted supportive care strategies can be provided. Objectives This study aimed to examine how uncertainty manifests in the experience of being at high risk to develop pancreatic cancer and to describe issues, sources of, and responses to uncertainty. Methods In this secondary qualitative descriptive study, we analyzed 19 interviews with persons living with inherited pancreatic cancer risk. Analysis was guided by a conceptual framework of uncertainty and responses to uncertainty. Results Participants described multiple personal, practical, and scientific issues of uncertainty, centering on what to expect for their future health. Participants also expressed positive and negative cognitive, emotional, and behavioral responses to uncertainty, including engaging in surveillance. Uncertainty sources were both individual experiences as well as perceptions of healthcare provider uncertainty with managing pancreatic cancer risk. Conclusion Pancreatic cancer risk includes issues of uncertainty related to personal mortality, defining and managing risk, and experiencing surveillance. Positive and negative responses to this uncertainty could be targeted through interventions. Implication for Practice The oncology nurse should assess for sources of and responses to uncertainty in persons at risk for pancreatic cancer and offer psychosocial and educational support.},
   author = {Meghan L. Underhill-Blazey and Yingzi Zhang and Susan Stanek and Sally Norton},
   doi = {10.1097/NCC.0000000000001171},
   issn = {15389804},
   issue = {1},
   journal = {Cancer Nursing},
   keywords = {Oncology nursing,Pancreatic cancer risk,Response to uncertainty,Uncertainty},
   month = {1},
   pages = {E10-E17},
   pmid = {36480347},
   publisher = {Lippincott Williams and Wilkins},
   title = {The Experience of Uncertainty in Individuals with High Risk for Pancreatic Cancer},
   volume = {47},
   year = {2024},
}


@article{Liebermann2024,
   abstract = {Purpose: Explore mothers of adolescents' use of social media and the influence of social media on hesitancy regarding HPV vaccine. Methods: A national online survey of mothers of adolescents aged 9–17 years was conducted in August 2023, with participants recruited from an online research panel of US residents. The study examined socio-demographic factors, social media use patterns, and influence of social media and their association with HPV vaccine hesitancy. Results: Survey sample included 3968 mothers of adolescents.  No significant associations were found with the number of daily-used social media platforms or influence from other platforms. Discussion: Our findings highlight the impact of uncertainty about social media messages and its effect on parents' HPV vaccine hesitancy. Our findings also highlight the potential role of health care providers in reducing vaccine hesitancy during clinical encounters. Future research is needed to better understand the elements (content, approach, platforms) of effective social media communication interventions to decrease vaccine hesitancy and improve HPV vaccination rates among adolescents in the US.},
   author = {Erica Liebermann and Melanie Kornides and Masako Matsunaga and Eungung Lim and Gregory Zimet and Gary Glauberman and Cable Kronen and Holly B. Fontenot},
   doi = {10.1016/j.vaccine.2024.126571},
   issn = {18732518},
   journal = {Vaccine},
   keywords = {Adolescent vaccination,Human papillomavirus (HPV) vaccine,Social media,Vaccine hesitancy},
   month = {1},
   publisher = {Elsevier Ltd},
   title = {Use of social media and its influence on HPV vaccine hesitancy: US National Online Survey of mothers of adolescents, 2023},
   year = {2024},
}


@article{Zheng2024,
   abstract = {In recent years, the automatic generation of radiology reports as an auxiliary solution for expert diagnosis has garnered considerable attention from researchers. However, due to the complexity of medical image interpretation, current models exhibit issues such as aleatoric uncertainty and epistemic uncertainty, leading to a lack of stability in the content description of the generated medical reports. To address these issues, we propose a Team Role Interaction Network (TRINet) for the automatic generation of radiology reports, which is composed of multiple Team-member role models and a Team-leader role model. Specifically, we proposed a Cross-Modal Communication Mechanism (CMCM) among Team-members, enabling each Team-member to interact with image features and textual features output by its adjacent Team-member role model through a predefined grid-shaped parameter plane queries, thereby facilitating cross-modal information exchange among Team-members. Additionally, the Team-leader role model employs a Multi-Modal Fusion Mechanism (MMFM), performing sequence-to-sequence operations on the multidimensional outputs generated by the Team-member role models and the original inputs, aggregating the knowledge of each Team-member to produce the final medical report. We tested TRINet on two public benchmark datasets (IU X-ray and MIMIC-CXR), demonstrating the effectiveness and state-of-the-art performance of our model. The BLEU-4 indicator on the MIMIC-CXR test set reached the latest 0.144, 3.6 points higher than the previous best technique. Further research has shown that TRINet can effectively leverage the complementary information between the modalities perceived by each Team-member role model, simulating the collaborative process of an expert team, thereby significantly improving the system's accuracy and robustness.},
   author = {Zhiqiang Zheng and Yujie Zhang and Enhe Liang and Zhi Weng and Jun Chai and Jianxiu Li},
   doi = {10.1016/j.compbiomed.2024.109275},
   issn = {18790534},
   journal = {Computers in Biology and Medicine},
   keywords = {Cross-modal communication,Medical image captioning,Radiology report generation,Team role interaction},
   month = {12},
   publisher = {Elsevier Ltd},
   title = {TRINet: Team Role Interaction Network for automatic radiology report generation},
   volume = {183},
   year = {2024},
}


@book{russell2020artificial,
  title     = {Artificial Intelligence: A Modern Approach},
  author    = {Stuart J. Russell and Peter Norvig},
  edition   = {4},
  year      = {2020},
  publisher = {Pearson},
  isbn      = {9780134610993},
  url       = {http://aima.cs.berkeley.edu/}
}

@article{lewis2024,
  author    = {Peter R. Lewis and Ştefan Sarkadi},
  title     = {Reflective Artificial Intelligence},
  journal   = {Minds \& Machines},
  volume    = {34},
  number    = {14},
  year      = {2024},
  doi       = {10.1007/s11023-024-09664-2},
  url       = {https://doi.org/10.1007/s11023-024-09664-2}
}
@misc{naderi2025,
      title={Self-Reported Confidence of Large Language Models in Gastroenterology: Analysis of Commercial, Open-Source, and Quantized Models}, 
      author={Nariman Naderi and Seyed Amir Ahmad Safavi-Naini and Thomas Savage and Zahra Atf and Peter Lewis and Girish Nadkarni and Ali Soroush},
      year={2025},
      eprint={2503.18562},
      archivePrefix={arXiv},
      primaryClass={cs.CL},
      url={https://arxiv.org/abs/2503.18562}, 
}
